Multivariate Hypergeometric Terms

In this 1997 Ph.D. dissertation we prove a piecewise form of the discrete part of Wilf and Zeilberger's 1992 conjecture that a hypergeometric term is proper if and only if it is holonomic. We show that a holonomic hypergeometric term on $Z^n$ is piecewise proper and we show that without such a qualification the conjecture is false. We call a term piecewise proper if $Z^n$ can be expressed as the union of a finite number of polyhedral regions (the "pieces") and a set of measure zero (which we define to be a finite union of hyperplanes) such that the restriction of the term to each polyhedral region is proper. We prove a similar result for terms that are not holonomic but honest. We call a term $h$ honest if for every vector $v$ in $Z^n$ there exist relatively prime polynomials $A_v$ and $B_v$ such that $A_v(z) h(z) = B_v(z) h(z+v)$ except on a set of measure zero. We also give a naive proof of the Ore--Sato Theorem using Gosper's Lemma. We solve an unrelated problem of Cameron by showing that there is a sum-free complete subset of $Z/mZ$ that is not symmetric for every sufficiently large modulus $m$, and we show that such a set must have the property that the cardinality of its sum set is greater than the cardinality of its difference set, which makes it a counterexample to a modular version of a conjecture of Conway. A set $S$ is said to be sum-free, complete, and symmetric respectively if $|S+S| \subset S^c$, $|S+S| \supset S^c$, and $S = -S$.

==> ack.tex <==
\hyperdef\chapteRAcknowledgements{ChapterSection}{chapteRAcknowledgements}{}

I would like to thank my advisor, George Andrews, for his infinite
patience and extraordinary generosity.  Without his support and
encouragement I would not have written this dissertation
or even come to graduate school (twice).

I am grateful to Jim Humphreys for writing the PSU Thesis Style
and for magically transforming my scribble into type with incredible
speed.

I would like to thank Leonid Vasserstein for showing me some
interesting mathematics and some excellent blackberry patches.

This thesis is dedicated to the divisibility of 28 by 7, without which I
might not have met Jenae, my wife.


==> errata.tex <==

\catcode`\@=11


\nopagenumbers
\headline={\hfil}
\he@dp@ge


\par{\centerline{\fourteenbf Corrigenda}}
\bigskip

\noindent
p. 6.
\vtop{
\noindent
``term on $\Z^k$ $f$''
has been corrected to read
``term $f$ on $\Z^k$''
.
}

\bigskip
\noindent
p. 14.
\vtop{
\noindent
``hence $d^{T_j} \mid Y(S_j)$''
has been corrected to read
``hence $d^{T_i} \mid Y(S_j)$''
.
}

\bigskip
\noindent
p. 17.
\vtop{
\noindent
``Let $A$ and $B$ be invertible $k \times k$ matrices''
has been corrected to read
``Let $A$ and $B$ be invertible $r \times r$ and $k \times k$ matrices
respectively''
.
}

\bigskip
\noindent
p. 25.
\vtop{
\noindent
Near the bottom of the page, 
``$r_i= $''
has been corrected to read
``$R_i= $''
.
}

\bigskip
\noindent
pp. 4, 36.
\vtop{
\noindent
``$\{\z\colon\v\cdot\z=0\}$, where  $\v$ $\ldots$
 $\{\z\colon\v\cdot\z>0\}$, where  $\v$''
has been corrected to read
``$\{\z\colon\v\cdot\z=n\}$, where $n\in\Z$ and  $\v$ $\ldots$
 $\{\z\colon\v\cdot\z>n\}$, where $n\in\Z$ and  $\v$''
.
}

\bigskip
\noindent
p. 38.
\vtop{
\noindent
``degree at most $k-1$'' has been corrected to read
``degree at most $n-1$''
}

\bigskip
\noindent
p. 41. 
\vtop{
\noindent
``$j-a_j$''
has been corrected to read
``$j-a_t$''
.
}

\bigskip
\noindent
p. 42. 
\vtop{
\noindent
Both occurances of
``$z_1 < 1$''
have been corrected to read
``$z_1 < 0$''
and ``$j-a_j$'' has been corrected to read ``$j-a_1$''
.
}

\bigskip
\noindent
p. 45.
\vtop{
\noindent
``entirely in $\R'.$''
has been corrected to read
``entirely in $\R$.''
.
}


\bigskip
\noindent
p. 57.
\vtop{
\noindent
``implies $f(\z+\v) \ne 0$ for some $\v \in V$''
has been corrected to read
``implies $f(\z+\v) \ne 0$ for some $\v \in V_i$''.
}


\bigskip
\noindent
p. 58.
\vtop{
\noindent
``$\sum_{z_k<0}f(z_1,\ldots,z_k)y^{z_k}$''
has been corrected to read
``$\sum_{z_k<0}f(z_1,\ldots,z_k)y^{-z_k}$''
.
}


\bigskip
\noindent
p. 61.
\vtop{
\noindent
``there exists $\u_j\in\Q_{i,j}\cap\ \rgal d$ such that $\u_j\notin\Q_i$.''
has been corrected to read
``there exists $\u_j\in\Q_{1,j}\cap\ \rgal d$ such that $\u_j\notin\Q_1$.''
}

\bigskip

\noindent
\hyperdef\oresato{Corrigendum}{Ore-Sato}{}
The author was unaware that Theorem~\hyperref\thmfifteena{\ref[thm:15a]}  is due to 
O. Ore [1] in the case of two variables
 and 
M. Sato [2] in the general case.

\noindent
[1] \space 
\vtop{
\hsize=5.7truein
\hoffset=0.5truein
\noindent
O. Ore, Sur la forme de fonctions hyperg\'eom\'etriques de plusieurs variables, 
J. 
Math. Pures et Appl. 9 (1930), 311-327.}


\bigskip
\noindent
[2]  \space
\vtop{
\hsize=5.7truein
\hoffset=0.5truein
\noindent 
M. Sato, Theory of Prehomogeneous Vector Spaces, Nagoya Math.
J. 120 
(1990), 
1-34.}







==> five.tex <==
\hyperdef\chapteRv{ChapterSection}{chapteRv}{}
\Chapter A Solution to a Problem of Cameron\\ 
On Sum-free Complete Sets


\hyperdef\chapteRvSECi{ChapterSection}{chapteRvSECi}{}
\Section Introduction

For any subsets $A$ and $B$ of an additive group $G$, define
$A+B=\{a+b:a \in A \text{ and } b \in B \}$ and $-A= \{-a:a
\in A \}$.  A subset $S$ of $G$ is said to be sum-free,
complete, and symmetric respectively if $S+S \subset S^\c$,
$S+S \supset S^\c$, and $S=-S$.  Hence, $S$ is sum-free and
complete if and only if $S+S=S^\c$.


Cameron observed that for any sufficiently small modulus $m$, 
every sum-free complete set in $\Z/m\Z$ is also symmetric.
In fact, Calkin found that $m=36$ is the smallest modulus  for which
there is a sum-free complete set that is not
symmetric \hyperref\CamPortrait{\bibref[CamPortrait]}.  Cameron asked if there exists
such a set for all sufficiently large moduli \hyperref\CamPortrait{\bibref[CamPortrait]}.
We answer Cameron's question by showing
there exists such a set for all moduli greater than or 
equal to $890626$.

We also show that every sum-free complete set in $\Z/m\Z$ that
is not symmetric can be used to construct a counterexample
to a conjecture of J.H.~Conway.  
 Conway conjectured that for any finite set
$S$ of integers, $|S+S| \le |S-S|$.  
Conway's conjecture
was disproved by Marica \hyperref\Marica{\bibref[Marica]}.  Later Stein showed
how to make the ratio ${|S+S|}/{|S-S|}$ arbitrarily large
\hyperref\Stein{\bibref[Stein]}.  We show that if $S$ is sum-free and complete
modulo $m$ but not symmetric, then $|S+S|>|S-S|$; hence, $S$
is a counterexample to a modular version of Conway's conjecture.
Further, we show that if $S' \subset \Z$ is a certain set
derived from $S$, then $|S'+S'| > |S'-S'|$; hence, $S'$ is a
counterexample to Conway's conjecture proper.

The history of sum-free sets begins with Schur who 
showed that the positive integers can not be partitioned
into finitely many sum-free sets \hyperref\Schur{\bibref[Schur]}.  Sum-free sets
have been used to find lower bounds for Ramsey numbers
(see pp.~28, 128, 264 in~\hyperref\Wallis{\bibref[Wallis]}).  Cameron describes  some
applications of sum-free sets and poses several problems
\hyperref\CamGraph{\bibref[CamGraph]},\hyperref\CamStructure{\bibref[CamStructure]},\hyperref\CamPortrait{\bibref[CamPortrait]}.  George Andrews
observed that sum-free complete
sets play a role in partition identities (personal communication). 
For example, the
set $\{1,4\} \in \Z/5\Z$, which arises in the Rogers-Ramanujan
Identities (p.~109 in~\hyperref\Andseventysix{\bibref[And76]}), is sum-free, complete,
and symmetric.  Calkin showed that the number of sum-free
sets contained within the first $n$ integers is $o(2^{n(1/2
+\epsilon)})$ for every $\epsilon > 0$ \hyperref\Calkin{\bibref[Calkin]}.  



\hyperdef\chapteRvSECii{ChapterSection}{chapteRvSECii}{}
\Section Cameron's problem

For any $S \subset \Z$ and $a$, $b \in \Z \cup \{-\infty,\infty\}$
define $S_a^b=\{s \in S : a \le s \le b \}$.
The following sets $S_1, \dots, S_5$ are used as building
blocks in the construction of infinite families of modular
sum-free complete sets that are not symmetric.
Define 
$$ 
\align
S_1&= 
   (-3+5\Z)_{-\infty}^{-354} \cup 
   (F_1)_{-353}^{353} \cup 
   (3+5\Z)_{354}^{\infty}, \\
S_2&= 
   (-1+5\Z)_{-\infty}^{-192} \cup 
   (F_2)_{-191}^{191} \cup 
   (1+5\Z)_{192}^{\infty}, \\
S_3&= 
   (-4+5\Z)_{-\infty}^{-185} \cup 
   (F_3)_{-184}^{184} \cup 
   (4+5\Z)_{185}^{\infty}, \\
S_4&= 
   (-2+5\Z)_{-\infty}^{-253} \cup 
   (F_4)_{-252}^{252} \cup 
   (2+5\Z)_{253}^{\infty}, 
	\quad \text{and} \\ 
S_5&= 
   (-1+3\Z)_{-\infty}^{-95} \cup 
   (F_5)_{-94}^{94} \cup 
   (1+3\Z)_{95}^{\infty}, \\
\endalign
$$ where 
$$ 
\allowdisplaybreaks
\align 
F_1=&  \{-6, 3\} \cup  \pm \{1, 8, 13, 17, 22, 27, 38, 42, 53, 58, 
62, 67, 72, 74, 86, 88, 93, 98, 107, \\ 
& \quad 117, 119, 121, 133,137, 142, 147, 152, 168, 173, 178, 182, 
187, 192, 197, 208, \\ 
& \quad 213, 218, 222, 227,232, 243, 248, 253,
288, 293, 298, 323, 328, 333, 338\},  \\ 
F_2=&  \{-6, 3\} \cup
\pm \{1, 8, 13, 17, 22, 27, 38, 42, 53, 58, 62, 72, 74, 86, 88,
93, 109, 119, \\ 
&\quad   121, 156, 166\},  \\ 
F_3=&  \{-6, 3\}
\cup  \pm \{1, 8, 13, 17, 22, 27, 38, 42, 53, 58, 62, 67, 72, 74,
86, 88, 93, 98, 119, \\ 
&\quad   149, 154,159,164,169\},  \\ 
F_4=&
\{-6, 3\} \cup  \pm \{1, 8, 13, 17, 22, 27, 38, 42, 53, 58, 62,
67, 72, 74, 86, 88, 93, 98, 107,  \\ 
&\quad  117, 119, 121, 133,
137,142, 147, 152, 182, 187, 192, 197, 202, 222, 227, 232, \\ 
&\quad
237, 247\}, \quad \text{and}   \\ 
F_5=&  \{ -1, 2 \} \cup  \pm \{5,
8, 14, 17, 29, 40, 44, 47, 67, 70, 79, 82, 85\}. \\ 
\endalign 
$$


Lemma~\hyperref\lemfivedashone{\ref[lem:5-1]} reduces to a computation the problem of determining
if a set of the form of $S_1, \dots , S_5$ is sum-free and
complete.

\Lemma[lem:5-1]  \hyperdef\lemfivedashone{Lemma}{5-1}{} Let $S = (A+m\Z)_{-\infty}^{-a} \cup
F_{-a+1}^{b-1} \cup (B+m \Z)_b^{\infty}$ where $a$, $b$, and
$m$ are positive integers and  $A$, $F$, and $B \subset
\Z$.  The set $S$ is sum-free and complete in $\Z$  if and only if
$$(S^\c)_{-2a-2m}^{2b+2m} = (S_{-(2a+b+3m)}^{2b+a+3m}
+ S_{-(2a+b+3m)}^{2b+a+3m})_{-2a-2m}^{2b+2m}.$$
\LemmaStop

\Proof Let $i=-(2a+2m)$, $j=2b+2m$,
$k=-(2a+2b+3m)$, and $l=2b+a+3m$.  We need to show that $S$ 
is sum-free and complete if and only if $(S^\c)_{i}^{j}
= (S_{k}^{l}+S_{k}^{l})_{i}^{j}$.  We first show that $S $ is
sum-free and complete if and only if $(S^\c)_{i}^{j} = 
(S+S)_{i}^{j}$, and then show that $(S+S)_{i}^{j} =
(S_{k}^{l}+S_{k}^{l})_{i}^{j} $.  
To prove the first assertion
it suffices to show that if $(S^\c)_{i}^{j} = (S+S)_{i}^{j}$,
then $S$ is sum-free and complete; the implication in the
other direction is trivial. 

We show that if $(S^\c)_{i}^{j} = (S+S)_{i}^{j}$, then $S$
is sum-free.  Suppose the contrary and let $s_1$, $s_2$, and
$s_3 \in S$ be such that $s_1+s_2=s_3$ and $|s_3|$ is minimal.
By assumption $(S+S)_{i}^{j} \subset
S^\c$, so $s_3 > j$ or $s_3 < i$.  We consider the case $s_3
> j$. Let $s_3'=s_3-m$. Since $s_3 > j > b+m$, it follows that $s_3 \in
(B+m\Z)_b^{\infty}$ and $s_3' \in (B+m\Z)_b^{\infty}$.
Since $s_3 \ge 2b+2m$, it follows that $s_1 \ge b+m$ or $s_2
\ge b+m$.  We may assume without loss of generality that $s_1 \ge
b+m$. Let $s_1'=s_1-m$.  
Since $s_1 \ge b+m$, it follows that $s_1 \in (B+m \Z)_b^{\infty}$ and
$s_1' \in (B+m \Z)_b^{\infty}$.  But $s_1'+s_2=s_3'$ and $|s_3'|<|s_3|$,
contradicting the minimality of $|s_3|$.  The case $s_3 < i$ is
similar.

We show that if $(S^\c)_{i}^{j} = (S+S)_{i}^{j}$, then $S$
is complete.  Suppose the contrary and let $c \in S^\c$ be
such that $c \notin S+S$ and $|c|$ is minimal.
By assumption, $(S^\c)_{i}^{j} \subset S+S$, so $c > j$ or
$c < i$.  We consider the case $c > j$.  
Let $T=(B+m\Z)^\c$. 
Since 
$c > j > b +m$, 
it follows that 
$c \in T_{b+m}^{\infty}$. 
Let $c'=c-m$.
Since $T=T+m\Z$, 
it follows that
$c' \in T_b^{\infty} \subset S^\c$.  
By the minimality of $|c|$, it follows that  $c'=s_1+s_2$ where $s_1$ and $s_2
\in S$.  Since $c' > j-m > 2b$, it follows that $s_1 \ge b$
or $s_2 \ge b$.  We may assume without loss of generality that
$s_1 \ge b$.  Let $s_1'=s_1+m$. Since $s_1 \ge b$, it follows that 
$s_1 \in (B+m\Z)_b^{\infty}$ and hence 
$s_1' \in (B+m\Z)_b^{\infty}$.
But $c=s_1'+s_2$ contradicting the assumption $c \notin S+S$.
The case $c < i$ is similar.

We complete the proof by showing that $(S+S)_{i}^{j} =
(S_{k}^{l}+S_{k}^{l})_{i}^{j}$.  It suffices to show that
$(S+S)_{i}^{j} \subset S_{k}^{l}+S_{k}^{l}$.  Let $c \in
(S+S)_{i}^{j}$ and let $s_1$ and $s_2 \in S$ be such that $s_1
+s_2=c$ and $|s_1| + |s_2|$ is minimal.  We claim that $s_1$,
$s_2 \in S_{k}^{l}$ and, hence, $c \in (S_{k}^{l}+S_{k}^{l})_{i}^{j}$.
Suppose to the contrary $s_1 > l$ or $s_1 < k$.  We consider
the case $s_1 > l$.  Let $s_1'=s_1-m$ and $s_2'=s_2+m$. Since
$s_1 > l > b+m$, it follows that $s_1 \in (B+m \Z)_b^{\infty}$
and $s_1' \in (B+m\Z)_b^{\infty}$.  Since $s_1 >l= 2b+a +3m$
and $c \le 2b+2m$, it follows that $s_2=c-s_1 \le -a -m$.
Since $s_2 \le -a-m$, it follows that $s_2 \in (A+m
\Z)_{-\infty}^{-a}$ and $s_2' \in (A+m \Z)_{-\infty}^{-a}$.
But $s_1'+s_2'=c$ and $|s_1'|+|s_2'|<|s_1|+|s_2|$, 
contradicting the minimality of $|s_1|+|s_2|$.
Hence, the claim is true in the case $s_1 > l$.  The case $s_1
< k$ is similar.
\ProofStop

Using Lemma~\hyperref\lemfivedashone{\ref[lem:5-1]}, it is easily shown that the sets $S_1,\dots,S_5$
are sum free and complete.  Taking $F=F_1$, $a=b=354$, $m=5$,
and $-A=B=\{3\}$ and verifying that $((S_1)^\c)_{-718}^{718}
= ((S_1)_{-1077}^{1077}+(S_1)_{-1077}^{1077})_{-718}^{718}$,
it follows from Lemma~\hyperref\lemfivedashone{\ref[lem:5-1]} that $S_1$ is sum-free and complete.
The cases corresponding to $S_2,\dots,S_5$ are proved similarly.




Let $T\subset \Z$ and let $n$ be a positive integer.
A sum-free complete set of the form $T + n\Z$ can
be identified with a sum-free complete set modulo $n$; 
the subset $T+n\Z$ of $\Z$ is sum-free and complete if and only 
if the subset $\{t+n\Z:t \in T\}$ of $\Z/n\Z$ is sum-free and 
complete.
Lemma~\hyperref\lemfivedashtwo{\ref[lem:5-2]} shows that a sum-free complete set of the form of
$S_1,\dots,S_5$ can be used to construct a sum-free complete set modulo
$n$ for all sufficiently large $n$ in an arithmetic progression.

\Lemma[lem:5-2]  \hyperdef\lemfivedashtwo{Lemma}{5-2}{} Let $S=(A+m\Z)_{-\infty}^{-a} \cup
F_{-a+1}^{b-1} \cup (B+m\Z)_b^{\infty}$ where $a$, $b$ and
$m$ are positive integers, $A$, $F$ and $B \subset \Z$, and
for some integer $d$, $d+A+m \Z=B+m \Z$.  If $S $ is sum-free
and complete in $\Z$, then $S_{-n/2}^{n/2} +n \Z$ is sum-free and
complete in $\Z$ for all $n$ such that $n \ge 2m+ 4\max(a,b)-2\ $ and
$\ n\cong d \pmod m$.
\LemmaStop

\Proof Let $n$ be such that $n \ge 2m+
4\max(a,b)-2$ and $n\cong d \pmod m$.

We show that $S_{-n/2}^{n/2} +n \Z$ is sum-free. Suppose the
contrary and let $s_1$, $s_2$, and $s_3 \in S_{-n/2}^{n/2} $
be such that $s_1+s_2\cong s_3 \pmod n$.  Since $|s_1+s_2-s_3| \le
|s_1|+|s_2|+|s_3| \le 3n/2 $ and $s_1+s_2-s_3 \neq 0$, it
follows that $s_1+s_2-s_3= \pm n$.  We consider the case
$s_1+s_2-s_3=n$.  Let $\sg(1)=\sg(2)=-\sg(3)=1$. 
If for all $i\in \{1,2,3\}$
either $s_i \in F_{-a+1}^{b-1}$ or $s_i \sg(i) \le
0$, then $s_1+s_2-s_3 \le 3b < n$, so we may assume there
exists $j=1$, $2$, or $3$ such that $s_j \notin F_{-a+1}^{b-1}$
and $s_j \sg(j) >0$.  In fact, we may assume without loss of
generality that either $j=1$ or $j=3$.

We consider the case $j=1$. Let $s_1'=s_1-n$. 
Since $s_1 \notin F_{-a+1}^{b-1}$ and $s_1 >0$,  
it follows that $s_1 \in B+m\Z$
and $s_1' \in B+m\Z-n$.  Since $n\cong d \pmod m$, it follows
that $m\Z-n=m\Z-d$. Hence, $s_1' \in B+m\Z-d=A+m\Z$.  Since
$s_1 \le n/2$, it follows that $s_1' \le -n/2 \le -a$.  Hence,
$s_1' \in (A+m\Z)_{-\infty}^{-a} \subset S$.  But $s_1'+s_2=s_3$,
contradicting the assumption that $S$ is sum-free.

The case $j=3$ is similar.  This completes the proof in the
case $s_1+s_2-s_3=n$.  The case $s_1+s_2-s_3=-n$ is similar.
We have shown that $S_{-n/2}^{n/2} +n \Z$ is sum-free.



We show $S_{-n/2}^{n/2} +n \Z$ is complete. Let $c \in S^\c$
be such that $|c| \leq n/2$.  We need to show that $c \cong t_1
+t_2 \pmod n$ for some $t_1$ and $t_2 \in S_{-n/2}^{n/2}$.
Since $S$ is complete, $c= s_1 + s_2$ for some $s_1$ and  $s_2
\in S$. Let $s_1$ and $s_2$ be such that $|s_1-s_2|$ is minimal.
If $s_1$ and $s_2$ have the same sign, $|s_1|+|s_2|=|c|\le
n/2$. Hence, $s_1$ and $s_2 \in S_{-n/2}^{n/2}$ and we are
done, so assume $s_1 >0$ and $s_2 <0$. 

We claim that  $s_1 <b+m$ or $s_2 >-a-m$. 
Suppose the contrary and let $s_1'=s_1-m$ and $s_2'=s_2+m$.  
Since $s_1 \ge b+m$, 
it follows that $s_1$ and $s_1' \in (B+m\Z)_b^\infty$. 
Hence,  $s_1' \in S$. Similarly,  $s_2' \in S$. 
But $s_1' +s_2'=c$ and $|s_1'-s_2'|<|s_1-s_2|$,
contradicting the minimality of $|s_1-s_2|$. Hence,
$s_1 <b+m$ or $s_2 >-a-m$ as claimed. 
 
We consider the case $s_2 >-a-m$.  If $s_1 \leq n/2$ we are 
done, so assume
$s_1 >n/2$ and let $s_1'=s_1-n$.  Since $s_1 > n/2 > b$, it
follows that $s_1 \in B+m\Z$.  Arguing as in the case $j=1$
above, $s_1' \in A+m\Z$.  Since $c \le n/2$ and $s_2 > -a-m$,
it follows that $s_1' = c-s_2-n < -n/2 +a+m $. Since $n \ge
2m +4a-2$, it follows that $ -n/2+ m +a \le -a +1$.  Hence,
$s_1' < -a+1$. Since $s_1' \le -a$ and $s_1' \in A+m\Z$, it
follows that $s_1' \in S$.  Since $s_1 >n/2$, it follows that
$s_1' > -n/2 $, and hence $s_1' \in S_{-n/2}^{n/2}$.  But
$s_1' +s_2 \cong c \pmod n$.  The case $s_1 <b+m$ is similar.
\ProofStop

\Theorem[thm:5-1]  \hyperdef\thmfivedashone{Theorem}{5-1}{} For all $n\ge 890626$,  there exists a sum-free complete set 
in $\Z/n\Z$ that is not symmetric.  
\TheoremStop


\Proof Applying Lemma~\hyperref\lemfivedashtwo{\ref[lem:5-2]} with $S=S_1$,
$A=\{-3\}$, $B=\{3\}$, $F=F_1$, $a=b=354$, $m=5$, and $d=1$,
it follows that for every $n$ such that $n \ge 1424 $ and $n
\cong 1 \pmod 5 $, the set $(S_1)_{-n/2}^{n/2} +n\Z$ is sum-free 
and complete.
Equivalently, for every $n$ such that $n \ge 1426 $ and $n \cong
1 \pmod 5 $, the set 
$T_n=\{s + n\Z : s \in (S_1)_{-n/2}^{n/2}  \} \subset
\Z/n\Z$ is sum-free and complete. Further, it is clear from
the form of $S_1$ that $3 \in T_n $ and $-3 \notin T_n$.
Hence, $T_n$ is not symmetric.  Thus, we have shown that
there is a sum-free complete set that is not symmetric for
all moduli in the set $R_1=\{m \geq 1426 : m \cong 1 \pmod 5
\}$.  Similar arguments using the sets $S_2, \dots S_5$ show
that there is a sum-free complete set that is not symmetric
for all moduli in sets
$R_2=\{m \geq 777 : m \cong 2 \pmod 5\} $, 
$R_3=\{m \geq 748 : m \cong 3 \pmod 5\} $, 
$R_4=\{m \geq 1024 : m \cong 4 \pmod 5\} $, and
$R_5=\{m \geq 386 : m \cong 2 \pmod 3\}$.

It is easily seen that if there is a sum-free complete set
that is not symmetric for the modulus $m$, then there is such
a set for any modulus that is a multiple of $m$.  Hence, there
is a sum-free complete set that is not symmetric for any
modulus with a divisor in the set $R= R_1 \cup R_2 \dots \cup
R_5$.

It remains only to show that for all $n \geq 890626$, $n$
has a divisor in the set $R$.  Let $n$ be greater than or
equal to $890626$ and write $n$ in the form $n=5^a b$ where
$b$ is not divisible by $5$.  Since $890626 = 5^4 \ 1425 +1$,
either $a \geq 5$ or $b \geq 1426$.  If $a \geq 5$, then
$5^5=3125$ divides $n$.  Since $3125 \in R_5$, it follows that
$3125 \in R$.  If $b \geq 1426$, then $b \in R$ since the set
$R_1 \cup R_2 \dots \cup R_4$ contains every number greater
than or equal to $1426$ that is not a multiple of $5$.  In
either case $n$ has a divisor in $R$.  We have shown that for
every $n$ greater than or equal to $890626$ there is a sum-free
complete set in $\Z/n\Z$ that is not symmetric.  
\ProofStop

The condition that $n\ge 890626$ in Theorem~\hyperref\thmfivedashone{\ref[thm:5-1]} is not sharp and can
undoubtedly be considerably reduced.






\hyperdef\chapteRvSECiii{ChapterSection}{chapteRvSECiii}{}
\Section Conway's conjecture

The following theorem shows that if $S$ is sum-free and complete
but not symmetric modulo $m$, then $S$ must be a counterexample
to a modular version of Conway's conjecture.

\Theorem[thm:5-2]  \hyperdef\thmfivedashtwo{Theorem}{5-2}{} If a set $S$ is sum-free and complete but
not symmetric modulo $m$, then $|S+S| > |S-S|$.
\TheoremStop

Before beginning the proof of Theorem~\hyperref\thmfivedashtwo{\ref[thm:5-2]}, it is useful to
observe that $S+S \subset S^\c$ if and only if $S-S \subset
S^\c$; there are no solutions $s_1,s_2,s_3 \in S$ to
$s_1+s_2=s_3$ if and only if there are no solutions to
$s_3-s_2=s_1$

\Proof Suppose to the contrary $S$ is
sum-free and complete but not symmetric modulo $m$ and $|S+S| \le
|S-S|$.  Since $S$ is sum-free, $S+S \subset S^\c$ and hence
$S-S \subset S^\c$.  Since $S^\c=S+S$, it follows that
$S-S \subset S+S$.  But $|S+S| \le |S-S|$, so $S-S = S+S$ and
hence $S-S = S^\c$.  The set $S-S$ is symmetric, hence
$S^\c$ is symmetric, hence $S$ is symmetric, contrary to
assumption.
\ProofStop

Theorem~\hyperref\thmfivedashthree{\ref[thm:5-3]} shows that if $S$ is sum-free and complete but not
symmetric modulo $m$, then $S$ can be used to construct a
counterexample to  Conway's conjecture.

\Theorem[thm:5-3]  \hyperdef\thmfivedashthree{Theorem}{5-3}{} Let $A \subset \Z/ m \Z$ be sum-free and
complete but not symmetric, let $r={|A-A|}/ {|A+A|} $, and
let $S$ be the set of integers congruent modulo $m$ to a member
of $A$.  For all $n \ge 2m/{(1-r)}$, we have ${|S_0^n+S_0^n|}
> {|S_0^n-S_0^n|}$.
\TheoremStop

We require the following lemma for the proof of Theorem~\hyperref\thmfivedashthree{\ref[thm:5-3]}.

\Lemma[lem:5-3]  \hyperdef\lemfivedashthree{Lemma}{5-3}{} Let $A$, $B \subset \Z$, $S=A+m \Z$, and
$T=B+m \Z$.  For any integers $i$, $j$, $k$, and $l$ such 
that $j-i\ge m-1$
and $k-l \ge m-1$, $$(S_i^j+T_k^l)_{i+k+m-1}^{j+l-m+1} =
(S+T)_{i+k+m-1}^{j+l-m+1}.  $$ 
\LemmaStop

\Proof To prove Lemma~\hyperref\lemfivedashthree{\ref[lem:5-3]}, we need only show $$(S_i^j+T_k^l)_{i+k+m-1}^{j+l-m+1}
\supset (S+T)_{i+k+m-1}^{j+l-m+1}, \tag 1$$ since the containment
in the other direction is trivial.  We first consider the case
$j-i = k-l = m-1$. Let $s=j+l-m+1=i+k+m-1$. Since $j-i \ge
m-1$, $S=S_i^j+ m \Z$.  Similarly, $T=T_k^l+ m \Z$.  Hence,
$$ 
\aligned
S+T &= (S_i^j+ m \Z)+(T_k^l+ m \Z)= S_i^j+T_k^l+ m \Z \\ 
&= S_i^j+T_k^l+ (m \Z_{-\infty}^{-1} 
	\cup \{0\} \cup m \Z_1^{\infty}) \\ 
&= (S_i^j+T_k^l+ m \Z_{-\infty}^{-1}) \cup (S_i^j+T_k^l)
      \cup (S_i^j+T_k^l+ m \Z_1^{\infty}) \\ 
&\subset \Z_{-\infty}^{j+l-m} 
	\cup (S_i^j+T_k^l) \cup \Z^{\infty}_{i+k+m}\\
&\subset \Z_{-\infty}^{s-1} \cup (S_i^j+T_k^l) 
	\cup \Z^{\infty}_{s+1}.  
\endaligned 
$$ 
It follows that $(S_i^j+T_k^l)_s^s
\supset (S+T)_s^s$ which is that statment of (1) for the
case $j-i = k-l = m-1$.

We derive the general case from the previous one.  Let $j-i
\ge m-1$, $k-l \ge m-1$ and define $ I=\{(a,b,c,d) :\Z_a^b
\subset \Z_i^j,\ \Z_c^d \subset \Z_k^l, \text{ and }b-a=d-c=m-1
\}$.  
$$ \split (S_i^j+T_k^l)_{i+k+m-1}^{j+l-m+1} &\supset
\bigcup_{(a,b,c,d) \in  I} (S_a^b+T_c^d)_{a+c+m-1}^{b+d-m+1}\\ 
&\supset \bigcup_{(a,b,c,d) \in I} (S+T)_{a+c+m-1}^{b+d-m+1}
\text{\quad by the previous case} \\ &\supset 
(S+T)_{i+k+m-1}^{j+l-m+1}, \endsplit $$ so (1) is proved.
\ProofStop

\Proof We now prove Theorem~\hyperref\thmfivedashthree{\ref[thm:5-3]}. Let $n \ge 2m/{(1-r)}$. By Theorem~\hyperref\thmfivedashtwo{\ref[thm:5-2]}, $r <1$
so $n \ge m-1$. Hence, by Lemma~\hyperref\lemfivedashthree{\ref[lem:5-3]}, $$(S_0^n+S_0^n)_{m-1}^{2n-m+1}
= (S+S)_{m-1}^{2n-m+1} = (S+S)_{m-1}^{m-1+km-1} \supset
(S+S)_{m-1}^{m-1+\floor k m-1}\quad , $$ where $k = (2n-2m+3)/m$ and
$\floor k$ is the greatest integer less than or equal to $k$.
Since $S+S$ is the set of integers congruent modulo $m$ to a
member of $A+A$, it follows that $|(S+S)_{a}^{a+im-1}| =
i|A+A|$ for any $a$ and $i \ge 0$.  In particular,
$|(S+S)_{m-1}^{m-1+\floor k m-1}| = \floor k|A+A|$.  Hence
$|S_0^n+S_0^n| >\floor k |A+A| > (k-1) |A+A|.$

Since $S_0^n-S_0^n \subset \Z_{-n}^{n}$, it follows that
$S_0^n-S_0^n \subset (S-S)_{-n}^{n} \subset (S-S)_{-n}^{-n+\ceil j 
m-1}$, where $j= (2n+1)/m$ and $\ceil j$ is the least integer
greater than or equal to $j$.  Arguing as before, 
$|(S-S)_{-n}^{-n+\ceil j m-1}| = 
\ceil j |A-A|$.  Hence, $|S_0^n-S_0^n|< \ceil j |A-A|
< (j+1) |A-A|$.

It follows that $$\frac{ |S_0^n+S_0^n|}{|S_0^n-S_0^n|} >
\frac{(k-1)|A+A|}{(j+1)|A-A|} = \frac{2n-3m+3}{(2n+m+1)r}.$$ 
The right side is greater than or equal to 1 if
and only if $$n \ge \dfrac{(3+r)m+r-3}{2(1-r)}.$$
Since $r<1$, a sufficient condition is that $n\ge 2m/{(1-r)}$.  
\ProofStop


==> four.tex <==
\hyperdef\chapteRiv{ChapterSection}{chapteRiv}{}
\Chapter A Holonomic Hypergeometric Term\\
Is Piecewise Proper


The theory of holonomic systems was developed by 
Bernstien~\hyperref\Berone{\bibref[Ber1]} and applied to the
the theory of hypergeometric identities by
Zeilberger~\hyperref\Zeilninety{\bibref[Zeil90]}.
In~\hyperref\WZninetytwo{\bibref[WZ92]}
Wilf and Zeilberger
developed a proof theory
for multisums
that applies
only to {\sl proper} \hgt s.
Wilf and Zeilberger conjectured \bibref[WZ92%
] that a \hgt\ is holonomic  if and only if it is proper. 
We consider the discrete case of their conjecture and
interpret it to
mean roughly that a \hgt\  on $\Z^k$ is holonomic if and only if it is
{\sl piecewise proper}.
We use only elementary facts about holonomic functions that can be
found in~\hyperref\Zeilninety{\bibref[Zeil90]}
and~\hyperref\Bjoone{\bibref[Bjo1]}.

\Definition[def:pwp]  \hyperdef\defpwp{Definition}{pwp}{} 
A \hgt\  $f$ on $\Z^k$ over an
field $K$ is \defword{piecewise proper} if
there exist a polynomial $C\in K[\z]$ 
and a finite number of \hyperref\defBeighteen{polyhedral
regions} $\R_1,\ldots,\R_L$ such that $\Z^k$ is the union of the
$\R_{\ell}$ and a \hyperref\defBeleven{set of measure zero}, and for each region $\R_{\ell}$
there exist a vector $\vecgamma\in K^k$, constants
$m_1,\ldots,m_p,n_1,\ldots,n_q\in K$, vectors $\v_1,\ldots,
\v_p,\w_1,\ldots,\w_q\in\Z^k$, and integers
$r_1,\ldots,r_p,s_1,\ldots,s_q$ such that 
\Enumerate
\item for all $\z\in \R_{\ell}$,
$$f(\z)=
\gamma_1^{z_1}\cdots\gamma_k^{z_k}
C(\z)
\frac{\prod_{i=1}^p(m_i)_{\v_i\cdot
\z+r_i}}{\prod_{j=1}^q(n_j)_{\w_j\cdot\z+s_j}};$$ 
\item for all
$i$ and $j$ and $\z\in \R_{\ell}$, $\v_i\cdot\z+r_i$ and
$\w_j\cdot\z+s_j$ are positive; 
\item the Pochhammer symbols occurring
in the products are nonzero.
\EnumerateStop
\DefinitionStop

Our interpretation of Wilf and Zeilberger's conjecture is
Theorem~\hyperref\thmCtwelve{\ref[thm:C12]}.
\Theorem[thm:C12]  \hyperdef\thmCtwelve{Theorem}{C12}{}
A holonomic \hgt\  $f$ on $\Z^k$ over an
algebraically closed field $K$ is \hyperref\defpwp{piecewise proper}.
Conversely,
if
$f $ is \hyperref\defpwp{piecewise proper} then there exists a
holonomic function $g$ such that
$f=g$~\hyperref\defBeleven{a.e.}
\TheoremStop

The following example shows 
the necessity of introducing
sets of measure zero
and polyhedral regions
to the conjecture.
Let
$$f(z_1,z_2)=
\cases
(z_1-z_2+1)(z_1-z_2-1)&\text{if $z_1\ne z_2$}\\
g(z_1,z_2)&\text{if $z_1=z_2$,}
\endcases$$
where $g$ is an arbitrary holonomic function. Letting 
$$p(z_1,z_2)=(z_1-z_2+1)(z_1-z_2-1),$$
it's easily verified that
$$p^{\e_1}f=pf^{\e_1}\text{ and }p^{\e_2}f=pf^{\e_2}$$
regardless of the choice of $g$, so $f$ is a \hgt. Furthermore, using the fact that the characteristic function of a half-space is holonomic, it's easily seen that $f$ is holonomic:
$$f=\chi(z_1>z_2)p+\chi(z_1<z_2)p+\chi(z_1\ge z_2)\chi(z_1\le z_2)g,$$
where $\chi(\relation(z_1,z_2))$ is the characteristic function of $\{(z_1,z_2)\colon\relation(z_1,z_2)\}$. Each of the relations in the equation defines a half-plane, so each characteristic function is holonomic. Sums and products of holonomic functions are holonomic, so $f$ is holonomic. But $f$ is clearly not proper hypergeometric for arbitrary~$g$.

The function $f$ is, however, {\sl piecewise} proper. The set of measure zero is the line $z_1=z_2$, and the polyhedral regions are the half-spaces $z_1>z_2$ and $z_1<z_2$.


The `conversely'
part of  Theorem~\hyperref\thmCtwelve{\ref[thm:C12]} follows by the arguments of~\hyperref\Zeilninety{\bibref[Zeil90]}.
Thus to prove the conjecture, we need only prove
the first part, which  is the content of Theorem~\hyperref\thmCeleven{\ref[thm:C11]}.

\smallskip

\Statement[thm:C11] 
\noindent{\bf Theorem~\hyperref\thmCeleven{\ref[thm:C11]}} \ 
A holonomic \hgt\  $f$ on $\Z^k$ over an
algebraically closed field $K$ is \hyperref\defpwp{piecewise proper}:
there exist a polynomial $C\in K[\z]$ (as
in Theorem~\hyperref\thmCnine{\ref[thm:C9]}) and a finite number of \hyperref\defBeighteen{polyhedral
regions} $\R_1,\ldots,\R_L$ such that $\Z^k$ is the union of the
$\R_{\ell}$ and a \hyperref\defBeleven{set of measure zero}, and for each region $\R_{\ell}$
there exist a vector $\vecgamma\in K^k$, constants
$m_1,\ldots,m_p,n_1,\ldots,n_q\in K$, vectors $\v_1,\ldots,
\v_p,\w_1,\ldots,\w_q\in\Z^k$, and integers
$r_1,\ldots,r_p,s_1,\ldots,s_q$ such that 
\Enumerate
\item for all $\z\in \R_{\ell}$,
$$f(\z)=
\gamma_1^{z_1}\cdots\gamma_k^{z_k}
C(\z)
\frac{\prod_{i=1}^p(m_i)_{\v_i\cdot
\z+r_i}}{\prod_{j=1}^q(n_j)_{\w_j\cdot\z+s_j}};$$ 
\item for all
$i$ and $j$ and $\z\in \R_{\ell}$, $\v_i\cdot\z+r_i$ and
$\w_j\cdot\z+s_j$ are positive; 
\item the Pochhammer symbols occurring
in the products are nonzero.
\EnumerateStop
\StatementStop

Theorem~\hyperref\thmCeleven{\ref[thm:C11]} 
and
Theorem~\hyperref\thmCtwelve{\ref[thm:C12]}
apply to \hgt s on polyhedral regions
other than $\Z^k$ via Lemma~\hyperref\lemBtwentyoneb{\ref[lem:B21b]}.
We define a function $f$ on a 
polyhedral region $\R\subset \Z^k$
to be holonomic if the function
$g$ on $\Z^k$  is holonomic,
where
$$g(\z)=
\cases
f(\z)&\text{if $\z \in \R$}\\
0&\text{otherwise.}
\endcases$$


\smallskip

\hyperdef\chapteRivSECi{ChapterSection}{chapteRivSECi}{}
\Section Proof of Theorem~\ref[thm:C11]

We require the following lemmas.

\Lemma[lem:C1]  \hyperdef\lemCone{Lemma}{C1}{} If $f$ is holonomic and \hyperref\defBeleven{nondegenerate} then there exists a finite set $V\subset\Z^k$ such that $f(\z)\ne0$ implies $f(\z+\v)\ne0$ for some $\v\in V$.
\LemmaStop

Let $E_i$ be the shift
operator for $z_i$. Thus, $\vec E^{\v}f(\z)=E_1^{v_1}\cdots
E_k^{v_k}f(\z)=f(\z+\v)$.

\Proof
Since $f$ is holonomic, by
Lemma~4.1 of~\hyperref\Zeilninety{\bibref[Zeil90]} or~1.5 of~\hyperref\WZninetytwo{\bibref[WZ92]}, for each
$i\in\{1,\ldots,k\}$ there exists a nonzero operator $L_i(z_i,\vec E)$
that annihilates~$f$; $L_i(z_i,\vec E)=\sum_{\v\in V_i}c_{i,
\v}(z_i)\vec E^{\v}$ for some finite set $V_i\subset\Z^k$ and nonzero
univariate polynomials $c_{i,\v}\in K[z]$. The point is that the
operator~$L_i$ is free of all the variables $z_1,\ldots,z_k$ except
$z_i$. Since $L_if=0$ implies $\vec E^{\v}L_if=0$, we may assume
that $\vec0\in V_i$.

Let $b_i=c_{i,\vec0}$. Thus $b_i$ is nonzero and
$$b_i(z_i)f(\z)=-\sum_{\v\in V_i\atop\v\ne\vec0}c_{i,
\v}(z_i)f(\z+\v).$$
Hence $b_i(z_i)f(\z)\ne0$ implies $f(\z+\v)\ne0$ for some
$\v\in V_i$. Letting $\bar V=V_1\cup\cdots\cup V_k$ and $S=\{
\z\colon b_i(z_i)=0\text{ for }1\le i\le k\}$, it follows that if
$f(\z)\ne0$ and $\z\notin S$, then $f(\z+\v)\ne0$ for
some $\v\in\bar V$. Of course, the set $S$ is finite since each of
the $b_i$ has a finite number of roots. Since $f$ is nondegenerate,
there exists $\z_0\in\Z^k$ such that $f(\z_0)\ne0$ and $
\z_0\notin S$. Finally, let $V=\bar V\cup\{\z_0-\z\colon
\z\in S\}$.
\ProofStop

\Lemma[lem:C3]  \hyperdef\lemCthree{Lemma}{C3}{} If $f$ is holonomic on $\Z^k$ and $f$ is a \hyperref\defBtwo{\zd}, then $f=0$~\hyperref\defBeleven{a.e.}
\LemmaStop

\Proof We prove by induction on the dimension $k$ and the total degree $d$ of $p$ that if $f$ is holonomic on $\Z^k$ and $pf=0$~a.e. then $f=0$~a.e. The statement is clearly true if either $k=1$ or $d=1$ since in either case $p$ is simple: by Lemma~\hyperref\lemBtwelve{\ref[lem:B12]}, $p(\z)\ne0$ except on a set of measure zero, so $f=0$~a.e.

We assume that the lemma is true if either the dimension is less than $k$ or the degree is less than $d$ and prove that it is true if the dimension is $k$ and the degree is $d$. Suppose, to the contrary, there exists a polynomial $p\in K[\z]$ of degree $d$ and a holonomic function $f$ on $\Z^k$ such that $pf=0$ but $f$ is nondegenerate. By Lemma~\hyperref\lemfour{\ref[lem:four]}, there exists a finite set $V$ such that $f(\z)\ne0$ implies $f(\z+\v)\ne0$ for some $\v\in V$. Let $\vec x=(x_1,\ldots,x_k)$ where the $x_i$ are indeterminates. Let $g=\sum_{\v\in V}ff^{\v}\vec x^{\v}$. If $f(\z)\ne0$, then $g(\z)\ne0$, so $g$ is nondegenerate. Since $V$ is finite, $ff^{\v}=0$~a.e.\ for each $\v\in V$ implies $g=0$~a.e. Thus for at least one $\v\in V$, $ff^{\v}$ is nondegenerate. If $p\ne p^{\v}$, then $q=p-p^{\v}$ is of lower degree and $qff^{\v}=f^{\v}(pf)-f(pf)^{\v}=0$~a.e. But $ff^{\v}$ is holonomic, contradicting the assumption that the statement is true if the degree is less than $d$ and the dimension is $k$.

If $p=p^{\v}$ we reduce the dimension. If $h$ is holonomic on
$\Z^k$, 
and $M$ is an invertible $k\times k$ integer matrix,
then $g(\z)=h(M\z)$
is
also holonomic. Thus, by a change of variable we may assume that $p=p^{\e_k}$, and hence $p$
is free of $z_k$.

Let $x$ and $y$ be indeterminates,
and let $K[[x,y]]$ be the ring of formal power series in
$x$ and $y$.
Define the function $F\colon \Z^{k-1} \to K[[x,y]]$ by
$$F(z_1,\ldots,z_{k-1})=\sum_{z_k\ge0}f(z_1,\ldots,z_k)x^{z_k}
+\sum_{z_k<0}f(z_1,\ldots,z_k)y^{-z_k}.$$
By Proposition~3.4 of~\hyperref\Zeilninety{\bibref[Zeil90]}, $F$ is holonomic in
$z_1,\ldots,z_{k-1}$. But $pF=0$, and therefore $F=0$~a.e.\ by the assumption
that the statement is true for dimension $k-1$ and degree~$d$. The
function
$F$ is constructed so that 
the formal power series
$F(z_1,\ldots,z_{k-1})=0$ only if
$f(z_1,\ldots,z_k)=0$ for all $z_k\in\Z$.
Using the fact that 
$F=0$~a.e.\ in $\Z^{k-1}$,
it is easily seen then that 
$f=0$~a.e. in $\Z^k$, contrary to assumption.
\ProofStop

\Corollary[cor:C4]  \hyperdef\corCfour{Corollary}{C4}{} A holonomic \hgt\ is \hyperref\defBthirteena{honest}.
\CorollaryStop

\Proof By Lemma~\hyperref\lemBthree{\ref[lem:B3]} there exist $\bar A_{\v}$ and $\bar
B_{\v}$ such that $\bar A_{\v}f=\bar B_{\v}f^{\v}$. Let
$\bar A_{\v}=pA_{\v}$ and $\bar B_{\v}=pB_{\v}$ where
$p$, $A_{\v}$, and $B_{\v}$ are polynomials and $A_{\v}$
and $B_{\v}$ are relatively prime. Then $p(A_{\v}f-B_{
\v}f^{\v})=0$. But $g=A_{\v}f-B_{\v}f^{\v}$ is
holonomic and a \zd, so by Lemma~\hyperref\lemCthree{\ref[lem:C3]}, $g=0$~a.e.
Hence, $A_{\v}f=B_{\v}f^{\v}$~a.e.
\ProofStop

\Lemma[lem:C5]  \hyperdef\lemCfive{Lemma}{C5}{} Let $f$ be a \hgt\  on $\Z^k$ that is not a \hyperref\defBtwo{\zd}, and let $R_{
\v}$ be the \hyperref\defBfour{term ratio} of $f$ in the direction $\v$. Let
$V\subset\Z^k$ be a finite set and let $c_{\v}\in K[\z]$ be
given for each $\v\in V$. If $\sum_{\v\in V}c_{\v}f^{
\v}=0$~\hyperref\defBeleven{a.e.}, then $\sum_{\v\in V}c_{\v}R_{\v}=0$.
If $f$ is also holonomic, then the converse is true.
\LemmaStop

\Proof Since $f$ is a \hgt, by Lemma~\hyperref\lemBthree{\ref[lem:B3]} there exist polynomials $A_{\v}$ and $B_{\v}$ for each $\v\in\Z^k$ such that $A_{\v}f=B_{\v}f^{\v}$. Since $\sum_{\v\in V}c_{\v}f^{\v}=0$~a.e., $(\prod_{\w\in V}B_{\w})\sum_{\v\in V}c_{\v}f^{\v}=0$~a.e., hence $\sum_{\v\in V}c_{\v}(\prod_{\w\in V\setminus\{\v\}}B_{\w})B_{\v}f^{\v}=0$~a.e., hence 
$$\left(\sum_{\v\in V}c_{\v}\left(\prod_{\w\in V\setminus\{\v\}}B_{\w}\right)A_{\v}\right)f=0 \text{\ a.e.\ .}$$
Since $f$ is not a \zd, 
$$\sum_{\v\in V}c_{\v}\left(\prod_{\w\in V\setminus\{\v\}}B_{\w}\right)A_{\v}=0.$$ 
Dividing by $\prod_{\w\in V}B_{\w}$ it follows that $\sum_{\v\in V}c_{\v}A_{\v}/B_{\v}=0$. By Lemma~\hyperref\lemBsix{\ref[lem:B6]}, $R_{\v}=A_{\v}/B_{\v}$.
Hence $\sum_{\v\in V}c_{\v}R_{\v}=0$. 

Conversely, assuming $f$ is holonomic,
if $\sum_{\v\in V}c_{\v}R_{\v}=0$,
then multiplying by
$\left(\prod_{\w\in V}B_{\w}\right)f$,
it follows that
$\sum_{\v\in V}c_{\v}\left(\prod_{\w\in V\setminus\{\v\}}B_{\w}\right)A_{\v}f=0$. 
Hence,
$$\sum_{\v\in V}c_{\v}\left(\prod_{\w\in V\setminus\{\v\}}B_{\w}\right)B_{\v}f^{\v}=0,$$ 
and hence,
$$\left(\prod_{\w\in V}B_{\w}\right)\sum_{\v\in V}c_{\v}f^{\v}=0.$$ 
Since $f$ is holonomic, 
$\sum_{\v\in V}c_{\v}f^{\v}$
is holonomic.
But $\sum_{\v\in V}c_{\v}f^{\v}$ is a \zd ,
 so by Lemma~\hyperref\lemCthree{\ref[lem:C3]},
$\sum_{\v\in V}c_{\v}f^{\v}=0$~a.e.
\ProofStop

\Lemma[lem:C6]  \hyperdef\lemCsix{Lemma}{C6}{} Let $V\subset\Z^2$ be finite and let $A_{\v}$ and $B_{\v}\in K[z_1,z_2]$ be products of nonzero \hyperref\defAtwo{simple} polynomials for each $\v\in V$. Let $R\in K(z_1,z_2)$ be a rational function such that
$$\sum_{\v\in V}\frac{A_{\v}}{B_{\v}}R^{\v}=0.$$
Then the denominator of $R$ is a product of \hyperref\defAtwo{simple} polynomials.
\LemmaStop

\Proof Let $R=P/Q$, where $P$ and $Q$ are relatively prime. Let $d$ be
an irreducible divisor of $Q$. We will show that $d$ is simple. Suppose
the contrary. Then the dimension of $\rgal d$ is less than~$1$ by the
corollary of Lemma~\hyperref\lemfour{\ref[lem:four]}, that is, the dimension is~$0$. Thus
$d\ne d^{\w}$ for any nonzero $\w\in\Z^2$. By a corollary of
Lemma~\hyperref\lemzero{\ref[lem:zero]}, $d\ne cd^{\w}$ for any nonzero $
\w\in\Z^2$ and $c\in K$. Thus $d^{\w}$ divides $Q$ for only finitely
many $\w\in\Z^2$. Let $\w_0$ be the leftmost of the lowest of
the $\w$ such that $d^{\w}\mid Q$. In other words,
$\w_0=(x_0,y_0)$ where
$$y_0=\min\{y\in\Z\colon d^{(x,y)}\mid Q\text{ for some }x\in\Z\}$$
and 
$$x_0=\min\{x\in\Z\colon d^{(x,y_0)}\mid Q\}.$$
Similarly, let $\v_0$ be the leftmost of the lowest vectors in $V$.

Multiplying the equation
$$\sum_{\v\in V}\frac{A_{\v}}{B_{\v}}R^{\v}=0$$
by $\prod_{\u\in V}B_{\u}Q^{\u}$, we have
$$\sum_{\v\in V}A_{\v}P^{\v}\prod_{\u\in V\setminus\{\v\}}B_{\u}Q^{\u}=0.\tag{*}$$
Since $d^{\w_0}\mid Q$, it follows that 
$d^{\v_0+\w_0}\mid Q^{\v_0}$. Since $Q^{\v_0}$ appears
in every term of the sum except the term for $\v=\v_0$, it
follows that $d^{\v_0+\w_0}\mid A_{\v_0}P^{
\v_0}\prod_{\u\in V\setminus\{\v_0\}}B_{\u}Q^{\u}$.
Furthermore, since $A_{\v}$ and $B_{\v}$ are simple and $d$ is
not and $Q^{\v_0}$ and $P^{\v_0}$ are relatively prime, it
follows that $d^{\v_0+\w_0}\mid Q^{\u}$ for some $
\u\in V\setminus\{\v_0\}$. Thus $d^{\w_0+\v_0-\u}\mid
Q$ for some $\u\in V\setminus\{\v_0\}$, contradicting the
definition of $\w_0$.
\ProofStop

\Lemma[lem:C7]  \hyperdef\lemCseven{Lemma}{C7}{} Let $f$ be a \hyperref\defBeleven{nondegenerate} 
holonomic \hgt\ on $\Z^k$ and let $R_{\v}$ be the \hyperref\defBfour{term ratio} of $f$ 
in the direction $\v$ for each $\v\in\Z^k$. Let
$$R_{\w}(\z)=\frac{C(\z+\w)}{C(\z)}\frac{D(\z)}{D(\z+\w)}\prod_{\v\in V}\gp j0{\v\cdot\w}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)}$$
as in Theorem~\hyperref\thmBnine{\ref[thm:B9]}. Then $D$ is a product of \hyperref\defAtwo{simple} polynomials.
\LemmaStop

\Proof By Lemma~4.1 of~\hyperref\Zeilninety{\bibref[Zeil90]}, for each $i,j\in\{1,\ldots,k\}$
there exists a nonzero operator
$$L(E_i,E_j,z_1,\ldots,z_{j-1},z_{j+1},\ldots,z_k)$$
such that $L$ is free of all $E$s except $E_i$ and $E_j$, and $L$ is
free of $z_j$. Thus
$$\sum_{\w\in W}\alpha_{\w}f^{\w}=0,$$
where $W$ is a finite subset of the subspace of $\Z^k$ generated by
$\e_i$ and $\e_j$. Furthermore, since each polynomial $\alpha_{\w}$ is free of
$z_j$,
each $\alpha_{\w}$ is simple
over the field
$K_{i,j}=K(\{z_1,\ldots,z_k\}\setminus\{z_i,z_j\})$.

By Lemma~\hyperref\lemCfive{\ref[lem:C5]}, $\sum_{\v\in W}\alpha_{\w}R_{\w}=0$. Hence 
$$\sum_{\w\in W}\alpha_{\w}\frac{C^{\w}}C\frac D{D^{\w}}\frac{\bar
A_{\w}}{\bar B_{\w}}=0,$$
where
$$\frac{\bar A_{\w}}{\bar B_{\w}}=\prod_{\v\in V}\gp
j0{\v\cdot\w}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)}.$$
Hence
$$\sum_{\w\in W}\alpha_{\w}\frac{\bar A_{\w}}{\bar
B_{\w}}\frac{C^{\w}}{D^{\w}}=0,$$
and hence
$$\sum_{\w\in W}\frac{A_{\w}}{B_{\w}}\frac{C^{\w}}{D^{\w}}=0,$$
where $A_{\w}$ and $B_{\w}$ are the products of polynomials
that are simple over $K_{i,j}$.


It follows by Lemma~\hyperref\lemCsix{\ref[lem:C6]} that any irreducible divisor $d$ of
$D$ is simple over $K_{i,j}$.
Hence,
by Corollary~\hyperref\coroldlemmafour{\ref[cor:oldlemmafour]},
the dimension of
$\rgal(d,(z_i,z_j),K_{i,j})$ is at least~$1$.
Let $\Q_{i,j}$ be the subspace of $\Q^k$ generated by $\e_i$ and
$\e_j$.
Since
$\rgal(d,(z_i,z_j),K_{i,j})$ is 
isomorphic to
$\Q_{i,j} \cap \rgal d$,
the dimension of $\Q_{i,j}\cap\rgal d$ is at
least~$1$.

We show that $d$ is simple in $z_1,\ldots,z_k$, that is, the dimension
of $\rgal d$ is at least $k-1$. Let $\Q_i$ be the subspace of $\Q^k$
generated by $\e_i$. If $\Q_i\subset\rgal d$ for each
$i\in\{1,\ldots,k\}$, then $\rgal d=\Q^k$. Hence the dimension is $k$.
Otherwise, say for concreteness that $\Q_1\not\subset\rgal d$. Then for
each $j\in\{2,\ldots,k\}$ there exists $\u_j\in\Q_{1,j}\cap\ \rgal d$ such that
$\u_j\notin\Q_1$. It's easily seen that $\u_2,\ldots,\u_k$ are
independent, so the dimension of $\rgal d$ is at least $k-1$.
\ProofStop



\Lemma[lem:C8]  \hyperdef\lemCeight{Lemma}{C8}{} Let $f$ be a holonomic \hgt\ on $\Z^k$ and let $R_{\v}$ be the \hyperref\defBfour{term ratio} of $f$ in the direction $\v$ for each $\v\in\Z^k$. There exist a polynomial $C$, a finite set $V\subset\Z^k$, and univariate polynomials $a_{\v}$ and $b_{\v}$ for each $\v\in V$ such that
$$R_{\w}(\z)=\frac{C(\z+\w)}{C(\z)}\prod_{\v\in V}\gp j0{\v\cdot\w}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)}.$$
\LemmaStop

\Proof By Theorem~\hyperref\thmBnine{\ref[thm:B9]} we can express $R_{\w}(\z)$ as
$$R_{\w}(\z)=\frac{C(\z+\w)}{C(\z)}\frac{D(\z)}{D(\z+\w)}\prod_{\v\in V}\gp j0{\v\cdot\w}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)},$$
and by Lemma~\hyperref\lemCseven{\ref[lem:C7]} the irreducible divisors of $D$ are simple. The result follows by noting that
$$\frac{d(\v\cdot\z)}{d(\v\cdot(\z+\w))}=\gp j0{\v\cdot\w}\frac{d(\v\cdot\z+j)}{d(\v\cdot\z+1+j)},$$
and hence the divisors of $D$ can be absorbed into the `factorial part'.
\ProofStop


\Theorem[thm:C9]  \hyperdef\thmCnine{Theorem}{C9}{} Let $f$ be a holonomic \hgt\ on $\Z^k$. Then there exist a polynomial $C$, a finite set $V\subset\Z^k$, and univariate polynomials $a_{\v}$ and $b_{\v}\in K[z]$ for each $\v\in V$ (as in Lemma~\hyperref\lemCeight{\ref[lem:C8]}) and a finite number of \hyperref\defBeighteen{polyhedral regions} $\R_1,\ldots,\R_m$ such that
\Enumerate
\item $\Z^k$ is the union of the $\R_i$ and a \hyperref\defBeleven{set of measure zero};
\item for each $i\in\{1,\ldots,m\}$ there exists $\z_0\in \R_i$ such that $C(\z_0)\ne0$, and for all $\z\in \R_i$,
$$f(\z)=f(\z_0)\frac{C(\z)}{C(\z_0)}\prod_{\v\in V}\gp j{\z_0\cdot\v}{\z\cdot\v}\frac{a_{\v}(j)}{b_{\v}(j)}.$$
\item  all the terms $a_{\v}(j)$ and $b_{\v}(j)$
occurring in the product are nonzero.
\EnumerateStop
\TheoremStop

Theorem~\hyperref\thmCnine{\ref[thm:C9]} applies to \hgt s on polyhedral regions
other than $\Z^k$ via Lemma~\hyperref\lemBtwentyoneb{\ref[lem:B21b]}.



\Proof The theorem is an immediate consequence of Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]} and Lem\-ma~\hyperref\lemCeight{\ref[lem:C8]}.
\ProofStop

\Corollary[cor:C10]  \hyperdef\corCten{Corollary}{C10}{} Let $f$ be an holonomic \hgt\ on $\Z^k$. Then there
exist a polynomials $C\in K[\z]$  and  a finite number of
\hyperref\defBeighteen{polyhedral regions}
$\R_1,\ldots,\R_L$ such that
$\Z^k$ is the union of the $\R_\ell$ and a \hyperref\defBeleven{set of measure zero} and for each
region $\R_\ell$
there exist a finite set $V\subset\Z^k$ and
univariate polynomials $a_{\v}$ and $b_{\v}\in K[z]$ and an
integer $n_{\v}$ for each $\v\in V$ such that, for all $
\z\in \R_\ell$,
\Enumerate
\item $\ds{f(\z)=C(\z)\prod_{\v\in V}\prod_{j=1}^{\v\cdot\z+n_{\v}}\frac{a_{\v}(j)}{b_{\v}(j)}}$,
\item for all $\v\in V$, $\v\cdot\z+n_{\v}$ is a positive integer, and
\item for all $\v\in V$ and $j$, $1\le j\le\v\cdot\z+n_{\v}$, $a_{\v}(j)\ne0$ and $b_{\v}(j)\ne0$.
\EnumerateStop
\CorollaryStop

Corollary~\hyperref\corCten{\ref[cor:C10]} applies to \hgt s on polyhedral regions
other than $\Z^k$ via Lemma~\hyperref\lemBtwentyoneb{\ref[lem:B21b]}.


\Proof This corollary is an immediate consequence of  Corollary~\hyperref\corBthirty{\ref[cor:B30]} and Lemma~\hyperref\lemCeight{\ref[lem:C8]}.
\ProofStop

\Theorem[thm:C11]  \hyperdef\thmCeleven{Theorem}{C11}{} A holonomic \hgt\  $f$ on $\Z^k$ over an
algebraically closed field $K$ is \hyperref\defpwp{piecewise proper}:
there exist a polynomial $C\in K[\z]$ (as
in Theorem~\hyperref\thmCnine{\ref[thm:C9]}) and a finite number of \hyperref\defBeighteen{polyhedral
regions} $\R_1,\ldots,\R_L$ such that $\Z^k$ is the union of the
$\R_{\ell}$ and a \hyperref\defBeleven{set of measure zero}, and for each region $\R_{\ell}$
there exist a vector $\vecgamma\in K^k$, constants
$m_1,\ldots,m_p,n_1,\ldots,n_q\in K$, vectors $\v_1,\ldots,
\v_p,\w_1,\ldots,\w_q\in\Z^k$, and integers
$r_1,\ldots,r_p,s_1,\ldots,s_q$ such that 
\Enumerate
\item for all $\z\in \R_{\ell}$,
$$f(\z)=
\gamma_1^{z_1}\cdots\gamma_k^{z_k}
C(\z)
\frac{\prod_{i=1}^p(m_i)_{\v_i\cdot
\z+r_i}}{\prod_{j=1}^q(n_j)_{\w_j\cdot\z+s_j}};$$ 
\item for all
$i$ and $j$ and $\z\in \R_{\ell}$, $\v_i\cdot\z+r_i$ and
$\w_j\cdot\z+s_j$ are positive; 
\item the Pochhammer symbols occurring
in the products are nonzero.
\EnumerateStop
\TheoremStop

Theorem~\hyperref\thmCeleven{\ref[thm:C11]} applies to \hgt s on polyhedral regions
other than $\Z^k$ via Lemma~\hyperref\lemBtwentyoneb{\ref[lem:B21b]}.


\Proof This theorem is an immediate consequence of  Corollary~\hyperref\corCten{\ref[cor:C10]} and Lemma~\hyperref\lemBtwentythree{\ref[lem:B23]}.
\ProofStop




==> one.tex <==
\hyperdef\chapteRi{ChapterSection}{chapteRi}{}
\Chapter Introduction



\hyperdef\chapteRiSECi{ChapterSection}{chapteRiSECi}{}
\Section Hypergeometric terms and term ratios

Throughout this work $K$ denotes a field of characteristic zero. We write $K[z]$ for the ring
of polynomials in one variable over $K$, and $K[
\z]=K[z_1,\ldots,z_k]$ for the ring of polynomials in $k$ variables over
$K$. Similarly, we write $K(z)$ for field of rational functions in one
variable over $K$, and $K(\z)=K(z_1,\ldots,z_k)$ for the field of
rational functions in $k$ variables over $K$. 

\Definition[def:shift]  \hyperdef\defshift{Definition}{shift}{} For any function $f\colon\Z^k\to K$ and any
vector $\v \in\Z^k$, the function $f^{\v}\colon\Z^k\to K$ is defined by
$$f^{\v}(\z)=f(\z+
\v)=f(z_{1}+v_{1},\ldots,z_{k}+v_{k}).$$
Similarly, for any rational function $R\in K(\z)$ and any
vector $\v \in\Q^k$, the rational
function $R^{\v} \in K(\z)$ is defined by
$$R^{\v}(\z)=R(\z+
\v)=R(z_{1}+v_{1},\ldots,z_{k}+v_{k}).$$
\DefinitionStop

\Definition[def:B1]  \hyperdef\defBone{Definition}{B1}{} A \defword{hypergeometric term} on $\Z^k$
over a field $K$ is
a function $f\colon\Z^k\to K$ such that for $i\in\{1,\ldots,k\}$ there
exist nonzero polynomials $A_1,\ldots,A_k$ and $B_1,\ldots,B_k\in K[\z]$
such that
$$A_if=B_if^{\e_i}.$$
Of course, this last equation is equivalent to $A_i(\z)f(
\z)=B_i(\z)f(\z+\e_i)$ for all $\z\in\Z^k$.
\DefinitionStop

For any \hgt\ $f$ on $\Z^k$ and any $\v\in\Z^k$, a rational
function $R_{\v}\in K(\z)$ is a \defword{term ratio in the
direction} $\v$ if
$$R_{\v}=\frac{A_{\v}}{B_{\v}}$$
for some nonzero polynomials $A_{\v},B_{\v}\in K[\v]$ such that
$A_{\v}f=B_{\v}f^{\v}$.

\Definition[def:B2]  \hyperdef\defBtwo{Definition}{B2}{} A function $f$ on $\Z^k$ is a \defword{zero
divisor} if there exists a nonzero polynomial $p\in K[\z]$ such that
$pf=0$.
\DefinitionStop

We show in Lemma~\hyperref\lemBsix{\ref[lem:B6]} that if a \hgt\ $f$ is not a \zd, then
for each $\v\in\Z^k$ there exists a unique term ratio $R_{\v}$
in the direction $\v$. Furthermore, we show in Lemma~\hyperref\lemBseven{\ref[lem:B7]}
that if $f$ is not a \zd\ then the term ratios satisfy
$$R_{\v}R_{\w}^{\v}=R_{\w}R_{\v}^{\w}$$
for all $\w,\v\in\Z^k$. In particular, letting $R_i=R_{
\e_i}$, we have $R_iR_j^{\e_i}=R_jR_i^{\e_j}$ for all
$i,j\in\{1,\ldots,k\}$
(cf.\ \hyperref\WZninety{\bibref[WZ90]}).
 This is the relation for the term ratios of a
\hgt. The first step in understanding the structure of a \hgt\ is to
understand the structure of rational solutions of this system of
equations.

\hyperdef\chapteRiSECii{ChapterSection}{chapteRiSECii}{}
\Section The rational solutions of $R_iR_j^{\e_i}=R_jR_i^{\e_j}$

It will be useful to define
$$\gp iabA_i=\cases
\prod_{i=a}^{b-1}A_i&\text{if $b>a$}\\
1&\text{if $b=a$}\\
1\big/\prod_{i=b}^{a-1}A_i&\text{if $a>b$.}
\endcases$$
The usefulness of the notation stems in part from the fact that
$$\gp iabA_i\,\gp ibcA_i=\gp iacA_i$$
and
$$\gp iabA_i=\gp iba\frac1{A_i},$$
which is easily verified.

In Chapter~2, we prove Theorem~\hyperref\thmfifteena{\ref[thm:15a]} \hyperref\oresato{\OreSato} which completely describes
the rational solutions of the system of equations
$$R_iR_j^{\e_i}=R_jR_i^{\e_j} \quad i,j \in \{1,\ldots,k\}.$$ 

\smallskip
\Statement[thm:15a] 
\noindent{\bf{}Theorem~\hyperref\thmfifteena{\ref[thm:15a]}} \ 
Let $R_i\in K(\z)$, $i=1,\ldots,k$, be rational functions such that
$$R_iR_j^{\e_i}=R_jR_i^{\e_j}
\text{\quad 
for all $i,j\in\{1,\ldots,k\}$.
}
$$
Then there exist polynomials $C$ and
$D\in K[\z]$, a finite set $V\subset\Z^k$, and univariate
polynomials $a_{\v}$ and $b_{\v}\in K[z]$ for each $\v\in
V$ such that for all $i\in\{1,\ldots,k\}$,
$$R_i(\z)=\frac{C(\z+\e_i)}{C(\z)}\frac{D(
\z)}{D(\z+\e_i)}\prod_{\v\in V}\gp j0{\v_i}\frac{a_{
\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)}.$$
\StatementStop

The proof of Theorem~\hyperref\thmfifteena{\ref[thm:15a]} is quite involved.
The first part of the proof is showing that the solution can be
expressed in the form
$$R_i=\frac{C^{\e_i}}{C}\frac{D}{D^{\e_i}}\frac{A_i}{B_i},$$
$i=1,\ldots,k$, where $C$ and $D$ are polynomials (not depending on
$i$) and $A_i$ and $B_i$ are products of {\sl simple} polynomials. 
A simple
polynomial is a composition of a univariate polynomial and a linear
polynomial $\v\cdot\z$. The one-dimensional case is
trivial. By using Gosper's Lemma~\hyperref\Gospseventyeight{\bibref[Gosp78]}, we reduce the
two-dimensional case to the following lemma. Let $A_1$, $A_2$, $B_1$,
and $B_2\in K[z_1,z_2]$. If $A_1$ and $B_1^{n\e_1}$ are
relatively prime for all $n\in\Z$, $A_2$ and $B_2$ are relatively
prime, and $R_1=A_1/B_1$ and $R_2=A_2/B_2$ satisfy $R_1R_2^{
\e_1}=R_2R_1^{\e_2}$, then the irreducible divisors of $A_1$, $B_1$,
$A_2$, and $B_2$ are simple. An interesting feature of the proof of the
lemma is the association of a lattice path with an irreducible divisor
of $A_1$, $B_1$, $A_2$, or $B_2$. 
(
A \defword{lattice path in $\Z^k$} is a sequence 
$\{T_i\}_{i\ge1}$ in $\Z^k$ such that
$T_i-T_{i-1}\in \{\pm \e_1,\ldots,\pm\e_k\}$ for all
$i>1$.
)
The primeness conditions of the lemma
impose restrictions of the shape of the lattice path, from which we
deduce that the path is unbounded. From the unboundedness of the
path, it follows that $d$ satisfies a nontrivial relation $d=d^{\v}$,
and from this it follows that $d$ is simple.
We derive the higher-dimensional cases from the two-dimensional case
with the aid of the notions of the {\sl rational Galois space} of a rational
function and the {\sl fixed factor} of a rational function for a subspace. 

The second part of the 
proof of Theorem~\hyperref\thmfifteena{\ref[thm:15a]} is deriving the formula for $R_i$
given the simplicity of the divisors of the $A_i$ and $B_i$.
A crucial step is observing that the
multiplicative components of the $R_i$ determined by rational Galois space
still satisfy the relation for the term ratios: if $s$ is a subspace of
$\Q^k$ and $R_{i,s}=\fix_sR_i$, then
$$R_{i,s}R_{j,s}^{\e_i}=R_{j,s}R_{i,s}^{\e_j}.$$

\hyperdef\chapteRiSECiii{ChapterSection}{chapteRiSECiii}{}
\Section The multiplicative structure of a hypergeometric term

Define a \defword{hyperplane} in $\Z^k$ to be a set of the form $\{
\z\colon\v\cdot\z=n\}$, where $n\in\Z$ and $\v$ is some vector in $\Z^k$.
Define a \defword{half-space} in $\Z^k$ to be a set of the form $\{
\z\colon\v\cdot\z>n\}$, where $n\in\Z$ and $\v$ is some vector in
$\Z^k$.
A \defword{set of measure zero} in $\Z^k$ is a set that can be covered
by a finite number of hyperplanes. Two functions $f,g\colon\Z^k\to K$
are \defword{equal almost everywhere} (written $f=g$~a.e.) if there
exists a set $S$ of measure zero such that $f(\z)=g(\z)$ for
all $\z\in\Z^k\setminus S$.
A region $\R\subset\Z^k$ is \defword{polyhedral} if 
$R=\Z^k$ or $R$ is the
intersection of a finite number of half-spaces. 


It is easily seen
(Lemma~\hyperref\lemBthirteen{\ref[lem:B13]}) that a function $f$ is a \hgt\ on $\Z^k$ if and only if,
for all $\v \in \Z^k$, there exist nonzero polynomials $A_{\v} $ and
$B_{\v}\in K[\z]$ such that
$A_{\v}f=B_{\v}f^{\v}$~a.e.
A \hgt\ $f$ on $\Z^k$ is \defword{honest}
if for all $\v\in\Z^k$ there exist {\sl relatively prime}
polynomials $A_{\v}$ and $B_{\v}\in K[\z]$ such that
$A_{\v}f=B_{\v}f^{\v}$~a.e.

The main results of Chapter 3  are Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]} and its
corollary for
algebraically closed fields, Corollary~\hyperref\corBthirtyone{\ref[cor:B31]}.

\smallskip

\Statement[thm:B29] 
\noindent{\bf Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]}} \ Let $f$ be an \hyperref\defBthirteena{honest} \hgt\ on
$\Z^k$. There exist relatively prime polynomials $C$ and $D\in K[\z]$, a finite
set $V\subset\Z^k$, univariate polynomials $a_{\v},b_{\v}\in
K[z]$, for each $\v\in V$, and a finite number of \hyperref\defBeighteen{polyhedral regions}
$\R_1,\ldots,\R_m$ such that
\Enumerate
\item $\Z^k$ is the disjoint union of the $\R_i$ and a \hyperref\defBeleven{set of measure
zero};
\item for each $i\in\{1,\ldots,m\}$ there exists $\z_0\in \R_i$ such
that $C(\z_0)\ne0$, and for all $\z\in \R_i$ for which $D(
\z)\ne0$,
$$f(\z)=f(\z_0)\frac{C(\z)}{C(\z_0)}\frac{D(
\z_0)}{D(\z)}\prod_{\v\in V}\gp j{\z_0\cdot\v}{
\z\cdot\v}\frac{a_{\v}(j)}{b_{\v}(j)}.$$
\item  all the terms $a_{\v}(j)$ and $b_{\v}(j)$
occurring in the product are nonzero.
\EnumerateStop
\StatementStop

The \hgt s that occur in practice can be expressed as products of
Pochhammer symbols, so the question arises: Is this true in general?
Corollary~\hyperref\corBthirtyone{\ref[cor:B31]} show that if the field $K$ is algebraically
closed and the \hgt\ is honest, then the answer is yes, at least
piecewise.

\smallskip

\Statement[cor:B31] 
\noindent{\bf Corollary~\hyperref\corBthirtyone{\ref[cor:B31]}} \ Let $f$ be an \hyperref\defBthirteena{honest}
\hgt\ on $\Z^k$ over a field $K$ that is algebraically closed. Then there exist
relatively prime polynomials $C$ and $D\in K[\z]$ and a finite number of \hyperref\defBeighteen{polyhedral regions}
$\R_1,\ldots,\R_L$ such that $\Z^k$ is the union of the $\R_{\ell}$ and a
\hyperref\defBeleven{set of measure zero}, and for each region $\R_{\ell}$ there exist a
vector $\vecgamma\in K^k$, constants $m_1,\ldots,m_p,n_1,\ldots,n_q\in
K$, vectors $\v_1,\ldots,\v_p,\w_1,\ldots,\w_q\in\Z^k$,
and integers $r_1,\ldots,r_p,s_1,\ldots,s_q$ such that
\Enumerate
\item for all $\z\in \R_{\ell}$ such that $D(\z)\ne0$,
$$f(\z)=
\gamma_{1}^{z_{1}}\cdots \gamma_{k}^{z_{k}}
\frac{C(\z)}{D(\z)}
\frac{\prod_{i=1}^p(m_i)_{\v_i\cdot
\z+r_i}}{\prod_{j=1}^q(n_j)_{\w_j\cdot\z+s_j}};$$
\item for all $i$ and $j$ and all $\z\in \R_{\ell}$, $\v_i\cdot
\z+r_i$ and $\w_j\cdot\z+s_j$ are positive;
\item the Pochhammer symbols occurring
in the products are nonzero.
\EnumerateStop
\StatementStop

If we assume that everything in sight is nonzero,
then the expression for $f$ in Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]} follows by
induction from the expression for the term ratios in
Theorem~\hyperref\thmfifteena{\ref[thm:15a]}.
Unfortunately, zeros of $C$, $D$ and the $a_{\v}$ and $b_{\v}$
are
deadly to the induction.
The polyhedral regions $\R_i$
arise as regions for which the nonzero points of these polynomials
have a certain connectedness property.


\hyperdef\chapteRiSECiv{ChapterSection}{chapteRiSECiv}{}
\Section A holonomic \hgt\ is piecewise proper

We prove the following result which settles the discrete part of
Wilf and Zeilberger's conjecture that a \hgt\  is holonomic if and only
if
it is proper.

\smallskip

\Statement[thm:C11] 
\noindent{\bf Theorem~\hyperref\thmCeleven{\ref[thm:C11]}} \ A holonomic \hgt\  $f$ on $\Z^k$ over an
algebraically closed field $K$ is \hyperref\defpwp{piecewise proper};
there exist a polynomial $C\in K[\z]$ 
and a finite number of \hyperref\defBeighteen{polyhedral
regions} $\R_1,\ldots,\R_L$ such that $\Z^k$ is the union of the
$\R_{\ell}$ and a \hyperref\defBeleven{set of measure zero}, and for each region $\R_{\ell}$
there exist a vector $\vecgamma\in K^k$, constants
$m_1,\ldots,m_p,n_1,\ldots,n_q\in K$, vectors $\v_1,\ldots,
\v_p,\w_1,\ldots,\w_q\in\Z^k$, and integers
$r_1,\ldots,r_p,s_1,\ldots,s_q$ such that
\Enumerate
\item for all $\z\in \R_{\ell}$,
$$f(\z)=
\gamma_{1}^{z_{1}}\cdots \gamma_{k}^{z_{k}}
C(\z)
\frac{\prod_{i=1}^p(m_i)_{\v_i\cdot
\z+r_i}}{\prod_{j=1}^q(n_j)_{\w_j\cdot\z+s_j}};$$
\item for all
$i$ and $j$ and all $\z\in \R_{\ell}$, $\v_i\cdot\z+r_i$ and
$\w_j\cdot\z+s_j$ are positive;
\item the Pochhammer symbols occurring in the products are nonzero.
\EnumerateStop
\StatementStop

Theorem~\hyperref\thmCeleven{\ref[thm:C11]} applies to \hgt s on polyhedral regions other than $\Z^k$ via Lemma~\hyperref\lemBtwentyoneb{\ref[lem:B21b]}.




The proof of Theorem~\hyperref\thmCeleven{\ref[thm:C11]} uses the results of Chapter 3 and
only elementary facts about holonomic functions
that can be found in \hyperref\Zeilninety{\bibref[Zeil90]} and \hyperref\Bjoone{\bibref[Bjo1]}.

\hyperdef\chapteRiSECv{ChapterSection}{chapteRiSECv}{}
\Section A Solution to a Problem of Cameron
On Sum-free Complete Sets

For any subsets $A$ and $B$ of an additive group $G$, define
$A+B=\{a+b:a \in A \text{ and } b \in B \}$ and $-A= \{-a:a
\in A \}$.  A subset $S$ of $G$ is said to be sum-free,
complete, and symmetric respectively if $S+S \subset S^\c$,
$S+S \supset S^\c$, and $S=-S$.  Hence, $S$ is sum-free and
complete if and only if $S+S=S^\c$.


Cameron observed that for any sufficiently small modulus $m$,
every sum-free complete set in $\Z/m\Z$ is also symmetric.
In fact, Calkin found that $m=36$ is the smallest modulus  for which
there is a sum-free complete set that is not
symmetric \hyperref\CamPortrait{\bibref[CamPortrait]}.  Cameron asked if there exists
such a set for all sufficiently large moduli \hyperref\CamPortrait{\bibref[CamPortrait]}.
We answer Cameron's question by showing
there exists such a set for all moduli greater than or
equal to $890626$.

We also show that every sum-free complete set in $\Z/m\Z$ that
is not symmetric can be used to construct a counterexample
to a conjecture of J.H.~Conway.
 Conway conjectured that for any finite set
$S$ of integers, $|S+S| \le |S-S|$.
Conway's conjecture
was disproved by Marica \hyperref\Marica{\bibref[Marica]}.  Later Stein showed
how to make the ratio ${|S+S|}/{|S-S|}$ arbitrarily large
\hyperref\Stein{\bibref[Stein]}.  We show that if $S$ is sum-free and complete
modulo $m$ but not symmetric, then $|S+S|>|S-S|$; hence, $S$
is a counterexample to a modular version of Conway's conjecture.
Further, we show that if $S' \subset \Z$ is a certain set
derived from $S$, then $|S'+S'| > |S'-S'|$; hence, $S'$ is a
counterexample to Conway's conjecture proper.

The history of sum-free sets begins with Schur who
showed that the positive integers can not be partitioned
into finitely many sum-free sets \hyperref\Schur{\bibref[Schur]}.  Sum-free sets
have been used to find lower bounds for Ramsey numbers
(see pp.~28, 128, 264 in~\hyperref\Wallis{\bibref[Wallis]}).  Cameron describes  some
applications of sum-free sets and poses several problems
\hyperref\CamGraph{\bibref[CamGraph]},\hyperref\CamStructure{\bibref[CamStructure]},\hyperref\CamPortrait{\bibref[CamPortrait]}.  George Andrews
observed that sum-free complete
sets play a role in partition identities (personal communication).
For example, the
set $\{1,4\} \in \Z/5\Z$, which arises in the Rogers-Ramanujan
Identities (p.~109 in~\hyperref\Andseventysix{\bibref[And76]}), is sum-free, complete,
and symmetric.  Calkin showed that the number of sum-free
sets contained within the first $n$ integers is $o(2^{n(1/2
+\epsilon)})$ for every $\epsilon > 0$ \hyperref\Calkin{\bibref[Calkin]}.





==> three.tex <==

\hyperdef\chapteRiii{ChapterSection}{chapteRiii}{}
\Chapter The Multiplicative Structure\\ 
of a Hypergeometric Term

The main results of  this chapter are Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]} and its
corollary for
algebraically closed fields, Corollary~\hyperref\corBthirtyone{\ref[cor:B31]}.

\smallskip

\Statement[thm:B29] 
\noindent{\bf Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]}} \ Let $f$ be an \hyperref\defBthirteena{honest} \hgt\ on
$\Z^k$. There exist relatively prime polynomials $C$ and $D\in K[\z]$, a finite
set $V\subset\Z^k$, univariate polynomials $a_{\v},b_{\v}\in
K[z]$, $\v\in V$ (all of which can be determined as in
Theorem~\hyperref\thmBnine{\ref[thm:B9]}), and a finite number of \hyperref\defBeighteen{polyhedral regions}
$\R_1,\ldots,\R_m$ such that
\Enumerate
\item $\Z^k$ is the disjoint union of the $\R_i$ and a \hyperref\defBeleven{set of measure
zero};
\item for each $i\in\{1,\ldots,m\}$ there exists $\z_0\in \R_i$ such
that $C(\z_0)\ne0$, and for all $\z\in \R_i$ for which $D(
\z)\ne0$,
$$f(\z)=f(\z_0)\frac{C(\z)}{C(\z_0)}\frac{D(
\z_0)}{D(\z)}\prod_{\v\in V}\gp j{\z_0\cdot\v}{
\z\cdot\v}\frac{a_{\v}(j)}{b_{\v}(j)}.$$
\item  all the terms $a_{\v}(j)$ and $b_{\v}(j)$
occurring in the product are nonzero.
\EnumerateStop
\StatementStop

The \hgt s that occur in practice can be expressed as products of
Pochhammer symbols, so the question arises: Is this true in general?
Corollary~\hyperref\corBthirtyone{\ref[cor:B31]} show that if the field $K$ is algebraically
closed and the \hgt\ is honest, then the answer is yes, at least
piecewise. \hyperdef\Honestpw{Remark}{honesthtgpiecewise}{}

\smallskip

\Statement[cor:B31] 
\noindent{\bf Corollary~\hyperref\corBthirtyone{\ref[cor:B31]}} \ Let $f$ be an \hyperref\defBthirteena{honest}
\hgt\ on $\Z^k$ over a field $K$ that is algebraically closed. Then there exist
relatively prime polynomials $C$ and $D\in K[\z]$ (as in
Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]}) and a finite number of \hyperref\defBeighteen{polyhedral regions}
$\R_1,\ldots,\R_L$ such that $\Z^k$ is the union of the $\R_{\ell}$ and a
\hyperref\defBeleven{set of measure zero}, and for each region $\R_{\ell}$ there exist a
vector $\vecgamma\in K^k$, constants $m_1,\ldots,m_p,n_1,\ldots,n_q\in
K$, vectors $\v_1,\ldots,\v_p,\w_1,\ldots,\w_q\in\Z^k$,
and integers $r_1,\ldots,r_p,s_1,\ldots,s_q$ such that
\Enumerate
\item for all $\z\in \R_{\ell}$ such that $D(\z)\ne0$,
$$f(\z)=
\gamma_{1}^{z_{1}}\cdots \gamma_{k}^{z_{k}}
\frac{C(\z)}{D(\z)}
\frac{\prod_{i=1}^p(m_i)_{\v_i\cdot
\z+r_i}}{\prod_{j=1}^q(n_j)_{\w_j\cdot\z+s_j}};$$
\item for all $i$ and $j$ and $\z\in \R_{\ell}$, $\v_i\cdot
\z+r_i$ and $\w_j\cdot\z+s_j$ are positive;
\item the Pochhammer symbols occurring
in the products are nonzero.
\EnumerateStop
\StatementStop


\hyperdef\chapteRiiiSECi{ChapterSection}{chapteRiiiSECi}{}
\Section Hypergeometric terms and term ratios

\Definition[def:B1]  \hyperdef\defBone{Definition}{B1}{} A \defword{hypergeometric term} on $\Z^k$ over a
field $K$ is a function $f\colon\Z^k\to K$ such that for
$i\in\{1,\ldots,k\}$ there exist
nonzero polynomials $A_1,\ldots,A_k$ and $B_1,\ldots,B_k\in K[\z]$
such that
$$A_i(\z)f(\z)=B_i(\z)f(\z+\e_i)$$
for every $\z\in\Z^k$.
\DefinitionStop

Unfortunately, the definition of a \hgt\ includes some pathological
functions. For example, if $f$ is any function $f\colon\Z^k\to K$ that
is supported by the set of zeros of a nonzero polynomial $p$, then
$p(\z)f(\z)=0$ for all $\z$, that is, $pf=0$.  It follows
that $p^{\e_i}f^{\e_i}=0$ for $i\in\{1,\ldots,k\}$, and hence
$pf=p^{\e_i}f^{\e_i}$ for $i\in\{1,\ldots,k\}$. By
Definition~\hyperref\defBone{\ref[def:B1]}, $f(\z)$ is a \hgt. Such a \hgt\ is called
a \defword{zero divisor}.


\Definition[def:B2]  \hyperdef\defBtwo{Definition}{B2}{} A function $f$ on $\Z^k$ is a \defword{zero
divisor} if there exists a nonzero polynomial $p\in K[\z]$ such
that $pf=0$.
\DefinitionStop

\Lemma[lem:B3]  \hyperdef\lemBthree{Lemma}{B3}{} If $f$ is a \hgt\ on $\Z^k$, then for all $
\v\in\Z^k$, there exist nonzero polynomials $A_{\v}$ and $B_{
\v}\in K[\z]$ such
$$A_{\v}f=B_{\v}f^{\v}.$$
\LemmaStop

\Proof
We prove the lemma by induction. By the definition (\hyperref\defBone{\ref[def:B1]}) of
\hgt, the statement of the lemma is true if $\v=\e_i$,
$i\in\{1,\ldots,k\}$, and clearly the statement is true if $\v=\vec0$.
We complete the induction by showing that
if the statement is true for $\v=\u$ and $
\v=\w$, then it is true for $\v=\u+\w$ and $\v=
\u-\w$. Taking $A_{\u+\w}=A_{\u}A_{\w}^{\u}$ and
$B_{\u+\w}=B_{\u}B_{\w}^{\u}$, we have $A_{
\u+\w}f=A_{\u}A_{\w}^{\u}f=A_{\w}^{\u}B_{
\v}f^{\u}=B_{\u}(A_{\w}f)^{\u}=B_{\u}(B_{
\w}f^{\w})^{\u}=B_{\u}B_{\w}^{\u}f^{\w+
\u}=B_{\u+\w}f^{\u+\w}$. 
Similarly, taking $A_{\u-\w}=A_{\u}B_{\w}^{
\u-\w}$ and $B_{\u-\w}=B_{\u}A_{\w}^{\u-
\w}$, $A_{\u-\w}f=A_{\u}B_{\w}^{\u-\v}f=B_{
\w}^{\u-\w}B_{\u}f^{\u}=B_{\u}(B_{\w}f^{
\w})^{\u-\w}=B_{\u}(A_{\w}f)^{\u-\w}=B_{
\u}A_{\w}^{\u-\w}f^{\u-\w}=B_{\u-\w}f^{
\u-\w}$.
\ProofStop




\Definition[def:B4]  \hyperdef\defBfour{Definition}{B4}{} For any \hgt\ $f$ on $\Z^k$ and any $
\v\in\Z^k$, a rational function $R_{\v}\in K(\z)$ is a
\defword{term ratio in the direction} $\v$ if
$$R_{\v}=\frac{A_{\v}}{B_{\v}}$$
for some nonzero polynomials $A_{\v},B_{\v}\in K[\z]$ such
that $A_{\v}f=B_{\v}f^{\v}$.
\DefinitionStop

Thus, by Lemma~\hyperref\lemBthree{\ref[lem:B3]}, a term ratio exists for each $\v$. Of
course, we use the term {\sl term ratio} because
$$\frac{f^{\v}(\z)}{f(\z)}=\frac{A_{\v}(
\z)}{B_{\v}(\z)}=R_{\v}(\z)$$
for all $\z$ such that $f(\z)\ne0$ and $B_{\v}(
\z)\ne0$. The following lemma shows that if $f$ is not a \zd\ then the
term ratio for $f$ in the direction $\v$ is unique.

\Lemma[lem:B6]  \hyperdef\lemBsix{Lemma}{B6}{} If a \hgt\ $f$ on $\Z^k$ is not a \hyperref\defBtwo{\zd}, then for each
$\v\in\Z^k$ there is a unique \hyperref\defBfour{term ratio in the direction $\v$.}
\LemmaStop

\Proof Let $R_{\v}$ and $\bar R_{\v}$ be two term ratios for
$f$ in the direction $\v$. Then
$$R_{\v}=\frac{A_{\v}}{B_{\v}}\text{ and }\bar R_{
\v}=\frac{\bar A_{\v}}{\bar B_{\v}}$$
where $A_{\v}f=B_{\v}f^{\v}$ and $\bar A_{\v}f=\bar
B_{\v}f^{\v}$. From the last two equations it follows that
$(\bar B_{\v}A_{\v}-B_{\v}\bar A_{\v})f=0$. Since $f$
is not a \zd, this implies that $\bar B_{\v}A_{\v}-B_{
\v}\bar A_{\v}=0$, which implies that $R_{\v}=\bar R_{\v}$.
\ProofStop

\Lemma[lem:B7]  \hyperdef\lemBseven{Lemma}{B7}{} Let $f$ be a \hgt\ on $\Z^k$ that is not a \hyperref\defBtwo{\zd}\ and let $R_{
\v}$ be the \hyperref\defBfour{term ratio} for $f$ in the direction $\v$ (which is
unique by Lemma~\hyperref\lemBsix{\ref[lem:B6]}). Then
$$R_{\v+\w}=R_{\v}R_{\w}^{\v}=R_{\w}R_{
\v}^{\w}$$
for all $\v,\w\in\Z^k$.
\LemmaStop

\Proof For each $\v\in\Z^k$, let $A_{\v}$ and $B_{\v}$ by
polynomials such that $A_{\v}f=B_{\v}f^{\v}$ as in
Lemma~\hyperref\lemBthree{\ref[lem:B3]}. Then $A_{\v}A_{\w}^{\v}f=A_{
\w}B_{\v}f^{\v}=B_{\v}(A_{\w}f)^{\v}=B_{
\v}(B_{\w}f^{\v})=B_{\v}B_{\w}^{\v}f^{\v+
\w}$. Thus, we have
$$A_{\v+\w}f
=B_{\v+\w}f^{\v+\w}$$
and
$$A_{\v}A_{\w}^{\v}f
=B_{\v}B_{\w}^{\v}f^{\v+\w}.$$
It follows from these equations that
$$(A_{\v+\w}B_{\v}B_{\w}^{\v}-B_{\v+
\w}A_{\v}A_{\w}^{\v})f=0.$$
Since $f$ is not a \zd, this implies that $A_{\v+\w}B_{
\v}B_{\w}^{\v}-B_{\v+\w}A_{\v}A_{\w}^{
\v}=0$, from which it follows that $R_{\v+\w}=R_{\v}R_{
\w}^{\v}$. By symmetry, $R_{\v+\w}=R_{\w}R_{
\v}^{\w}$.
\ProofStop

\Proposition[prop:B8]  \hyperdef\propBeight{Proposition}{B8}{}
If a \hgt\ $f$ on $\Z^k$ is a \hyperref\defBtwo{\zd}, then 
for each 
$\v\in \Z^k$
there exist nonzero 
$A_{\v}$
and $B_{\v}\in K[\z]$  such that $A_{\v}=B_{
\v}f^{\v}$ and $R_{\v}=A_{\v}/B_{
\v}$ satisfies $R_{\v}R_{\w}^{\v}=R_{\w}R_{\v}^{
\w}$ for $\v,\w\in\Z^k$.
\PropositionStop

\Proof Since $pf=0$ for some polynomial $p\in K[\z]$, $p^{
\v}f^{\v}=0$ for all $\v\in\Z^k$. Thus, $pf=p^{\v}f^{\v}$
for all $\v\in\Z^k$. Taking $A_{\v}=p$ and $B_{\v}=p^{
\v}$, it's easily verified that $R_{\v}R_{\w}^{\v}=R_{
\w}R_{\v}^{\w}$ for all $\v,\w\in\Z^k$.
\ProofStop

\Theorem[thm:B9]  \hyperdef\thmBnine{Theorem}{B9}{} Let $f$ be a \hgt\ on $\Z^k$ that is not a \hyperref\defBtwo{\zd}.
For all $\w\in\Z^k$, let $R_{\w}$ be the \hyperref\defBfour{term ratio} of $f$ in
the direction $\w$. Then there exist polynomials $C$ and $D$ in
$K[\z]$, a finite set $V\subset\Z^k$, and univariate polynomials
$a_{\v}$ and $b_{\v}\in K[z]$ for each $\v\in V$ such
that
$$R_{\w}(\z)=\frac{C(\z+\w)}{C(\z)}\frac{D(
\z)}{D(\z+\w)}\prod_{\v\in V}\gp j0{\v\cdot
\w}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot
\v+j)}\text{for all $w\in \Z^k$.}$$
\TheoremStop

\Proof By Lemma~\hyperref\lemBseven{\ref[lem:B7]}, $R_{\v + \w}=R_{\v}R_{
\w}^{\v}$ for all $\v,\w\in\Z^k$. The result follows
immediately by Corollary~\hyperref\corsixteen{\ref[cor:16]}.
\ProofStop

\hyperdef\chapteRiiiSECii{ChapterSection}{chapteRiiiSECii}{}
\Section Sets of measure zero

When considering sequences of one variable, it is useful to
identify sequences that are equal except at a finite number of points.
Thus, we identify sequences that are equal `almost everywhere' and
think of finite sets as `sets of measure zero'. When considering
sequences of several variables, that is, functions from $\Z^k$ to a
field $K$, it is useful to consider the `sets of measure zero' to
be not finite sets, but sets that can be covered by a finite number of
hyperplanes. Thus, in dimension~2, a `set of measure zero' can be covered
by a finite number of lines, and in three dimensions a `set of measure
zero' can be covered by a finite number of planes.

\Definition[def:B10]  \hyperdef\defBten{Definition}{B10}{} Define a \defword{hyperplane} in $\Z^k$ to be a
set of the form $\{\z\colon\v\cdot\z=n\}$, where $n\in\Z$ and $\v$
is some vector in $\Z^k$. Define a \defword{half-space} in $\Z^k$ to be
a set of the form $\{\z\colon\v\cdot\z>n\}$, where $n\in\Z$ and $\v$
is some vector in $\Z^k$. The boundary of the half-space $\{
\z\colon\v\cdot\z>n\}$ is the hyperplane $\{\z\colon
\v\cdot\z=n\}$. Since $\{\z\colon\v\cdot\z<n\}=\{
\z\colon-\v\cdot\z>-n\}$ is a half-space with boundary $\{
\z\colon\v\cdot\z=n\}$, each hyperplane is the boundary of two
half-spaces, and $\Z^k$ is the disjoint union of these two half-spaces
and the boundary.
\DefinitionStop

\Definition[def:B11]  \hyperdef\defBeleven{Definition}{B11}{} A \defword{set of measure zero} in $\Z^k$ is a set
that can be covered by a finite number of \hyperref\defBten{hyperplanes}. Two functions
$f,g\colon\Z^k\to K$ are \defword{equal almost everywhere} (written
$f=g$~a.e.) if there exists a set $S$ of measure zero such that $f(
\z)=g(\z)$ for all $\z\in\Z^k\setminus S$. We say $f$ is
\defword{degenerate} if $f=0$~a.e.\ and $f$ is \defword{nondegenerate}
if it is not degenerate.
\DefinitionStop

Clearly, a finite union of sets of measure zero is a set of measure zero.
Note that although we have defined a set of measure zero, we have not
defined a measure. We use the phrase only because it is familiar and
suggestive.

\Lemma[lem:B12]  \hyperdef\lemBtwelve{Lemma}{B12}{} A nonzero \hyperref\defAtwo{simple} polynomial $p\in K[\z]$ is nonzero
except on a \hyperref\defBeleven{set of measure zero}.
\LemmaStop

\Proof Let $p(\z)=\bar p(\z\cdot\v)$, where $\v\in\Z^k$
and $\bar p\in K[z]$ is a univariate polynomial. Let $n_1,\ldots,n_m$
be the integer roots of $\bar p$. If $p(\z_0)=0$, then $
\z_0\cdot\v$ is a root of $\bar p$, and hence $\z_0\cdot
\v=n_i$ for some $i$. Hence $\z_0$ lies in one of the $m$
hyperplanes $\{\z\colon\z\cdot\v=n_j\}$, $j=1,\ldots,m$,
the union of which is a set of measure zero.
\ProofStop

\Lemma[lem:B13]  \hyperdef\lemBthirteen{Lemma}{B13}{} A function $f$ is a \hgt\ on $\Z^k$ if and only if, for all $
\v \in \Z^k$, there exist nonzero polynomials $A_{\v} $ and $B_{
\v}\in K[\z]$ such that
$A_{\v}f=B_{\v}f^{\v}\text{ \hyperref\defBeleven{a.e.}}$
\LemmaStop

\Proof If $f$ is a \hgt, 
$A_{\v}f=B_{\v}f^{\v}\text{ a.e.}$
automatically. Conversely, if
$A_{\v}f=B_{\v}f^{\v}\text{ a.e.}$,
then
$p_{\v}A_{\v}f=p_{\v}B_{\v}f^{\v}$,
where $p_{\v}\in K[\z]$ is a product of nonzero linear polynomials.
Hence $f$ is a \hgt.
\ProofStop

\Definition[def:B13a]  \hyperdef\defBthirteena{Definition}{B13a}{} A \hgt\ $f$ on $\Z^k$ is \defword{honest} if for
all $\v\in\Z^k$ there exist relatively prime polynomials $A_{
\v}$ and $B_{\v}\in K[\z]$ such that $A_{\v}f=B_{
\v}f^{\v}$~\hyperref\defBeleven{a.e.}
\DefinitionStop

\hyperdef\chapteRiiiSECiii{ChapterSection}{chapteRiiiSECiii}{}
\Section Boxes

\Definition[def:box]  \hyperdef\defbox{Definition}{box}{} A \defword{$k$-dimensional box of size $n$} is a set of the
form $\{\z \in \Z^k\colon c_i\le z_i\le c_i+n\}$, where
$c_1,\ldots,c_k\in\Z$. (A 
$k$-dimensional box is the set of integer points in
a 
$k$-dimensional hypercube.)
\DefinitionStop

\Lemma[lem:B15]  \hyperdef\lemBfifteen{Lemma}{B15}{} If a $k$-variable polynomial $p\in K[\z]$ is $0$ on
a \hyperref\defbox{$k$-dimensional box of size $n$,} where $n$ is the total degree of
$p$, then $p$ is identically $0$.
\LemmaStop

\Proof The lemma is clearly true if the degree of $p$ is $0$. We assume
that it is true if the degree of $p$ is $n-1$, and show that it is true
if the degree of $p$ is $n$. Suppose $p$ is of degree $n$ and is zero
on a
$k$-dimensional box of size $n$. For $i\in\{1,\ldots,k\}$, $p-p^{
\e_i}$ is $0$ on a
$k$-dimensional box of size $n-1$. By Lemma~\hyperref\lemzero{\ref[lem:zero]} $p-p^{
\e_i}$ is of degree at most $n-1$, so $p-p^{\e_i}$ is identically
$0$ by assumption. Thus, $p=p^{\e_i}$ for all $i\in\{1,\ldots,k\}$.
By Lemma~\hyperref\lemthree{\ref[lem:three]} $p$ is free of $z_i$ for $i\in\{1,\ldots,k\}$.
Thus $p$ is constant, and hence $p$ is identically zero.
\ProofStop

\Lemma[lem:B16]  \hyperdef\lemBsixteen{Lemma}{B16}{} If a \hgt\  on $\Z^k$ 
is not a \hyperref\defBtwo{\zd}, then for any sequence $
\w_1,\ldots,\w_n$ of vectors in $\Z^k$ the \hgt\ $f^{
\w_1}f^{\w_2}\cdots f^{\w_n}$ is not a \hyperref\defBtwo{\zd}.
\LemmaStop

\Proof By Lemma~\hyperref\lemBthree{\ref[lem:B3]}, for any $\v\in\Z^k$ there exist
nonzero polynomials $A_{\v},B_{\v}\in K[\z]$ such that
$A_{\v}f=B_{\v}f^{\v}$. If $f^{\w_1}f^{\w_2}\cdots
f^{\w_n}$ is a \zd, then for some nonzero polynomial $p$, $pf^{
\w_1}f^{\w_2}\cdots f^{\w_n}=0$.
Hence, $$pB_{\w_1}\cdots B_{\w_n}f^{\w_1}f^{\w_2}\cdots
f^{\w_n}=0,$$ hence, $pA_{\w_1}\cdots A_{\w_n}f^n=0$,
hence, $pA_{\w_1}\cdots A_{\w_n}f=0$, and hence, $f$ is a \zd,
contrary to assumption.
\ProofStop

\Lemma[lem:B17]  \hyperdef\lemBseventeen{Lemma}{B17}{} If $f$ is a \hgt\ on $\Z^k$, then either $f$ is a
\hyperref\defBtwo{\zd}\ or $f$ is nonzero on arbitrarily large
$k$-dimensional \hyperref\defbox{boxes}.
\LemmaStop

\Proof Let $V$ be the $k$-dimensional box
$\{\z\in\Z^k\colon 0\le z_i\le n\}$,
and let $V=\{\v_1,\ldots,\v_m\}$. If $f$ is not a \zd, by
Lemma~\hyperref\lemBsixteen{\ref[lem:B16]} $g=f^{\v_1}\cdots f^{\v_m}$ is not a \zd,
hence for some $\w$ (infinitely many), $g(\w)\ne0$, and hence
$f(\w+\v_j)\ne0$ for $j\in\{1,\ldots,m\}$. Thus $f$ is nonzero
on the
$k$-dimensional box
$$\{\z+\w\colon 0\le z_i\le n,\ i=1,\ldots,k\},$$
which is of size $n$.
\ProofStop

\hyperdef\chapteRiiiSECiv{ChapterSection}{chapteRiiiSECiv}{}
\Section Polyhedral regions

\Definition[def:B18]  \hyperdef\defBeighteen{Definition}{B18}{} A region $\R\subset\Z^k$ is
\defword{polyhedral} if $R=\Z^k$ or $R$
is the intersection of a finite number
of \hyperref\defBten{half-spaces} of $\Z^k$. 
\DefinitionStop

\Lemma[lem:B19]  \hyperdef\lemBnineteen{Lemma}{B19}{} The characteristic function of a \hyperref\defBten{half-space} in $\Z^k$ is a \hgt;
in fact, for all $w\in \Z^k$, $f=f^{\w}$ \hyperref\defBeleven{a.e.}
\LemmaStop

\Proof Let the half-space be $\{\z\colon\v\cdot\z>n\}$ for
some $\v\in\Z^k$ and $n\in\Z$. Then $f(\z)=f(\z+\w)$ unless $
\z\cdot\v>n$ and $(\z+\w)\cdot\v\le n$, or
unless $\z\cdot\v\le n$ and $(\z+\w)\cdot\v> n$;
that is, $n<\z\cdot\v\le n-\v\cdot\w$ or $n-
\v\cdot\w<\z\cdot\v\le n$. In either case, the set of
exceptions is just the union of $|\v\cdot\w|$ hyperplanes. Thus
$f(\z)=f(\z+\w)$ a.e.
\ProofStop

\Lemma[lem:B20]  \hyperdef\lemBtwenty{Lemma}{B20}{} The characteristic function of a \hyperref\defBeighteen{polyhedral region} is a
\hgt.
\LemmaStop

\Proof By definition, the region is the intersection of a finite number
of half-spaces, so the characteristic function of the region is just
the product of the characteristic functions of the half-spaces, which
are all hypergeometric terms
by Lemma~\hyperref\lemBnineteen{\ref[lem:B19]}. Since the product of two \hgt s
is a \hgt, the characteristic function of the region is a \hgt.
\ProofStop

\Lemma[lem:B21]  \hyperdef\lemBtwentyone{Lemma}{B21}{} If $\R$ is a \hyperref\defBeighteen{polyhedral region} in $\Z^k$, then either
$\R$ contains arbitrarily large
$k$-dimensional \hyperref\defbox{boxes}, or $\R$ is a \hyperref\defBeleven{set of measure zero}.
\LemmaStop

Lemma~\hyperref\lemBtwentyone{\ref[lem:B21]} can be proved by elementary means, but we can't
resist this short proof based on a result from Chapter~4.

\Proof Let $f$ be the characteristic function of the region $\R$. By
Lemma~\hyperref\lemBtwenty{\ref[lem:B20]}, $f$ is a \hgt. The function $f$ is the product of
characteristic functions of half-spaces, so $f$ is holonomic. If $f$ is
a \zd, then by Lemma~\hyperref\lemCthree{\ref[lem:C3]} $f=0$~a.e., so $\R$ is a set of
measure $0$. If $f$ is not a \zd, then by Lemma~\hyperref\lemBseventeen{\ref[lem:B17]}, $f$ is
nonzero on arbitrarily large
$k$-dimensional boxes, and hence $\R$ contains arbitrarily large 
$k$-dimensional boxes.
\ProofStop

\Definition[def:B21a]  \hyperdef\defBtwentyonea{Definition}{B21a}{} Let $\R\subset\Z^k$ be a \hyperref\defBeighteen{polyhedral region}. A
\defword{hypergeometric term} on $\R$ over $K$ is a function $f\colon
\R\to K$ such that for $i\in\{1,\ldots,k\}$ there exist nonzero
polynomials $A_i,B_i\in K[\z]$ such that
$$A_i(\z)f(\z)=B_i(\z)f(\z+\e_i)$$ 
for all $\z$ such that $\z$ and $\z+\e_i$ are in $\R$.
\DefinitionStop

\Lemma[lem:B21b]  \hyperdef\lemBtwentyoneb{Lemma}{B21b}{} If $f$ is a \hgt\ on a \hyperref\defBeighteen{polyhedral region}
$\R\subset\Z^k$, then the function
$$g(\z)=\cases
f(\z)&\z\in \R\\
0&\z\notin \R\endcases$$
is a \hgt\ on $\Z^k$.
\LemmaStop

\Proof For $i\in\{1,\ldots,k\}$ there exist nonzero polynomials $A_i$
and $B_i$ such that
$$A_i(\z)f(\z)=B_i(\z)f^{\e_i}(\z)$$
for all $\z$ such that $\z\in \R$ and $\z+\e_i\in \R$.
Let $h$ be the characteristic function for $\R$. By
Lemma~\hyperref\lemBtwentyone{\ref[lem:B21]}, $h$ is a \hgt\ on $\Z^k$, so for
$i\in\{1,\ldots,k\}$ there exist nonzero polynomials $\bar A_i$ and
$\bar B_i$ such that
$$\bar A_i(\z)h(\z)=\bar B_i(\z)h(\z+\e_i)$$
for all $\z\in\Z^k$. By considering separately the cases
\Enumerate
\item $\z\in \R$, $\z+\e_i\in \R$,
\item $\z\in \R$, $\z+\e_i\notin \R$,
\item $\z\notin \R$, $\z+\e_i\in \R$, and
\item $\z\notin \R$, $\z+\e_i\notin \R$,
\EnumerateStop
it is easily seen that 
$$A_i\bar A_ig=B_i\bar B_ig^{\e_i}$$
for $i\in\{1,\ldots,k\}$.
\ProofStop



\hyperdef\chapteRiiiSECv{ChapterSection}{chapteRiiiSECv}{}
\Section Factorial hypergeometric terms

\Definition[def:B22]  \hyperdef\defBtwentytwo{Definition}{B22}{} A \hgt\ on $\Z^k$ is \defword{factorial} on a region
$\R\subset\Z^k$ if there exist a finite set $V\subset\Z^k$, univariate
polynomials $a_{\v}$ and $b_{\v}\in K[z]$ and an integer
$n_{\v}$ for each $\v\in V$ such that, for all $\z\in \R$,
\Enumerate
\item $\ds{f(\z)=\prod_{\v\in V}\prod_{j=1}^{\v\cdot
\z+n_{\v}}\frac{a_{\v}(j)}{b_{\v}(j)}}$,
\item for all $\v\in V$, $\v\cdot\z+n_{\v}$ is a
positive integer, and
\item for all $\v\in V$ and $j$, $1\le j\le\v\cdot
\z+n_{\v}$, $a_{\v}(j)\ne0$ and $b_{\v}(j)\ne0$.
\EnumerateStop
\DefinitionStop

Recall that $\vecgamma^{\z}=\gamma_1^{z_1}\cdots\gamma_k^{z_k}$ and
$(m)_r=m(m+1)\cdots(m+r-1)$.

\Lemma[lem:B23]  \hyperdef\lemBtwentythree{Lemma}{B23}{} If $f$ is a \hgt\ on $\Z^k$ over a field that is
algebraically closed and $f$ is \hyperref\defBtwentytwo{factorial} on a region $\R$, then there
exist a vector $\vecgamma\in K^k$, constants $m_1,\ldots,m_p$ and
$n_1,\ldots,n_q\in K$, vectors $\v_1,\ldots,\v_p$ and $
\w_1,\ldots,\w_q\in\Z^k$, and integers $r_1,\ldots,r_p$ and
$s_1,\ldots,s_q\in\Z$ such that, for all $\z\in \R$,
\Enumerate
\item $\ds{f(\z)=
\vecgamma^{\z}
\frac{\prod_{i=1}^p(m_i)_{\v_i\cdot
\z+r_i}}{\prod_{j=1}^q(n_j)_{\w_j\cdot\z+s_j}}}$;
\item $\v_i\cdot\z+r_i$ and $\w_j\cdot\z+s_j$ are
positive integers for each $i\in\{1,\ldots,p\}$ and $\{1,\ldots,q\}$;
\item all the terms appearing in the numerator and denominator are nonzero.
\EnumerateStop
\LemmaStop

\Proof Since $f$ is factorial on $\R$,
$$f(\z)=\prod_{\v\in V}\prod_{j=1}^{\v\cdot\z+n_{
\v}}\frac{a_{\v}(j)}{b_{\v}(j)}$$
for all $\z\in \R$ where $V$, $n_{\v}$, $a_{\v}$, and
$b_{\v}$ are as in Definition~\hyperref\defBtwentytwo{\ref[def:B22]}. Since a product of
functions of the form~(1) satisfying conditions~(2) and~(3) is of the
same form (and likewise for reciprocals), we need only prove the lemma
for
$$f(\z)=\prod_{j=1}^{\u\cdot\z+\ell}a(j).$$
Since $K$ is algebraically closed, $a(j)=\alpha(j-a_1)\cdots(j-a_t)$,
where $\alpha,a_i\in K$. By the same reasoning as before, we need only
prove the lemma for
$$\prod_{j=1}^{\u\cdot\z+\ell}\alpha$$
and
$$\prod_{j=1}^{\u\cdot\z+\ell}(j-a_1).$$
The first is $\alpha^{\u\cdot
\z+\ell}=\alpha^{\ell}\alpha^{u_1z_1+\cdots
u_kz_k}=(\alpha^{\ell})_1\boldsymbol\gamma^{\z}$, where
$\boldsymbol\gamma=(\alpha^{u_1},\ldots,\alpha^{u_k})$, and the second
is $(1-a_1)_{\u\cdot\z+\ell}$. We're given that $
\u\cdot\z+\ell$ is positive on $\R$ and $a(j)$ is nonzero for $1\le
j\le\u\cdot\z+\ell$, so conditions~(2) and~(3) follow.
\ProofStop

\Definition[def:B24]  \hyperdef\defBtwentyfour{Definition}{B24}{} A \hgt\ $f$ on $\Z^k$ is \defword{weakly factorial} on a
region $\R\subset\Z^k$ if there exist a finite set
$V\subset\Z^k$, univariate polynomials $a_{\v}$ and $b_{\v} \in
K[z]$ for each $\v\in V$, and $\z_0\in \R$ such that, for all
$\z\in \R$,
\Enumerate
\item $\ds{f(\z)=\prod_{\v\in V}\gp j{\z_0\cdot\v}{
\z\cdot\v}\frac{a_{\v}(j)}{b_{\v}(j)}}$, and
\item for all $\v\in V$ and all $j$ occurring in the product
$\ds{\gp j{\z_0\cdot\v}{\z\cdot\v}\frac{a_{
\v}(j)}{b_{\v}(j)}}$, $a_{\v}(j)\ne0$ and $b_{\v}(j)\ne0$.
\EnumerateStop
\DefinitionStop

An example of a \hgt\ on $\Z$ that is weakly factorial but 
not factorial is 
$$f(z_1)=\gp j0{z_1}(2j+1)=\cases
\ds{\prod_{j=0}^{z_1-1}(2j+1)},&z_1\ge0\\
\ds{\prod_{j=1}^{-z_1}\frac1{1-2j}},&z_1<0.
\endcases$$
Though $f$ is not factorial, the domain of $f$ can be split into two
regions, $\{z_1\ge0\}$ and $\{z_1<0\}$, such that it is factorial on
each region. The following lemma shows that this is true in general.


\Lemma[lem:B25]  \hyperdef\lemBtwentyfive{Lemma}{B25}{} If a \hgt\ is \hyperref\defBtwentyfour{weakly factorial} on a \hyperref\defBeighteen{polyhedral region}
$\R$, then there exist a finite number of \hyperref\defBeighteen{polyhedral regions}
$\R_1,\ldots,\R_m$ such that $\R=\R_1\cup\cdots\cup \R_m$ and $f$ is
\hyperref\defBtwentytwo{factorial} on each of the $\R_i$.
\LemmaStop

\Proof Since $f$ is weakly factorial on $\R$,
$$f(\z)=\prod_{\v\in V}\gp j{\v\cdot\z_0}{
\v\cdot\z}\frac{a_{\v}(j)}{b_{\v}(j)},$$
where $a_{\v},b_{\v},V$, and $\z_0$ are as in
Definition~\hyperref\defBtwentyfour{\ref[def:B24]}. Let $\Cal G$ be the set of functions $g\colon
V\to\{-1,1\}$. We show that $\R$ can be divided into at most $2^{|V|}$
regions $\{\R_g\colon g\in\Cal G\}$, such that for each $\v\in V$,
$g\in\Cal G$, and region $\R_g$, there exist $\w=\pm\v$,
$n=\pm\v\cdot\z_0$, univariate polynomials $a_{\v}$ and
$b_{\v}$ which are nonzero for $1\le j\le\w\cdot\v+n$, such
that
$$\gp j{\v\cdot\z_0}{\v\cdot\z}\frac{a_{
\v}(j)}{b_{\v}(j)}=\prod_{j=1}^{\w\cdot\z+n}\frac{a_{
\v}(j)}{b_{\v}(j)}.\tag{*}$$

We construct the region $\R_g$ so that for every $\v\in V$, the
sign of $\v\cdot(\z-\z_0)$ is constant over $\z\in
\R_g$. For each $\v\in V$ define the half-spaces
$${\Cal H}_{\v}(1)=\{\z\colon\v\cdot(\z-\z_0)\ge0\}$$
and
$${\Cal H}_{\v}(-1)=\{\z\colon\v\cdot(\z-\z_0)<0\}.$$
For each $g\in\Cal G$, the region $\R_g$ is defined by
$$\R_g=\R\cap\bigcap_{\v\in V}{\Cal H}_{\v}(g(\v)).$$
Clearly $\R=\bigcup_g\R_g$ and $\R_g$ is polyhedral. Note $|{\Cal
G}|=2^{|V|}$, so $|\{\R_g\colon g\in{\Cal G}\}|\le2^{|V|}$. By
definition, the sign of $\v\cdot(\z-\z_0)$ is constant on
${\Cal H}_{\v}(g(\v))$, so, for each $\v$, the sign of
$\v\cdot(\z-\z_0)$ is constant
for $\z \in \R_g$.

We need to show that for a given region (*) is true. Let a region
$\R_g$ and a vector $\v$ be given. If $\v\cdot\z-
\v\cdot\z_0=\v\cdot(\z-\z_0)$ is nonnegative on $\R_g$,
then
$$\gp j{\v\cdot\z_0}{\v\cdot\z}\frac{a_{
\v}(j)}{b_{\v}(j)}
=\prod_{j=\v\cdot\z_0}^{\v\cdot
\z-1}\frac{a_{\v}(j)}{b_{\v}(j)}
=\prod_{j=1}^{\v\cdot
\z-\v\cdot\z_0}\frac{a_{\v}(j+\v\cdot
\z_0-1)}{b_{\v}(j+\v\cdot\z_0-1)}
=\prod_{j=1}^{\w\cdot
\z +n_{\v}}\frac{\bar a_{\v}(j)}{\bar b_{\v}(j)}
,$$
where $\bar a_{\v}(j)=a_{\v}(j+\v\cdot\z_0-1)$, $\bar b_{
\v}(j)=b_{\v}(j+\v\cdot\z_0-1)$,
$\w=\v$, and
$n_{\v}=-\v\cdot\z_0$. 
If $\v\cdot\z-\v\cdot\z_0=
\v\cdot(\z-\z_0)$ is negative on $\R_g$,
$$\align
\gp j{\v\cdot\z_0}{\v\cdot\z}\frac{a_{
\v}(j)}{b_{\v}(j)}
&=\prod_{j=\v\cdot\z_0}^{\v\cdot\z-1}\frac{b_{
\v}(j)}{a_{\v}(j)}\\
&=\prod_{j=1-\v\cdot\z_0}^{-\v\cdot\z}\frac{b_{
\v}(-j)}{a_{\v}(-j)}\\
&=\prod_{j=1}^{\v\cdot\z_0-\v\cdot\z}\frac{b_{
\v}(-j-\v\cdot\z_0)}{a_{\v}(-j-\v\cdot\z)}\\
&=\prod_{j=1}^{\w\cdot\z+n_{\v}}\frac{\bar a_{
\v}(j)}{\bar b_{\v}(j)},
\endalign$$ 
where $\bar a_{\v}(j)=b_{\v}(-j-\v\cdot\z_0)$ and $\bar
b_{\v}=a_{\v}(-j-\v\cdot\z_0)$,
$\w=-\v$, and $n_{\v}= \v \cdot \z_0$.
\ProofStop

\hyperdef\chapteRiiiSECvi{ChapterSection}{chapteRiiiSECvi}{}
\Section Path connected regions

Recall that a lattice path in $\Z^k$ is a sequence 
$\{T_i\}_{i\ge1}$ in $\Z^k$ such that
$T_i-T_{i-1}\in \{\pm \e_1,\ldots,\pm \e_k\}$ for all
$i>1$.
\Definition[def:B26]  \hyperdef\defBtwentysix{Definition}{B26}{} 
Let  $\R$ and $\bar \R\in \Z^k$. 
The region $\R$ is
\defword{lattice path connected in $\bar \R$} 
if for all $\z_1$ and $\z_2\in \R$ there exists a lattice path
$\{T_i\}_{i\ge1}$ contained in $\bar \R$ such that $T_1=\z_1$ and
$T_i=\z_2$ for some positive integer~$i$.
The region $\R$ is
\defword{lattice path connected } if it is lattice path connected in itself.
\DefinitionStop

\Definition[def:B27]  \hyperdef\defBtwentyseven{Definition}{B27}{} For any subsets $S$, $\R$,
and $\bar \R \subset\Z^k$, the region $\R$ is
\defword{$S$-path connected in $\bar R$} if for all $\z_1$
and $\z_2\in \R$ there
exists a sequence $\{T_i\}_{i\ge1}$ contained in $\bar \R$ such that
$T_1=\z_1$
and  $T_i=\z_2$ for some positive integer~$i$, and $T_i-T_{i-1}\in S$ for all
$i>1$.
\DefinitionStop

Thus a region is lattice path connected if it is $S$-path connected in itself
for $S=\{\pm\e_1,\ldots,\e_k\}$.

\Lemma[lem:B28a]  \hyperdef\lemBtwentyeighta{Lemma}{B28a}{} Let $\R\subset\Z^k$ be a \hyperref\defBeighteen{polyhedral region}. For any
positive integer $n$, $\R$ can be written as the union of a \hyperref\defBeleven{set of
measure zero} and a \hyperref\defBeighteen{polyhedral region} $\R'$ such that
every $\z\in \R'$ lies in a \hyperref\defbox{$k$-dimensional box of size $n$}
contained entirely in $\R$.
\LemmaStop

\Proof
Let $\R'=\cap_{\v\in B} (R-\v)$ where 
$B=\{\b\in \Z^k: \text{\ for each\ }
 i\in \{1,\ldots, k\}, 0\le b_i \le n\}$.
Clearly $\R'$ is a polyhedral region and for every $\z \in \R'$
the box $\z + B=\{\z + \b:\b\in B\}$
is contained in $\R$, so we need to show 
that $S=\R\setminus \R'$ is a set of measure zero.

Since $\R$ is the intersection of a finite number of half-spaces, 
there exists a finite set $T\subset \Z^k \times \Z$ such that 
$\z\in\R$ if and only if $\z \in \Z^k$ and $\v\cdot\z\le n$
for all $(\v,n)\in T$.
Thus, $\z \in S$ implies there exists $(\v, n) \in T$ and 
$\b\in B$ such that $\v \cdot \z\le n$ and $\v \cdot
(\z+\b) > n$, which in turn implies $\v \cdot \z = m$
for some integer
$m$ such that $n-\v \cdot \b < m\le n$.
It follows that $S$ can be covered by hyperplanes of the form 
$\{\z:\v \cdot\z =m\}$, where $\b \in B$,
$(\v, n) \in T$ and $n-\v \cdot \b < m\le n$. Clearly, there are
a finite number of such hyperplanes, so $S$ is a set of measure zero.
\ProofStop


\Lemma[lem:B28b]  \hyperdef\lemBtwentyeightb{Lemma}{B28b}{}
Let $B_0$ and $B_1$ be \hyperref\defbox{$k$-dimensional boxes of size $1$,} 
let $\bar S$ be the convex hull of $B_0$ and $B_1$ 
in $\Q^k$, and let $S$ be the set of integer points
in $\bar S$. Then $S$ is \hyperref\defBtwentysix{lattice path connected}.
\LemmaStop

\Proof
Let $M$ be a $k\times k$ matrix with entries equal to
$\pm 1$ on the diagonal and $0$ off the diagonal.  It is easily seen
that the lemma is true for the boxes $B_0$ and $B_1$ 
if and only if it is true for the reflections 
$M B_0 = \{Mb:b\in B_0\}$ and 
$M B_1 = \{Mb:b\in B_1\}$ of $B_0$ and $B_1$. Similarly, letting
$\v \in \Z^k$, the lemma is true for $B_0$ and $B_1$ if and 
only if it is true for the translations 
$B_0+\v=\{\b+\v:\b \in B_0\}$ 
and 
$B_1+\v=\{\b+\v:\b \in B_1\}$ 
of $B_0$ and $B_1$.  By applying a sequence of such transformations,
we may assume that $B_0$ is the unit 
$k$-dimensional box at the origin in the first
orthant, $B_0=\{\z \in \Z^k: \text {\ for each\ } i \in
\{1,\ldots,k\}, 0\le z_i \le 1\}$, and that $B_1=B_0+\w$ where
$\w \in \Z^k$ and $w_i\ge0$ for each $i\in\{1,\ldots,k\}$.

Further, if $w_i=0$ for some $i\in\{1,\ldots,k\}$, then the lemma
follows easily by induction from the case of dimension $k-1$.
Since the case of dimension $1$ is trivial, we may assume that 
$w_i > 0$ for each $i\in\{1,\ldots,k\}$. 

Let $\bar B_0$
be the convex hull of $B_0$ in $\Q^k$.  
Thus, $\bar B_0
=\{\z \in \Q^k: \text {\ for each\ } i \in
\{1,\ldots,k\}, 0\le z_i \le 1\}$.

We claim that any $\z\in S$ 
can be written in the form
$\z=\z'+ s \w$,
where
$\z'\in \bar B_0$,
$s\in\Q$, and $s\ge 0$.
Since $\z \in S$, 
$$ \z=
\sum_{\b\in B_0} \lambda_{\b} \b
+ \sum_{\b\in B_1} \lambda_{\b} \b \quad,
$$
where 
$$ \sum_{\b\in B_0} \lambda_{\b} +
\sum_{\b\in B_1} \lambda_{\b} =1\quad.
$$
Hence,
$$\align \z &=
\sum_{\b\in B_0} \lambda_{\b} \b +
\sum_{\b\in B_0} \lambda_{\b+\w} (\b +\w)\\
&= \sum_{\b\in B_0} (\lambda_{\b}+\lambda_{\b +\w}) \b +
\sum_{\b\in B_0} \lambda_{\b+\w} \w\\
&=\z' + s \w 
\quad,\\
\endalign
$$
where
$$ \z'
= \sum_{\b\in B_0} (\lambda_{\b}+\lambda_{\b +\w}) \b 
$$
and
$$ s= \sum_{\b\in B_0} \lambda_{\b+\w} \ge 0
\quad.$$
Since
$$
\sum_{\b\in B_0} (\lambda_{\b}+\lambda_{\b +\w}) 
= \sum_{\b\in B_0} \lambda_{\b}+
\sum_{\b\in B_1} \lambda_{\b } 
=1 \quad,
$$
it follows that 
$\z'\in \bar B_0$.

We claim that for any $\z\in S\setminus B_1$, there exists $j \in
\{1,\ldots,k\}$ such that $\z+\e_j\in S$.
Let $\z=\z'+s\w$ where
$\z'\in \bar B_0$, $s\in \Q$ and $s\ge 0$.  
For each $i\in \{1,\ldots,k\}$,
the line $\{\z'-r\w:r\in\Q\}$ intersects the hyperplane
$\z\cdot \e_i=0$ at a point $\v_i=\z'-r_i \w$ where
$r_i\in\Q$ and $r_i\ge 0$.  
Thus, $v_{i,i}=0$ for each $i\in\{1,\ldots,k\}$.  Let $j\in\{1,\ldots,k\}$
be such that $r_j$ is minimal.  By the minimality of $r_j$
and the positivity of $w_i$, it follows that $v_{j,i}\ge v_{i,i}=0$
for $i\ne j$.  Thus, $v_{j,i}\ge 0$ for all $i\in\{1,\ldots,k\}$.
Further, since $0\le z_{i}'\le 1$, and $r_i\ge 0$, it follows that
$0\le v_{j,i}\le 1$ for all $i\in\{1,\ldots,k\}$ and $v_{j,j}=0$.
Letting $t=r+s$, it follows that $\z=\v_j+t \w$,
and, hence,
$$\z+\e_j=(1-t)(\v_j+\e_j)+t(\v_j+\e_j+\w)
\quad.$$
It is easily seen
that $t<1$, otherwise $\z \in B_1$.
Since $v_{j,j}=0$ and $\v_j \in \bar B_0$, it follows that $
\v_j+\e_j\in \bar B_0$, 
and, hence, $\v_j+\e_j+\w\in \bar B_1$. 
Thus, $\z+\e_j\in \bar S$ as claimed.

We show that every $\z\in S$ is lattice path connected to
a point in $B_1$.  
Suppose to the contrary some $\z \in S\setminus B_1$ is not
lattice path connected to a point in $B_1$.  Assume that 
$\sum_{i=1}^k z_i$ is maximal.  Such a $\z$ exists since 
$\sum_{i=1}^k z_i<\sum_{i=1}^k w_i$ for all $\z\in S\setminus B_1$.
For some $j\in \{1,\ldots,k\}$, we have $\z+\e_j \in S$.
By the maximality of $\sum_{i=1}^k z_i$, it follows that 
$\z+\e_j \in B_1$.
Thus, $\z$ is lattice path connected to $B_1$ contrary to 
assumption. 
Clearly $B_1$ is lattice path connected, so
$S$ is lattice path connected.

\ProofStop

\Corollary[cor:B28c]  \hyperdef\corBtwentyeightc{Corollary}{B28c}{} Let $\R\subset\Z^k$ be a \hyperref\defBeighteen{polyhedral region} 
and let $\z_1$ and $\z_2\in R$.
If $\z_1$ and $\z_2$ are contained in 
\hyperref\defbox{$k$-dimensional boxes of size $1$} contained entirely
in $R$, then
there exists a lattice path from $\z_1$ to $\z_2$ contained
entirely in $R$.  
\CorollaryStop

\Proof
Let $B_1$ and $B_2\subset \R$ be $k$-dimensional boxes
containing $\z_1$ and $\z_2$ respectively.
Let $\bar S$ be the convex hull of $B_0$ and $B_1$ in $\Q^k$
and let $S$ be the set of integer points in $\bar S$. By the definition
of a polyhedral region there exists a convex subset $\bar R$ of $\Q^k$
such that $R$ is the set of integer points in $\bar R$.  Since $\bar R$
is convex, it contains the convex hull of any of its subsets.
Thus, 
$\bar S\subset \bar R$ and, hence, $S\subset R$.  But $S$ is lattice path
connected by Lemma~\hyperref\lemBtwentyeightb{\ref[lem:B28b]}.
\ProofStop

\hyperdef\chapteRiiiSECvii{ChapterSection}{chapteRiiiSECvii}{}
\Section Structure theorem for honest hypergeometric terms

\Theorem[thm:B29]  \hyperdef\thmBtwentynine{Theorem}{B29}{} Let $f$ be an \hyperref\defBthirteena{honest} \hgt\ on $\Z^k$. There exist
relatively prime
polynomials $C$ and $D\in K[\z]$, a finite set $V\subset\Z^k$,
univariate polynomials $a_{\v},b_{\v}\in K[z]$, $\v\in V$
(all of which can be determined as in Theorem~\hyperref\thmBnine{\ref[thm:B9]}), and a
finite number of \hyperref\defBeighteen{polyhedral regions} $\R_1,\ldots,\R_m$ such that
\Enumerate
\item $\Z^k$ is the disjoint union of the $\R_i$ and a \hyperref\defBeleven{set of measure zero};
\item for each $i\in\{1,\ldots,m\}$ there exists $\z_0\in \R_i$
such that $C(\z_0)\ne0$, and for all $\z\in \R_i$ for which
$D(\z)\ne0$,
$$f(\z)=f(\z_0)\frac{C(\z)}{C(\z_0)}\frac{D(
\z_0)}{D(\z)}\prod_{\v\in V}\gp j{\z_0\cdot\v}{
\z\cdot\v}\frac{a_{\v}(j)}{b_{\v}(j)}.$$
\item  all the terms $a_{\v}(j)$ and $b_{\v}(j)$
occurring in the product are nonzero.
\EnumerateStop
\TheoremStop

We conjecture that Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]} is true for \hgt s that
are not honest if the condition that $C$ and $D$ are relatively prime
is dropped.

Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]} applies to \hgt s on polyhedral regions
other than $\Z^k$ via Lemma~\hyperref\lemBtwentyoneb{\ref[lem:B21b]}.

\Proof 
If $f$ is a \zd\  and $pf=0$, then the lemma is true with $D=p$, $C=1$,
$V$ empty, and one region $\R_1=\Z^k$.
We assume hence forth that $f$ is not a \zd\.
Let $R_{\w}$ be the term ratio of $f$ in the direction $\w$.
By Theorem~\hyperref\thmBnine{\ref[thm:B9]},
$$R_{\w}(\z)=\frac{C(\z+\w)}{C(\z)}\frac{D(
\z)}{D(\z+\w)}\prod_{\v\in V}\gp j0{\v\cdot
\w}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot
\v+j)}$$
for all $\w\in\Z^k$.  We may assume $C$ and $D$ are relatively prime.
Let $\bar A_{\w}$ and $\bar B_{\w} \in K[\z]$ 
be relatively prime polynomials such that
\hyperdef\Btwentyninezero{item}{zero}{
$$
\frac{\bar A_{\w}}{\bar B_{\w}}=\prod_{\v\in V}\gp
j0{\v\cdot\w}\frac{a_{\w}(\z\cdot\v+j)}{b_{
\w}(\z\cdot\v+j)}.\tag 1$$}
Thus $\bar A_{\w}$ and $\bar B_{\w}$ are products of simple
polynomials, and by Lemma~\hyperref\lemBtwelve{\ref[lem:B12]} $\bar A_{\w}$ and $\bar
B_{\w}$ are nonzero except on a set of measure zero.

Since $f$ is honest, for each $\w\in\Z$ there exist relatively
prime polynomials $A_{\w}$ and $B_{\w}\in K[\z]$ such
that $A_{\w}f=B_{\w}f^{\w}$~a.e. Since $f$ is not a \zd, by
Lemma~\hyperref\lemBsix{\ref[lem:B6]} the term ratio $R_{\w}$ is unique. Hence,
$$\frac{A_{\w}}{B_{\w}}=R_{\w}=\frac{C^{\w}D\bar
A_{\w}}{CD^{\w}\bar B_{\w}}$$
for all $\w\in\Z^k$ and, hence,
there exist relatively prime polynomials 
$p_{\w} $
and 
$q_{\w} \in K[\z]$ such that
$$p_{\w}A_{\w}
=q_{\w}C^{\w}D\bar A_{\w}
\text{ and }
p_{\w}B_{\w}
=q_{\w}CD^{\w}\bar B_{\w}\quad.$$
Since $p_{\w}$ and $q_{\w}$ are relatively prime,
it follows that 
$q_{\w} \mid A_{\w}$
and 
$q_{\w} \mid B_{\w}$, and 
since $A_{\w}$ and $B_{\w}$ are relatively prime, it follows that 
$q_{\w}$ must be trivial.
Hence, for each $\w\in\Z^k$,
$$C^{\w}D\bar A_{\w}f
=CD^{\w}\bar B_{\w}f^{\w}\text{ a.e.}$$

Let $d$ be the total degree of $CD$. By Lemma~\hyperref\lemBfifteen{\ref[lem:B15]}, $CD$ is
nonzero for at least one point in any 
$k$-dimensional box of size $d$. Let
$S_0\subset\Z^k$ be the union of all 
$k$-dimensional boxes of size $d$ containing $0$.
Let $S_1=\{\vec s\pm\e_i\colon\vec s\in S_0\text{ and
}i\in\{1,\ldots,k\}\}$. Thus, $S_1$ is the union of all 
$k$-dimensional boxes of size
$d$ containing a point $\pm\e_i$, $i\in\{1,\ldots,k\}$. Finally,
let $S=S_0-S_1=\{\vec s_0-\vec s_1\colon\vec s_0\in S_0,\vec s_1\in
S_1\}$. 
For each $\w\in\Z^k$, the polynomials $\bar A_{\w}$ and
$\bar B_{\w}$ are nonzero except on a set of measure zero, and
$\bar A_{\w}C^{\w}Df
=\bar B_{\w}CD^{\w}f^{\w}$
except on a set of measure zero.
Call the union of these two sets of measure zero $H_1(\w)$
and let $H_1=\cup_{\w\in S}H_1(\w)$.  Since $S$ is finite,
it follows that $H_1$ is a set of measure zero.   
Thus, for all $\w\in S$ and all $
\z\notin H_1$,
\Enumerate \itemno=1
\item[B29:one] \hyperdef\Btwentynineone{item}{one}{} $\bar A_{\w}(\z)\ne0$,
$\bar B_{\w}(\z)\ne0$, and
\item[B29:three] \hyperdef\Btwentyninethree{item}{three}{} $\bar A_{\w}(\z)C(\z+\w)D(
\z)f(\z)=\bar B_{\w}(\z)C(\z)D(\z+\w)f(\z+
\w)$.
\EnumerateStop

\def\RR{{\bar {\R}}}
\accentedsymbol\RRR{{\Bar {\Bar {\Cal R}}}}
Let $H_2$ be a finite set of hyperplanes covering $H_1$. The
hyperplanes in $H_2$ divide space into a finite number of polyhedral
regions $\RRR_i$ such that $\Z^k$ is the disjoint union of the regions and the
union of the hyperplanes. (The hyperplanes are not necessarily disjoint,
but the regions are disjoint from each other and from the hyperplanes.)
Further, by Lemma~\hyperref\lemBtwentyeighta{\ref[lem:B28a]} each region
$\RRR_i$ can be written as a union of a polyhedral region $\RR_i$ and a set of
measure zero such that 
each $\z\in\RR_i$ is
contained in a
$k$-dimensional box of size $d$ contained entirely in $\RRR_i$.
By Lemma~\hyperref\lemBtwentyeightb{\ref[lem:B28b]} each $\RR_i$ can be written as a union of
a polyhedral region $\R_i$ and a set of measure zero such that 
$\R_i$ is lattice path connected in $\RR_i$. 
Thus, 
\Enumerate \itemno=3
\item[B29:four] \hyperdef\Btwentyninefour{item}{four}{} $\Z^k=\R_1\cup\cdots\cup \R_m\cup H$, where $H$ is
a set of measure zero;
\item[B29:five] \hyperdef\Btwentyninefive{item}{five}{} $\bar A_{\w}C^{\w}Df=\bar B_{\w}CD^{
\w}f^{\w}$ for every $\z\in \RRR_i$, $i\in\{1,\ldots,m\}$, and
every $\w\in S$;
\item[B29:six] \hyperdef\Btwentyninesix{item}{six}{} $\bar A_{\w}$ and $\bar B_{\w}$ are nonzero on
$\RRR_i$, $i\in\{1,\ldots,m\}$, for every $\w\in S$;
\item[B29:seven] \hyperdef\Btwentynineseven{item}{seven}{} $\R_i$ is lattice path connected in $\RR_i$ for $i\in\{1,\ldots,m\}$;
\item[B29:eight] \hyperdef\Btwentynineeight{item}{eight}{} for every $\z\in \RR_i$, $\z$ is contained in a
$k$-dimensional box of size $d$ contained in $\RRR_i$, $i\in\{1,\ldots,m\}$.
\EnumerateStop
From (\hyperref\Btwentyninezero{1}), (\hyperref\Btwentyninefive{\ref[B29:five]}) and (\hyperref\Btwentyninesix{\ref[B29:six]}) it follows that
\Enumerate \itemno=8
\item[B29:nine] \hyperdef\Btwentyninenine{item}{nine}{} $\ds{f(\z_2)C(\z_1)D(\z_2)=f(
\z_1)C(\z_2)D(\z_1)\prod_{\v\in V}\gp j{\z_1\cdot
\v}{\z_2\cdot\z}\frac{a_{\v}(j)}{b_{\v}(j)}}$ if $
\z_1\in \RRR_i$ and $\z_2-\z_1\in S$, $i\in\{1,\ldots,m\}$.
\EnumerateStop
Since any $\R_i$ of measure zero can be absorbed into~$H$ we may assume
$\R_i$ is not a set a measure zero for $i\in\{1,\ldots,m\}$.
For each $i\in\{1,\ldots,m\}$ let 
$\R_i'=\{\z\in \R_i\colon C(\z)D(\z)\ne0\}$, and let
$\RRR_i'=\{\z\in \RRR_i\colon C(\z)D(\z)\ne0\}$.
 Since $\R_i$ is not a set of measure zero, $\R_i$
contains a 
$k$-dimensional box of size~$d$ by Lemma~\hyperref\lemBtwentyone{\ref[lem:B21]}.
Hence, by Lemma~\hyperref\lemBfifteen{\ref[lem:B15]}, $C(
\z)D(\z)$ is nonzero for some $\z\in \R_i$, and hence $\R_i'$ is
not empty.

We claim $\R_i'$ is $S$-path connected in $\RRR_i'$ for each
$i\in\{1,\ldots,m\}$. Let $\z_1$ and $\z_2\in \R_i'$ be given.
We construct a sequence $\v_1',\ldots,\v_\ell'$ in $\RR_i'$
such that 
$\v_1'=\z_1$, $\v_\ell'=\z_2$, and $\v_j'-\v_{j-1}'\in S$
for $j=2,\ldots,\ell$.
Since $\R_i$ is lattice path connected in $\RR_i$, there exists a sequence
$\v_1,\ldots,\v_\ell$ in $\RR_i$ such that
$\v_1=\z_1$, $\v_{\ell}= \z_2$, and $\v_j-\v_{j-1}\in
\{\pm\e_1,\ldots,\pm\e_k\}$. For each $j\in\{1,\ldots,\ell\}$ there is a 
$k$-dimensional box of size $d$
containing $\v_j$ contained in $\RRR_i$. This box contains a point
$\v_j'$ such that $C(\v_j')D(\v_j')\ne0$, since the total
degree of $CD$ is~$d$. Obviously, we can take $\v_1'=\z_1$ and $\v_{\ell}'=
\z_2$. By the construction of $S$, it's clear that $\v_j'-\v_{j-1}'\in S$ for
$j\in\{2,\ldots,\ell\}$. Thus, $\R_i'$ is $S$-path connected in $\RRR_i'$ as
claimed.


For all $\z_1$ and $\z_2\in\RRR_i'$, 
define 
$$g(\z_1,\z_2)
=\frac{C(\z_2)}{C(\z_1)}
\frac{D(\z_1)}{D(\z_2)}
\prod_{\v\in V}\gp j{\z_1\cdot\v}{\z_2\cdot\v}
\frac{a_{\v}(j)}{b_{\v}(j)}.$$
We claim that for all $\z_1$ and $\z_2\in \R_i'$ ,
$$ f(\z_2) =f(\z_1)g(\z_1,\z_2). $$
We show by induction on $j$ that if $\{\z_\nu\}_{\nu\ge 1}$ is a sequence
in $\RRR_i$ such that $\z_\nu-\z_{\nu-1}\in S$ for all $\nu\ge 2$,
then 
$$ f(\z_j)=f(\z_1)g(\z_1,\z_j) $$
for all $j\ge 1$.
The statement is clearly true if $j=1$.  Suppose inductively that 
$f(\z_{j-1})=f(\z_1)g(\z_1,\z_{j-1})$.  Since $\z_j-\z_{j-1}\in S$,
it follows by 
(\hyperref\Btwentyninenine{\ref[B29:nine]})
that $f(\z_j)=f(\z_{j-1})g(\z_{j-1},\z_j)$.
Hence, 
$f(\z_j)=
f(\z_1)g(\z_1,\z_{j-1})
g(\z_{j-1},\z_j)$.
Using the fact that 
$\gp iab\,\gp ibc=\gp iac$,
it is easily seen that 
$ f(\z_j)=f(\z_1)g(\z_1,\z_j) $,
as was to be shown.
Since $\R_i'$ is $S$-path connected in $\RRR_i'$, it follows that
$ f(\z_2) =f(\z_1)g(\z_1,\z_2)$ for all $\z_1$ and $\z_2\in \R_i'$.


Let $\z_0\in \R_i'$. 
We claim that for all 
$\z\in \R_i$ 
such that $D(\z)\ne0$,
$$f(\z)=f(\z_0)g(\z_0,\z).$$
If $\z\in\R_i'$, we're done.
If $\z\notin \R_i'$, then, since $D(\z)\ne0$,
we must have $C(\z)=0$.
In this case~(\hyperref\Btwentyninenine{\ref[B29:nine]}) implies $f(\z)=0$.
But $g(\z_0,\z)=0$, 
so $f(\z)=f(\z_0)g(\z_0,\z)$.

\ProofStop

\Corollary[cor:B30]  \hyperdef\corBthirty{Corollary}{B30}{} Let $f$ be an \hyperref\defBthirteena{honest} \hgt\ on $\Z^k$. Then there
exist relatively prime polynomials $C$ and $D\in K[\z]$ (as in
Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]}) and  a finite number of \hyperref\defBeighteen{polyhedral regions}
$\R_1,\ldots,\R_L$ such that
$\Z^k$ is the union of the $\R_\ell$ and a \hyperref\defBeleven{set of measure zero} and for each
region $\R_\ell$
there exist a finite set $V\subset\Z^k$ and
univariate polynomials $a_{\v}$ and $b_{\v}\in K[z]$ and an
integer $n_{\v}$ for each $\v\in V$ such that, for all $
\z\in \R_\ell$,
\Enumerate
\item $\ds{f(\z)=\frac{C(\z)}{D(\z)}\prod_{\v\in
V}\prod_{j=1}^{\v\cdot\z+n_{\v}}\frac{a_{
\v}(j)}{b_{\v}(j)}}$
for all $\z\in \R_{\ell}$ for which $D(\z)\ne 0$,
\item for all $\v\in V$, $\v\cdot\z+n_{\v}$ is a
positive integer, and
\item for all $\v\in V$ and $j$, $1\le j\le\v\cdot
\z+n_{\v}$, $a_{\v}(j)\ne0$ and $b_{\v}(j)\ne0$.
\EnumerateStop
\CorollaryStop


Corollary~\hyperref\corBthirty{\ref[cor:B30]} applies to \hgt s on polyhedral regions
other than $\Z^k$ via Lemma~\hyperref\lemBtwentyoneb{\ref[lem:B21b]}.

\Proof
This follows from Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]} and Lemma~\hyperref\lemBtwentyfive{\ref[lem:B25]}.
The product 
$$
\prod_{\v\in V}\gp j{\z_0\cdot\v}{\z\cdot
\v}\frac{a_{\v}(j)}{b_{\v}(j)}$$
that occurs in the expression for $f(\z)$ in Theorem \hyperref\thmBtwentynine{\ref[thm:B29]}
is a weakly factorial \hgt\ on the region $\R_i$.
By lemma \hyperref\lemBtwentyfive{\ref[lem:B25]}, the region $\R_i$ can be divided into 
polyhedral subregions such that the weakly factorial
\hgt\ is factorial on
each subregion.
\ProofStop

\Corollary[cor:B31]  \hyperdef\corBthirtyone{Corollary}{B31}{} Let $f$ be an \hyperref\defBthirteena{honest} \hgt\ on $\Z^k$
over a field $K$ that is algebraically closed. Then there exist
relatively prime polynomials $C$ and $D\in K[\z]$ (as in
Theorem~\hyperref\thmBtwentynine{\ref[thm:B29]}) and a finite number of \hyperref\defBeighteen{polyhedral regions}
$\R_1,\ldots,\R_L$ such that $\Z^k$ is the union of the $\R_{\ell}$ and
a \hyperref\defBeleven{set of measure zero}, and for each region $\R_{\ell}$ there exist a
vector $\vecgamma\in K^k$, constants $m_1,\ldots,m_p,n_1,\ldots,n_q\in
K$, vectors $\v_1,\ldots,\v_p,\w_1,\ldots,\w_q\in\Z^k$,
and integers $r_1,\ldots,r_p,s_1,\ldots,s_q$ such that
\Enumerate
\item for all $\z\in \R_{\ell}$ such that $D(\z)\ne0$,
$$f(\z)=
\gamma_1^{z_1}\cdots\gamma_k^{z_k}
\frac{C(\z)}{D(\z)}
\frac{\prod_{i=1}^p(m_i)_{\v_i\cdot
\z+r_i}}{\prod_{j=1}^q(n_j)_{\w_j\cdot\z+s_j}};$$
\item for all $i$ and $j$ and $\z\in \R_{\ell}$, $\v_i\cdot
\z+r_i$ and $\w_j\cdot\z+s_j$ are positive;
\item the Pochhammer symbols occurring
in the products are nonzero.
\EnumerateStop
\CorollaryStop


Corollary~\hyperref\corBthirtyone{\ref[cor:B31]} applies to \hgt s on polyhedral regions
other than $\Z^k$ via Lemma~\hyperref\lemBtwentyoneb{\ref[lem:B21b]}.

\Proof This corollary is an immediate consequence of
Corollary~\hyperref\corBthirty{\ref[cor:B30]} and Lemma~\hyperref\lemBtwentythree{\ref[lem:B23]}.
\ProofStop




==> two.tex <==

\hyperdef\chapteRii{ChapterSection}{chapteRii}{}
\Chapter The Rational Solutions of \\
$R_iR_j^{\e_i}=R_jR_i^{\e_j}$

The main result of this chapter is Theorem~\hyperref\thmfifteena{\ref[thm:15a]} \hyperref\oresato{\OreSato}, which reveals
the multiplicative structure of solutions to the relation for the term ratios.

\smallskip
\Statement[thm:15a] 
\noindent{\bf{}Theorem~\hyperref\thmfifteena{\ref[thm:15a]}} \ 
Let $R_i\in K(\z)$, $i=1,\ldots,k$, be rational functions such that
$$R_iR_j^{\e_i}=R_jR_i^{\e_j}$$
for all $i,j\in\{1,\ldots,k\}$. Then there exist polynomials $C$ and $D\in K[\z]$, a finite set $V\subset\Z^k$, and univariate polynomials $a_{\v}$ and $b_{\v}\in K[z]$ for each $\v\in V$ such that for all $i\in\{1,\ldots,k\}$,
$$R_i(\z)=\frac{C(\z+\e_i)}{C(\z)}\frac{D(\z)}{D(\z+\e_i)}\prod_{\v\in V}\gp j0{\v_i}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)}.$$
\StatementStop

Recall that the symbol $\gp jab{}$ denotes 
$\prod_{j=a}^{b-1}$ if $b>a$,
$1$ if $a=b$,
and
$1/\prod_{j=b}^{a-1}$ if $a>b$.



We require the following definitions.

\Definition[def:A1]  \hyperdef\defAone{Definition}{A1}{} Define the \defword{lead term} of a nonzero polynomial $p\in 
K[z_{1},\ldots,z_{k}]$ to be the nonzero term $cz_{1}^{n_{1}}\cdots 
z_{k}^{n_{k}}$ of~$p$ for which the degree vector $(n_{1},\ldots,n_{k})$ is 
maximal in the standard ordering. The polynomial $p$ is 
\defword{monic} if the coefficient of the lead term is~$1$.
\DefinitionStop

For any $\vecgamma=(\gamma_1,\ldots,\gamma_k)\in (K(\z))^k$ such
that $\gamma_i\ne 0$ for each $i\in \{1,\ldots,k\}$ and
$\v=(v_1,\ldots,v_k)\in \Z^k$, we denote
$\gamma_{1}^{v_{1}}\cdots \gamma_{k}^{v_{k}}$
by $\vecgamma^{\v}$.

\Lemma[lem:zero]  \hyperdef\lemzero{Lemma}{zero}{} Let $\z=(z_{1},\ldots,z_{k})$, let $\vec m\in\Z^{k}$, 
and 
let $p=\sum_{\vec n\in\Z^{k}}c_{\vec n}\z^{\vec n}\in 
K[z_{1},\ldots,z_{k}]$ be a polynomial. If the term $c_{\vec m}
\z^{\vec m}$ 
is maximal in the sense that $\z^{\vec m}\mid \z^{\vec n}$ and 
$\vec m\ne\vec n$ 
imply $c_{\vec n}=0$, then for any $\v\in\Q^{k}$, the coefficient of 
$\z^{\vec m}$ in $p^{\v}$ is equal to the coefficient $c_{\vec m}$ of 
$\z^{\vec m}$ in $p$.
\LemmaStop

\Proof By the binomial theorem, if $\z^{\vec m}$ is not a proper 
divisor of $\z^{\vec n}$, then the coefficient of $\z^{\vec m}$ in 
$(\z+\v)^{\vec n}-\z^{\vec n}$ is~$0$. If $\z^{\vec m}$ is a proper 
divisor of $\z^{\vec n}$, then $c_{\vec n}=0$. Hence, in either case, the 
coefficient of $\z^{\vec m}$ in $c_{\vec n}((\z+\v)^{
\vec n}-\z^{\vec n})$ 
is~$0$, and, hence, the coefficient of $\z^{\vec m}$ in $p^{
\v}-p=\sum c_{\vec n}((\z+\v)^{\vec n}-\z^{\vec n})$ is~$0$.
\ProofStop

\Corollary If $p\in K[z_{1},\ldots,z_{k}]$ is monic, then so is 
$p^{\v}$ for any $\v\in\Q^{k}$.
\CorollaryStop

\Corollary[cor:second]  \hyperdef\corsecond{Corollary}{second}{} If $p\in K(z_{1},\ldots,z_{k})$ is nonzero, $
\v\in\Q^{k}$, $c\in K$, and $p^{\v}=cp$, then $c=1$.
\CorollaryStop

\hyperdef\chapteRiiSECi{ChapterSection}{chapteRiiSECi}{}
\Section Gosper's lemma

We require the following adaptation of 
Petkov\hacek sek's refinement~\hyperref\Petninetytwo{\bibref[Pet92]} of 
Gosper's lemma~\hyperref\Gospseventyeight{\bibref[Gosp78]}.

\Lemma[lem:one]  \hyperdef\lemone{Lemma}{one}{} 
Let $K$ be a field of characteristic~$0$, and let $R\in 
K(z_1,\ldots,z_k)$ be a nonzero rational function. There exist polynomials $A$, $B$, 
$C$, and~$D\in K[z_1,\ldots,z_k]$ such that
$$R=\frac AB\frac{C^{\e_{1}}}C\frac D{D^{\e_{1}}}$$
and
\Enumerate
\item $A$ and $B^{n\e_1}$ are relatively prime for all $n\in\Z$,
\item $A$ and $CD^{\e_{1}}$ are relatively prime,
\item $B$ and $C^{\e_{1}}D$ are relatively prime, and
\item $C$ and $D$ are relatively prime.
\EnumerateStop
\LemmaStop

\Proof The lemma is proved by a double application 
of Gosper's 
lemma. The gcds below are with respect to $z_1$. By Gosper's lemma there exist $a$, $b$, 
and~$c\in K(z_2,\ldots,z_k)[z_1]$ such that $\ds{R=\frac ab\frac{c^{\e_1}}c}$ where 
$\gcd(a,b^{n\e_1})=1$ for all nonnegative integers~$n$ and by Petkov\hacek 
sek's refinement we may assume in addition that $\gcd(a,c)=1$ and 
$\gcd(b,c^{\e_1})=1$. Applying this principle again, this time to 
$\ds{\frac ba}$, we can write
$$\frac ba=\frac BA\frac {d^{\e_1}}d\leqno(1)$$
where $A,B,d\in K(z_2,\ldots,z_k)[z_1]$, $\gcd(B,A^{n\e_1})=1$ for all integers~$n\ge0$, 
$\gcd(B,d)=1$, and $\gcd(A,d^{\e_1})=1$. Since $\gcd(B,Ad)=1$, it 
follows from~$(1)$ that $B\mid b$. Similarly, $A\mid a$. Hence, 
$\gcd(A,B^{n\e_1})=1$ for all nonnegative integers~$n$. On the other 
hand, since $\gcd(B,A^{n\e_1})=1$ for all nonnegative integers~$n$, it 
follows that $\gcd(A,B^{n\e_1})=1$ for all nonpositive integers~$n$. 
Hence $\gcd(A,B^{n\e_1})=1$ for all integers~$n$, positive, negative, or 
zero. Let $g=\gcd(c,d)$, let $C=c/g$, and let $D=d/g$. It's easily 
seen that $\ds{R=\frac AB\frac{C^{\e_1}}C\frac D{D^{\e_1}}}$, 
$\gcd(A,CD^{\e_1})=1$, $\gcd(B,C^{\e_1})=1$, and $\gcd(C,D)=1$.

For some $\alpha$ and $\beta\in K[z_2,\ldots,z_k]$, $\alpha A$ and
$\beta B$ are in $K[\z]$. Replace $A$ with $\alpha\beta A$ and $B$
with $\alpha\beta B$; the ratio $A/B$ is unchanged, hence, $R$ is unchanged.
 Similarly, adjust $C$ and $D$ so that $A$, $B$,
$C$, and $D$ are in $K[\z]$. If $A$ and $B$ have a common factor
$d$ (which must be free of $z_1$), we replace $A$ and $B$ by $A/d$
and $B/d$. Since $d=d^{n\e_1}$ it follows that $A$ and
$B^{n\e_1}$ are relatively prime for $n\in\Z$. If $C$ has any
divisor $d$ that is free of $z_1$, replace $C$ with $C/d$. Since
$d^{\e_1}=d$, $C^{\e_1}/C$ is unchanged. Similarly, adjust $D$.
If follows that $A_1$ and $CD^{\e_1}$ are relatively prime, $B_1$
and $C^{\e_1}D$ are relatively prime, $C$ and $D$ are
relatively prime, and
$\ds{R=\frac AB\frac{C^{\e_1}}C\frac D{D^{\e_1}}}$. 
\ProofStop

\Definition[def:A2]  \hyperdef\defAtwo{Definition}{A2}{} Let $R\in K(z_{1},\ldots,z_{k})$ be 
a rational function. The rational function~$R$ is said to be 
\defword{simple} over $K$ if it can be written in the form
$$R(\z)=\bar R(\v\cdot\z)=\bar R(v_1z_1+\cdots+v_kz_k)$$
where $\bar R\in K(z)$ is a univariate rational function and $\v\in\Q^k$.
\DefinitionStop

Hence, $(z_{1}^{2}+z_{2}+3z_{3})^{2}$ is simple over $\Q(z_{1})$ but 
(apparently) not over $\Q$. It's easily proved that it's not simple 
over $\Q$ using Corollary~\hyperref\coroldlemmafour{\ref[cor:oldlemmafour]}.

\Lemma[lem:two]  \hyperdef\lemtwo{Lemma}{two}{} Let $K$ be a field of characteristic~$0$, and let 
$R_{1},\ldots,R_{k}\in K(z_{1},\ldots,z_{k})$ be nonzero rational 
functions satisfying the relation
$$R_{i}R_{j}^{\e_{i}}=R_{j}R_{i}^{\e_{j}}$$
for all $i,j\in\{1,\ldots,k\}$. Then there exist polynomials 
$A_{1},\ldots A_{k}$, $B_{1},\ldots,B_{k}$, $C$, and $D$ such that
$$R_{i}=\frac {A_{i}}{B_{i}}\frac{C^{\e_{i}}}C\frac D{D^{
\e_{i}}}$$
for $i\in\{1,\ldots,k\}$, and the irreducible divisors of $A_{i}$ and 
$B_{i}$ are all \hyperref\defAtwo{simple} for $i\in\{1,\ldots,k\}$.
\LemmaStop

\Proof The one-variable case of Lemma~\hyperref\lemtwo{\ref[lem:two]} is trivial. 
The proof of the two-variable case continues through
section
2.4 and the proof of the higher dimensional cases occupies
sections 2.5 through 2.7.

\def\AB{1}
We prove the two-variable case.
In fact, we prove a stronger version of the two-variable
case that is needed for the proof of the higher dimensional cases:
if 
$$R_{1}=\frac{\bar A_{1}}{\bar B_{1}}\frac{\bar C^{\e_{1}}}{\bar C}
\frac {\bar D}{\bar D^{ \e_{1}}}$$
and
$\bar A_{1}$ and $\bar B_{1}^{n\e_{1}}$ are relatively prime
for all $n\in\Z$,
then we may take
$A_1=\bar A_1$,
$B_1=\bar B_1$,
$C=\bar C$,
and
$D=\bar D$.
By Lemma~\hyperref\lemone{\ref[lem:one]}, such
$\bar A_1$,
$\bar B_1$,
$\bar C$,
and
$\bar D$ exist.
Thus, we assume that
$$R_{1}=\frac{A_{1}}{B_{1}}\frac{C^{\e_{1}}}C\frac D{D^{
\e_{1}}}$$
where 
$$A_{1}\text{ and }B_{1}^{n\e_{1}}\text{ are relatively prime
for all $n\in\Z$. 
}\tag{\AB}$$

Let $\ds{r_{i}=R_{i}\frac C{C^{\e_{1}}}\frac{D^{\e_{1}}}D}$.
Thus, $\ds{r_{1}=\frac{A_{1}}{B_{1}}}$. Let $A_{2}$ and $B_{2}$ be 
relatively prime polynomials such that $\ds{r_{2}=\frac{A_{2}}{B_{2}}}$. 
Using $R_{1}R_{2}^{\e_{1}}=R_{2}R_{1}^{\e_{1}}$ and the 
definition of~$r_i$, it's easily verified that $r_{1}r_{2}^{
\e_{1}}=r_{2}r_{1}^{\e_{2}}$ and, hence,
$$A_{1}A_{2}^{\e_{1}}B_{1}^{\e_{2}}B_{2}=A_{1}^{
\e_{2}}A_{2}B_{1}B_{2}^{\e_{1}}.\leqno(2)$$
We will show that the irreducible divisors of the left side of~$(2)$ 
are simple.

\hyperdef\chapteRiiSECii{ChapterSection}{chapteRiiSECii}{}
\Section The divisibility lattice path

For any irreducible divisor $d$ we construct a lattice path 
$\{T_{i}\}$ in $\Z^{2}$ such that for all $i\ge0$, $d^{T_{i}}$ divides 
one of the four factors on the left side of~$(2)$. Further, the 
factor $T_{i}$ divides is determined by the value of 
$S_{i}=T_{i}-T_{i-1}$, which, since $T_{i}$ is a lattice path, is one 
of the four directions $\e_{1}$, $-\e_{1}$, $\e_{2}$, 
and $-\e_{2}$.

To be precise, define
$$X(-\e_{2})=A_{1},\quad X(\e_{1})=A_{2}^{\e_{1}},\quad 
X(\e_{2})=B_{1}^{\e_{2}},\quad X(-\e_{1})=B_{2}.$$
We will construct $T_{i}$ so that
$$d^{T_{i}}\mid X(S_{i}),\quad\text{where 
}S_{i}=T_{i}-T_{i-1}.\leqno(3)$$
The product of the values of $X$ is the left side of~$(2)$. It will be 
useful to also define
$$Y(-\e_{2})=A_{2}^{\e_{1}},\quad Y(\e_{1})=A_{2},\quad 
Y(\e_{2})=B_{1},\quad Y(-\e_{1})=B_{2}^{\e_{1}}$$
so that the product of the values of~$Y$ is the right side of~$(2)$. 
The relationship between terms on the left side of~$(2)$ and terms on 
the right side is captured by the shift relation
$$(Y(\v))^{\v}=X(\v)\leqno(4)$$
and coprimeness condition
$$X(\v)\text{ and }Y(-\v))\text{ are relatively prime}\leqno(5)$$
for $\v\in\{\pm\e_{1},\pm\e_{2}\}$, which are easily 
verified.

We construct the lattice path $\{T_{i}\}$ by induction. Let an 
irreducible divisor~$d$ of the left side of~$(2)$ be given. Since~$d$ 
is irreducible, $d$ must divide $X(\v)$ for some $
\v\in\{\pm\e_{1},\pm\e_{2}\}$. Define $T_{0}=0$ and 
$S_{0}=\v$. Thus, $d^{T_{0}}\mid X(S_{0})$. Now assume inductively 
that $T_{i}$ and $S_{i}$ have been defined for $0\le i\le j$. Since 
$d^{T_{j}}$ divides the left side of~$(2)$, it must also divide the 
right side, and since $d^{T_{j}}$ is irreducible, $d^{T_{j}}\mid 
Y(\v)$ for some $\v\in\{\pm\e_{1},\pm\e_{2}\}$. Let 
$S_{j+1}=\v$ and let $T_{j+1}=T_{j}+S_{j+1}$. Since 
$d^{T_{j}}\mid Y(S_{j+1})$, it follows that 
$d^{T_{j}+S_{j+1}}\mid(Y(S_{j+1}))^{S_{j}+1}$, and hence 
$d^{T_{j+1}}\mid X(S_{j+1})$ by~$(4)$. This completes the induction 
step. We have constructed $T_{i}$ and $S_{i}$ satisfying~$(3)$.


\hyperdef\chapteRiiSECiii{ChapterSection}{chapteRiiSECiii}{}
\Section What goes up must not come down

Having constructed the path~$T$, we explore what restrictions the 
coprimeness conditions~$(5)$ and~(\AB) impose on the shape of~$T$.

From the condition~$(5)$ we deduce path~$T$ does not traverse the same 
segment of the lattice path in opposite directions. By the path~$T$ 
traversing a segment of the lattice in the direction~$\v$, we 
mean for some $i\ge1$, the end points of the segment are $T_{i-1}$ 
and $T_{i}$, and $T_{i}-T_{i-1}=\v$.

Suppose to the contrary the path traverses the same segment in 
opposite directions. Then for some $i$ and $j>0$ we have 
$S_{i}=-S_{j}$ and $T_{i}=T_{j-1}$. By~$(3)$, $d^{T_{j}}\mid 
X(S_{j})$, hence, by~$(4)$, $d^{T_{j-1}}\mid Y(S_{j})$, hence 
$d^{T_{i}}\mid Y(S_{j})$, and hence $d^{T_{i}}\mid Y(-S_{i})$. But 
$d^{T_{i}}\mid X(S_{i})$ which contradicts condition~$(5)$.

Taking $j=i+1$ we see that the path can't reverse directions 
without going in a perpendicular direction first ($S_{i}\ne -S_{i+1}$).

From the condition~(\AB) we deduce that 
the path~$T$ doesn't go up a 
segment and come down one of its horizontal translates. (By go 
up and come down, we mean traverse in the directions $\e_{2}$ 
and $-\e_{2}$, respectively.) Suppose the contrary. Then for 
some $i$ and $j>0$ and $n\in\Z$ we have $S_{i}=-\e_{2}$, 
$S_{j}=\e_{2}$, and $T_{i}=T_{j-1}+n\e_{1}$. By~$(3)$, 
$d^{T_{j}}\mid X(S_{j})$, hence by~$(4)$ $d^{T_{j-1}}\mid Y(S_{j})$, 
hence $d^{T_{i}-n\e_{1}}\mid Y(S_{j})$, hence by the definition 
of~$Y$, $d^{T_{i}-n\e_{1}}\mid B_{1}$, and hence $d^{T_{i}}\mid 
B_{1}^{n\e_{1}}$. But $d^{T_{i}}\mid X(S_{i})=A_{1}$, which 
contradicts~(\AB).

The condition that the path~$T$ doesn't go up a 
segment and come down one of its horizontal translates
immediately implies a stronger condition:
$$
\text{If $T$ goes up any segment, it must not come down any segment.
}\leqno(6)$$
Suppose to the contrary $T$ goes up to $T_{i}$ 
and down to $T_{j}$ ($S_{i}=\e_{2}$ and $S_{j}=-\e_{2}$), and 
assume that $|i-j|$ is minimal. By the minimality of $|i-j|$, 
$S_{k}\ne\pm\e_{2}$ for any $k$ between $i$ and $j$. It follows 
that the segments $(T_{i-1},T_{i})$ and $(T_{j-1},T_{j})$ are 
horizontal translates of each other, contradicting the original condition.

Finally, from ~$(6)$
it's easy to deduce that the path $T$ is unbounded. 
If the path is unbounded vertically, we are done. Thus, we may assume that for 
some $k\ge0$, $|T_{i}\cdot\e_{2}|\le k$ for all~$i$. It follows 
from~$(6)$ that the path can go in a vertical direction at most~$k$ 
times. Since the path can't reverse direction without going in a 
perpendicular direction first, the path can change horizontal 
direction at most $k$ times. Hence the path is unbounded horizontally.

\hyperdef\chapteRiiSECiv{ChapterSection}{chapteRiiSECiv}{}
\Section The divisor $d$ is simple.

Using the fact that the path $T$ is unbounded, we show that it 
satisfies a nontrivial relation $d=d^{\v}$ for some $
\v\in\Z^{2}$. By the fact that $T$ is unbounded, the set ${\Cal 
T}=\{T_{i}:i\ge0\}$ of values assumed by $T$ is infinite. Let $P$ be 
the left side of~$(2)$. For every $t\in\Cal T$, $d^{t}\mid P$. Since 
$\Cal T$ is infinite and $P$ has only finitely many monic divisors, 
$cd^{t_{1}}=d^{t_{2}}$ for some $t_{1}$ and $t_{2}\in\Cal T$ and 
$c\in K$. By Corollary~\hyperref\corsecond{\ref[cor:second]}, $c=1$. Letting $\v=t_{1}-t_{2}$, we have 
$d^{\v}=d$.

Using the equation $d=d^{\v}$, we show that $d$ is the composition 
of a univariate polynomial and a linear polynomial:
$$d(z_{1},z_{2})=p(v_{2}z_{1}-v_{1}z_{2})\quad\text{where }p\in 
K[z].\leqno(7)$$
We may assume without loss of generality that $v_{2}\ne0$. Define 
$$q(z_{1},z_{2})=d(z_{1}+v_{1}z_{2},v_{2}z_{2}).$$ 
Thus, $q=q^{
\e_{2}}$. Iterating the last equation, $q=q^{n\e_{2}}$ for all 
positive integers $n$. Thus,
$q(z_{1},z_{2})=q(z_{1},z_{2}+n)$ identically.
The left side of the last equation 
is free of~$n$ and the right side is symmetric in $n$ and $z_{2}$; thus,  
the left side must also be free of $z_{2}$. Hence $q$ is free of its 
second argument. It's easily verified that 
$d(z_{1},z_{2})=q(z_{1}-(v_{1}/v_{2})z_{2},z_{2}/v_{2})$. Letting 
$p(z)=q(z/v_{2},0)$, $(7)$ is proved and, hence, $d$ is simple.

This completes the proof of the two-variable case.

\hyperdef\chapteRiiSECv{ChapterSection}{chapteRiiSECv}{}
\Section The rational Galois space of a rational function

We require the following definitions and lemmas for the proof of the 
$k>2$ case of Lemma~\hyperref\lemtwo{\ref[lem:two]}.

\Definition[def:A3]  \hyperdef\defAthree{Definition}{A3}{}
Let $S=\{x_1,\ldots,x_k\}$ be a finite set
that is algebraically independent
over $K$, and 
let $R\in K(S)$ be a rational function in
$\vec x=(x_1,\ldots,x_k)$. 
We define the \defword{rational Galois 
space} of $R$ over $K$ with respect to $\vec x$ to be the set 
$$\rgal(R,\vec x,K)=
\{ \v\in \Q^k: R(\vec x + \v)=R(\vec x) \}.$$
\DefinitionStop
We write $\rgal(R)$ for $\rgal(R,\z,K)$;
thus, 
$\rgal(R)=\{ \v\in\Q^{k}:R^{\v}=R\}$.


Let $G$ be the Galois group of $K(\vec x)$ over $K$.
It's easily seen that
$\rgal(R,\vec x,K)$
is isomorphic to the subgroup 
$
\{ g\in G:g(R)=R \text {\ and $g(x_i)-x_i\in \Q$
for $i\in \{1,\ldots,k\}$}\}$ of $G$.


We show that the rational Galois space is a subspace of $\Q^{k}$. It's 
clearly closed under vector addition. By iterating $R^{\v}=R$, it 
follows that $R^{n\v}=R$ for any positive integer~$n$. Writing 
$R=A/B$ where $A$ and $B$ are polynomials, it follows that $AB^{n
\v}=BA^{n\v}$ for all positive integers~$n$. Each side of the last 
equation is a polynomial in~$n$. Thus, $AB^{n\v}=BA^{n\v}$ 
identically. Hence $R^{n\v}=R$ for all $n\in\Q$ and the rational Galois 
space is closed under multiplication by scalars.

\Lemma[lem:three]  \hyperdef\lemthree{Lemma}{three}{} Let $R\in K(z_{1},\ldots,z_{k})$ be a rational 
function such that $\e_{j}\in\rgal(R)$. Then $R$ is free of $z_{j}$.
\LemmaStop

\Proof Since $R=R^{n\e_{j}}$ for all $n\in\Q$, it follows that 
$$R(z_{1},\ldots,z_{k})=R(z_{1},\ldots,z_{j}+n,\ldots,z_{k})$$ 
identically. The left side is free of $n$ and the right side is 
symmetric in $z_{j}$ and $n$, so the left side must be free of $z_{j}$.
\ProofStop

\Lemma[lem:four]  \hyperdef\lemfour{Lemma}{four}{} Let $R\in K(z_1,\ldots,z_k)$ be a rational function
and let $M$ be an $r\times k$ matrix over $\Q$. If the kernel of $M$ is
equal to the \hyperref\defAthree{rational Galois space} of $R$, then there exists a rational
function $\bar R\in K(z_1,\ldots,z_r)$ such that $R(\z)=\bar
R(M\z)$.
\LemmaStop

\Proof Let $A$ and $B$ be invertible $k\times k$ 
and $r\times r$ matrices
respectively such that 
the $r\times k$ matrix $AMB$ is of the form
 $$AMB=\left[\matrix I_{j,j} & {Z}_{j,k-j}\\
{Z}_{r-j,j} & {Z}_{r-j,k-j} \endmatrix\right]$$
where $j$ is the rank of $M$, $I_{j,j}$ is the $j\times j$ identity
matrix, and ${Z}_{\ell,m}$ is the $\ell\times m$ zero matrix. Since $j$
is the rank of $M$, it follows that
 $j\le r$. Let $R_1(\z)=R(B\z)$. Then $\rgal R_1=B^{-1}\rgal
R=B^{-1}\ker M=\ker MB=\ker AMB=\spn(\e_{j+1},\ldots,\e_k)$. By
Lemma~\hyperref\lemthree{\ref[lem:three]}, $R_1(\z)$ is free of $z_{j+1},\ldots,z_k$.
It follows that $R_1(\z)=\bar R_1(AMB\z)$, where $\bar R_1\in
K(z_1,\ldots, z_r)$ is defined by
$$\bar R_1(z_1,\ldots,z_r)=R_1(z_1,\ldots,z_k)=R_1(z_1,\ldots,z_j,0,\ldots,0).$$
Letting $\bar R(\z)=\bar R_1(A\z)$, we have $R_1(\z)=\bar R(MB\z)$. Hence $R(\z)=R_1(B^{-1}\z)=\bar R(M\z)$ as claimed.
\ProofStop

\Corollary[cor:oldlemmafour]  \hyperdef\coroldlemmafour{Corollary}{oldlemmafour}{} A nontrivial rational function $R\in 
K(z_{1},\ldots,z_{k})$ is \hyperref\defAtwo{simple} if and only if the dimension of $\rgal 
R$ is $k-1$.
\CorollaryStop

\Proof If $R$ is simple, then there exists $\v\in\Q^{k}$ and 
a univariate rational function $r\in K(\z)$ such that 
$R(\z)=r(\z\cdot\v)$. Clearly $\rgal R$ contains the space orthogonal to $\v$, and thus
$\dim\rgal R\ge k-1$. If the dimension were $k$, then $R$ would be
trivial; therefore, the dimension must be $k-1$.

Conversely, if the dimension of $\rgal(R)$ is $k-1$, there exists a 
$1\times k$ matrix $\v=[v_1,\ldots,v_k]$ with kernel equal to $\rgal R$. By Lemma~\hyperref\lemfour{\ref[lem:four]}, $R(\z)=\bar R(\v\cdot\z)=\bar R(v_1z_1+\cdots+v_kz_k)$, so $R$ is simple.
\ProofStop

\Lemma[lem:five]  \hyperdef\lemfive{Lemma}{five}{} Let $d$ and $A\in K[z_{1},\ldots,z_{k}]$ be 
polynomials. If $d\mid A$, then $\rgal d\supseteq\rgal A$.
\LemmaStop

\Proof Suppose the contrary. Then the quotient space $\rgal A/(\rgal 
A\cap\rgal d)$ is infinite. Let $S$ be a set of representatives of the 
cosets.

For any $s\in S$, $A^{-s}=A$, hence $d\mid A^{-s}$, hence $d^{s}\mid A$. 
Since $S$ is infinite and $A$ has only finitely many monic divisors, 
$d^{s_{1}}=cd^{s_{2}}$ for some $s_{1}$ and $s_{2}\in S$ and $c\in K$. 
Letting $s=s_{1}-s_{2}$, $d^{s}=cd$ and, by a corollary of 
Lemma~\hyperref\lemzero{\ref[lem:zero]}, $c=1$. But $d^{s_{1}}=d^{s_{2}}$, contradicting 
the definition of~$s$.
\ProofStop

\Corollary If $A$ and $B\in K[z_{1},\ldots,z_{k}]$ are polynomials 
such that $\rgal A=\rgal B=s$, then $\rgal AB=s$.
\CorollaryStop

\Proof By Lemma~\hyperref\lemfive{\ref[lem:five]}, $\rgal AB\subseteq s$. But clearly 
$\rgal AB\supseteq s$, so $\rgal AB=s$.
\ProofStop

\Lemma[lem:fiveprime]  \hyperdef\lemfiveprime{Lemma}{fiveprime}{} If $A$ and $B\in K[z_{1},\ldots,z_{k}]$ are 
relatively prime polynomials, then
$$\rgal\frac AB\subseteq\rgal A\cap\rgal B.$$
\LemmaStop

\Proof Suppose the contrary. Then the quotient space
$$\rgal\frac AB\bigg/(\rgal\frac AB\cap\rgal A\cap\rgal B)$$
is infinite. Let $S$ be a set of representatives of the cosets, and 
let $s_{1}$ and $s_{2}\in S$.

Since $(A/B)^{s_{1}}=(A/B)^{s_{2}}$, letting $s=s_{1}-s_{2}$ it 
follows that $(A^{s}/B^{s})=(A/B)$. Hence $AB^{s}=BA^{s}$. Since $A$ 
and $B$ are relatively prime, $A\mid A^{s}$. Similarly, $A^{s}\mid 
A$. Hence $A=cA^{s}$, and hence, by corollary~\hyperref\corsecond{\ref[cor:second]} of 
Lemma~\hyperref\lemzero{\ref[lem:zero]}, $c=1$. Hence $A=A^{s}$. Similarly, $B=B^{s}$. 
Hence $s_{1}-s_{2}=s\in\rgal(A/B)\cap\rgal A\cap\rgal B$, contradicting 
the definition of $s_1$ and $s_2$.
\ProofStop

\Lemma[lem:six]  \hyperdef\lemsix{Lemma}{six}{} Every rational function $R\in K(z_{1},\ldots,z_{k})$ 
can be written as a product
$$R=g\prod_{s\in S}\frac{A_{s}}{B_{s}},$$
where $S$ is the collection of all proper subspaces of $\Q^{k}$, 
$g\in K$, and, for all $s\in S$, $A_{s}$ and $B_{s}\in 
K[z_{1},\ldots,z_{k}]$ are relatively prime \hyperref\defAone{monic} polynomials such 
that if $d$ is a nontrivial divisor of $A_{s}$ or $B_{s}$, then 
$\rgal(d)=s$. This expression is unique.
\LemmaStop

Of course, $A_{s}=B_{s}=1$ for all but a finite number of $s\in S$.

\Proof We first show that such a factorization exists. Let $R=gA/B$,
where $A$ and $B$ are relatively prime monic polynomials and $g\in
K$. Write $A$ and $B$ as products of nontrivial irreducible monic
factors
$$A=a_1a_2\cdots a_m\text{ and }B=b_1\cdots b_n,\ m,n\ge0.$$

For all $s\in S$ let $A_s$ be the product of all $a_i$ such that
$\rgal(a_i)=s$, with the understanding that empty products
are~$1$. Similarly define $B_s$. Clearly $A=\prod_{s\in S}A_s$ and
$B=\prod_{s\in S}B_s$. Hence 
$$R=g\prod_{s\in S}\frac{A_s}{B_s}$$
and $A_s$ and $B_s$ are relatively prime.

Let $d$ be a nontrivial monic divisor of $A_s$ or $B_s$. Then $d$ can
be expressed as a product of a subset of the $a_i$ for which $\rgal
a_i=s$ and the $b_i$ for which $\rgal b_i=s$. Hence, by the corollary
of Lemma~\hyperref\lemfive{\ref[lem:five]}, $\rgal d=s$.

We show that the factorization is unique. Let
$$R=g\prod_{s\in S}\frac{A_s}{B_s}\text{ and }R=h\prod_{s\in
S}\frac{C_s}{D_s}\leqno(1)$$
be two factorizations satisfying the conditions of the lemma. We will
show that $g=h$ and $A_s=C_s$ and $B_s=D_s$ for all $s\in
S$. By~$(1)$, 
$$g\prod A_s\prod D_s=h\prod B_s\prod C_s.\leqno(2)$$
For any $t\in S$, $A_t$ is relatively prime to $\prod_{s\ne
t}B_s\prod_{s\ne t}C_s$ since any nontrivial irreducible divisor
$d$ of the former has $\rgal(d)=s$ and any nontrivial divisor $d$
of the latter has $\rgal(d)\ne s$. Since $A_t$ and $B_t$ are
relatively prime by assumption, it follows that $A_t\mid
C_t$. Similarly $C_t\mid A_t$. Hence $C_t=A_t$. Similarly
$B_t=D_t$. It follows that $g=h$.
\ProofStop

\hyperdef\chapteRiiSECvi{ChapterSection}{chapteRiiSECvi}{}
\Section Fixed factors

The complementary idea to the rational Galois space is the fixed factor.

\Definition[def:A4]  \hyperdef\defAfour{Definition}{A4}{}
Using Lemma~\hyperref\lemsix{\ref[lem:six]}, we define the \defword{fixed
factor} $\fix_s(R)$ of a rational function $R\in K(z_1,\ldots,z_k)$
for a subspace $s$ of $\Q^k$.
Let $S$ be the set of all proper subspaces of $\Q^k$.
Let $R=g\prod_{s\in S}(A_s/B_s)$ be the unique expression guaranteed
by Lemma~\hyperref\lemsix{\ref[lem:six]}. 
Define
$$
\fix_s(R)=
\cases
\frac{A_s}{B_s}&\text{ for all }s\in S\\
g&\text{ for }s = \Q^k.
\endcases
$$
\DefinitionStop

\Lemma[lem:seven]  \hyperdef\lemseven{Lemma}{seven}{} Let $R\in K(z_1,\ldots,z_k)$ be a rational function
and let $s$ be a subspace of $\Q^k$. Then
$$\rgal\fix_sR=s$$
unless $\fix_sR=1$.
\LemmaStop

\Proof If $\fix_sR\ne1$ then either $\fix_sR$ has a nontrivial divisor
or $\fix_sR=c$ for some $c\in K$, $c\ne1$. In the first case,
$\rgal\fix_sR\subseteq\rgal d=s$ by Lemma~\hyperref\lemfive{\ref[lem:five]}. But clearly
$\rgal\fix_sR\supseteq s$, so $\rgal\fix_sR=s$. In the second case,
$s=\Q^k$ and $\rgal c=\Q^k$.
\ProofStop

\Lemma[lem:nine]  \hyperdef\lemnine{Lemma}{nine}{} For any nonzero rational functions $R_1$ and $R_2\in
K(z_1,\ldots,z_k)$, any subspace $s$ of $\Q^k$, and any $\v\in\Q^k$
\Enumerate
\item[nine:one] \hyperdef\nineone{item}{one}{} $\fix_sR_1R_2=\fix_sR_1\fix_sR_2$
\item[nine:two] \hyperdef\ninetwo{item}{two}{} $\ds{\fix_s\frac1{R_1}=\frac1{\fix_sR_1}}$
\item[nine:three] \hyperdef\ninethree{item}{three}{} $\fix_sR_1^{\v}=(\fix_sR_1)^{\v}$
\EnumerateStop
\LemmaStop

\Proof Let $S$ be the set of proper subspaces of $\Q^k$.
Let $R_3=R_1R_2$, $R_4=1/R_1$, and $R_5=R_1^{\v}$. For
$i=1,2,3,4$, and $5$ let 
$$R_i=g_i\prod_{s\in S}\frac{A_{i,s}}{B_{i,s}}$$
be the unique expression guaranteed by Lemma~\hyperref\lemsix{\ref[lem:six]}.

(\hyperref\nineone{\ref[nine:one]}): Since $R_3=R_1R_2$, it follows that
$$g_3\prod_{s\in S}\frac{A_{3,s}}{B_{3,s}}=g_1g_2\prod_{s\in
S}\frac{A_{1,s}A_{2,s}}{B_{1,s}B_{2,s}}.$$
Let $C_s$ and $D_s$ be relatively prime polynomials such that
$$\frac{C_s}{D_s}=\frac{A_{1,s}A_{2,s}}{B_{1,s}B_{2,s}}.$$
Since $C_s\mid A_{1,s}A_{2,s}$ and every nontrivial divisor of
$A_{1,s}$ or $A_{2,s}$ has $\rgal d=s$, it follows by the corollary of
Lemma~\hyperref\lemfive{\ref[lem:five]} that every nontrivial divisor $d$ of $C_s$ has
$\rgal d=s$. Similarly, every nontrivial divisor $d$ of $D_s$ has $\rgal
d=s$. It follows that 
$$R_3=g_1g_2\prod_{s\in S}\frac{C_s}{D_s}$$
is the unique expression guaranteed by Lemma~\hyperref\lemsix{\ref[lem:six]}, hence
$$\frac{A_{3,s}}{B_{3,s}}=\frac{C_s}{D_s}=\frac{A_{1,s}}{B_{1,s}}
\cdot\frac{A_{2,s}}{B_{2,s}}$$
for all $s\in S$. Hence $\fix_sR_3=\fix_sR_1\fix_sR_2$ for all $s\in
S$. Clearly $g_3=g_1g_2$ since the polynomials in~(\hyperref\nineone{\ref[nine:one]}) are
monic, so $\fix_sR_3=\fix_sR_1\fix_sR_2$ for $s=\Q^k$.

(\hyperref\ninetwo{\ref[nine:two]}): We have
$$g_4\prod_{s\in
S}\frac{A_{4,s}}{B_{4,s}}=R_4=\frac1{R_1}=\frac1{g_1}\prod_{s\in
S}\frac{B_{1,s}}{A_{1,s}}.$$
It follows immediately that the factorization
$$R_4=\frac1{g_1}\prod_{s\in S}\frac{B_{1,s}}{A_{1,s}}$$
satisfies the conditions of the lemma, hence $g_4=1/g_1$ and 
$$\frac{A_{4,s}}{B_{4,s}}=\frac{B_{1,s}}{A_{1,s}}.$$
Hence $\fix_sR_4=1/(\fix_sR_1)$ for all $s\in S$ and for $s=\Q^k$.

(\hyperref\ninethree{\ref[nine:three]}): We have
$$g_5\prod_{s\in S}\frac{A_{5,s}}{B_{5,s}}=R_5=R_1^{\v}=g_1^{
\v}\prod_{s\in S}\frac{A_{1,s}^{\v}}{B_{1,s}^{\v}}.$$
Since $\rgal d^{\v}=\rgal d$ for any polynomial $d$ and any $
\v\in\Q^k$, 
$$R_5=g_1^{\v}\prod_{s\in S}\frac{A_{1,s}^{\v}}{B_{1,s}^{
\v}}$$ 
satisfies the conditions of the lemma. Hence
$$g_5=g_1^{\v}\text{ and
}\frac{A_{5,s}}{B_{5,s}}=\frac{A_{1,s}^{\v}}{B_{1,s}^{\v}}$$
for all $s\in S$. Hence $\fix_sR_5=(\fix_sR_1)^{\v}$ for all $s\in
S$ and for $s=\Q^k$.
\ProofStop

\Lemma[lem:ten]  \hyperdef\lemten{Lemma}{ten}{} Let $R_1,\ldots,R_k\in K(z_1,\ldots,z_k)$ be rational
functions satisfying the relation
$$R_iR_j^{\e_i}=R_jR_i^{\e_j}$$
for all $i,j\in\{1,\ldots,k\}$. For $i=1,\ldots,k$ and all subspaces
$s$ of $\Q^k$ define $R_{i,s}=\fix_s(R_i)$. Then for all subspaces $s$
of $\Q^k$ and all $i,j\in\{1,\ldots,k\}$,
$$R_{i,s}R_{j,s}^{\e_i}=R_{j,s}R_{i,s}^{\e_j}.$$
\LemmaStop

\Proof By Lemma~\hyperref\lemnine{\ref[lem:nine]},
$$\align
\fix_sR_i(\fix_sR_j)^{\e_i}
&=\fix_sR_iR_j^{\e_i}\\
&=\fix_sR_jR_i^{\e_j}\\
&=\fix_sR_j(\fix_sR_i)^{\e_j}.
\endalign$$
\ProofStop

\Lemma[lem:eleven]  \hyperdef\lemeleven{Lemma}{eleven}{} Let $R_1,\ldots,R_k\in K(z_1,\ldots,z_k)$ be
rational functions satisfying the relation
$$R_iR_j^{\e_i}=R_jR_i^{\e_j}$$
for all $i,j\in\{1,\ldots,k\}$. Let $s$ be a proper subspace of $\Q^k$
such that $\e_i\in s$. Then $\fix_sR_i=1$.
\LemmaStop

\Proof By Lemma~\hyperref\lemten{\ref[lem:ten]}, for $j\in\{1,\ldots,k\}$,
$$\align
\frac{\fix_sR_i}{(\fix_sR_i)^{\e_j}}
&=\frac{\fix_sR_j}{(\fix_sR_j)^{\e_i}}\\
&=\frac{\fix_sR_j}{\fix_sR_j}\\
&=1.
\endalign$$
Hence $\e_j\in\rgal\fix_sR_i$. By Lemma~\hyperref\lemseven{\ref[lem:seven]}, either
$\fix_sR_i=1$ or $\rgal\fix_sR_i=s$. In the first case we are done. In
the second case $\e_j\in s$ for all $j\in\{1,\ldots,k\}$. Hence
$s=\Q^k$, contradicting the assumption that $s$ is a proper subspace.
\ProofStop
\secno=6

\hyperdef\chapteRiiSECvii{ChapterSection}{chapteRiiSECvii}{}
\Section Proof of Lemma~\ref[lem:two] for $k>2$

Now we are in a position to prove the case $k>2$ of Lemma~\hyperref\lemtwo{\ref[lem:two]}. 
We proceed by induction. Assume the case of $k-1$ variables is proved. 
Let
$$R_{1}=\frac{A_{1}}{B_{1}}\frac{C_{1}}{C_{1}^{
\e_{1}}}\frac{D_{1}^{\e_{1}}}{D_{1}}$$
as in Lemma~\hyperref\lemone{\ref[lem:one]}. Let 
$K_{i,j}=K(\{z_{1},\ldots,z_{k}\}\setminus\{z_{i},z_{j}\})$ and let 
$\Q_{i,j}$ be the subspace of $\Q^{k}$ generated by $\e_{i}$ and 
$\e_{j}$. Let $r_{1}=A_{1}/B_{1}$. 

Let $i\in\{2,\ldots,k\}$.
Applying the strong version
of the two-variable case of Lemma~\hyperref\lemtwo{\ref[lem:two]} to $R_{1}$ and 
$R_{i}$ over the field $K_{1,i}$, it follows that we can write
$$R_{i}=\frac{A_{i}}{B_{i}}\frac{C_{1}}{C_{1}^{
\e_{i}}}\frac{D_{1}^{\e_{i}}}{D_{1}},$$
where the irreducible divisors of $A_{1}$, $A_{i}$, $B_{1}$, and 
$B_{i}$ are all simple over $K_{1,i}$. 
The point of using the strong version of
the two-variable case is that the same
$C_1$ and $D_1$ can be used for all 
$i\in\{2,\ldots,k\}$.

Let $d$ be a nontrivial 
irreducible divisor of $A_{1}$ or $B_{1}$. The subspace 
$\rgal(d)\cap\Q_{1,j}$ of $\Q_{1,j}$ is isomorphic to the subspace 
$\rgal(d,(z_1,z_j),K_{1,j})$ of $\Q^{2}$.
Hence $\rgal(d)\cap\Q_{1,j}$ is a one-dimensional subspace 
of $\Q_{1,j}$ by Lemma~\hyperref\lemfour{\ref[lem:four]}. Let $s=\rgal(d)$. Let $r_i=A_i/B_i$ for $i\in\{2,\ldots,k\}$. It's easily 
verified that $r_{i}$ satisfies
$$r_{i}r_{j}^{\e_{i}}=r_{j}r_{i}^{\e_{j}}$$
for $i,j\in\{1,\ldots,k\}$, hence, by Lemma~\hyperref\lemeleven{\ref[lem:eleven]}, if $
\e_{1}\in s$ then $\fix_{s}R_{1}=1$. But $\fix_{s}R_{1}=1$ implies 
$\fix_{s}A_{1}=\fix_{s}B_{1}=1$, which implies $d=1$. Since $d$ is 
nontrivial, $\e_{1}\notin s$.

Let $\v_{i}$ be a nonzero vector in $\rgal d\cap\Q_{1,i}$. Since 
$\e_{1}\notin s$, it follows that $\e_{i}\cdot\v_{i}\ne0$. 
Let $ \vec t=\sum_{i=2}^{k}c_{i}\v_{i}$.
It is easily seen that the vectors 
$\v_{2},\ldots,\v_{k}$ are linearly independent:
if $c_{j}\ne0$, then $
\e_{j}\cdot\vec t=c_{j}(\e_{j}\cdot\v_{j})$ is nonzero, hence 
$\vec t$ is nonzero.

It follows that the dimension of $\rgal(d)$ is at least $k-1$.  
By Lemma~\hyperref\lemfour{\ref[lem:four]}, $d$ is simple over $K$. We have shown all 
the nontrivial irreducible divisors of $A_{1}$ and $B_{1}$ are simple 
over $K$.

Define $\bar R_{i}$ and $\tilde R_{i}$ by
$$\bar R_{i}=\prod\fix_{s}r_{i}$$
and
$$\tilde R_{i}=\mathop{{\prod}'}\fix_{s}r_{i}$$
where the first product is taken over all subspaces $s$ of $\Q^{k}$ 
such that $\e_{1}\notin s$, and the second is taken over all 
subspaces such that $\e_{1}\in s$. Hence $r_{i}=\bar R_{i}\tilde 
R_{i}$. It follows from Lemma~\hyperref\lemten{\ref[lem:ten]} that
$$\bar R_{i}\bar R_{j}^{\e_{i}}=\bar R_{j}\bar R_{i}^{
\e_{j}}$$
and
$$\tilde R_{i}\tilde R_{j}^{\e_{i}}=\tilde R_{j}\tilde R_{i}^{
\e_{j}}$$
for all $i,j\in\{1,\ldots,k\}$.

Let $\bar A_{i}$ and $\bar B_{i}$ be relatively prime polynomials such 
that $\bar R_{i}=\bar A_{i}/\bar B_{i}$. We claim that the irreducible 
divisors of $\bar A_{i}$ and $\bar B_{i}$ are simple. By 
Lemma~\hyperref\lemeleven{\ref[lem:eleven]}, $\tilde R_{1}=1$. Hence $\bar R_{1}=r_{1}$, 
and hence the irreducible divisors of $\bar A_{1}=A_{1}$ and $\bar 
B_{1}=B_{1}$ are simple. Let $d$ be an irreducible divisor of $\bar 
A_{i}$ or $\bar B_{i}$ for $i\in\{2,\ldots,k\}$, and let $s=\rgal(d)$. 
If the dimension of $s$ is less than $k-1$, then $\fix_{s}\bar R_{1}=1$ 
since all the irreducible divisors of $\bar A_{1}$ and $\bar B_{1}$ 
are simple and, by Lemma~\hyperref\lemfour{\ref[lem:four]}, have rational Galois spaces of 
dimension $k$ or $k-1$. By Lemma~\hyperref\lemten{\ref[lem:ten]},
$$\frac{\fix_{s}\bar R_{i}}{\fix_{s}\bar R_{i}^{
\e_{1}}}=\frac{\fix_{s}\bar R_{1}}{\fix_{s}\bar R_{1}^{\e_{i}}}=1,$$
so $\e_{1}\in\rgal(\fix_{s}\bar R_{i})$. Hence $\e_{1}\in s$ 
by Lemma~\hyperref\lemseven{\ref[lem:seven]}, which contradicts the definition of $\bar 
R_{i}$, so the dimension of $\rgal d$ is $k-1$ or $k$ and $d$ is 
simple by Lemma~\hyperref\lemfour{\ref[lem:four]}.

By Lemma~\hyperref\lemthree{\ref[lem:three]}, $\tilde R_{i}$ is free of $z_{i}$ for all 
$i\in\{1,\ldots,k\}$. Inductively applying the $k-1$ variable case of 
Lemma~\hyperref\lemtwo{\ref[lem:two]} to $\tilde R_{2},\ldots,\tilde R_{k}\in 
K(z_{2},\ldots,z_{k})$, there exist $\tilde C$ and $\tilde D$ such 
that
$$\tilde R_{i}=\frac{\tilde A_{i}}{\tilde B_{i}}\frac{\tilde C}{\tilde 
C^{\e_{i}}}\frac{\tilde D^{\e_{i}}}{\tilde D}\leqno(1)$$
for $i\in\{2,\ldots,k\}$, and the irreducible divisors of $\tilde 
A_{i}$ and $\tilde B_{i}$ are simple over $K$. Let $\tilde 
A_{1}=\tilde B_{1}=1$. Then $(1)$ is true for $i=1$.

Letting $C=C_{1}\tilde C$, $D=D_{1}\tilde D$, $a_{i}=\bar A_{i}\tilde 
A_{i}$, and $b_{i}=\bar B_{i}\tilde B_{i}$,
$$R_{i}=\frac{a_{i}}{b_{i}}\frac{C}{C^{\e_{i}}}\frac{D^{
\e_{i}}}D$$
where the irreducible divisors of $a_{i}$ and $b_{i}$ are all simple.
This completes the proof of Lemma~\hyperref\lemtwo{\ref[lem:two]}.
\ProofStop

\secno=7
\hyperdef\chapteRiiSECviii{ChapterSection}{chapteRiiSECviii}{}
\Section The multiplicative structure of $R_i$


\Lemma[lem:thirteen]  \hyperdef\lemthirteen{Lemma}{thirteen}{} Let $R_1,\ldots,R_k\in K(z_1,\ldots,z_k)$ be \hyperref\defAtwo{simple} rational functions with the same \hyperref\defAthree{rational Galois space} such that
$$R_iR_j^{\e_i}=R_jR_i^{\e_j}\leqno(1)$$
for all $i,j\in\{1,\ldots,k\}$. Then there exist $\v\in\Z^k$, a univariate rational function $t\in K(z)$, and $c_1,\ldots,c_k\in K$ such that
$$R_i(z_1,\ldots,z_k)=c_i\gp j0{v_i}t(\v\cdot\z+j)$$
for $i\in\{1,\ldots,k\}$.
\LemmaStop


\Proof Let $s=\rgal R_i$. The case $s=\Q^k$ is trivial: if $s=\Q^k$, then $R_i\in K$ for all $i\in\{1,\ldots,k\}$, so we may take $c_i=R_i$, $t=1$, and $\v=\vec 0$.

We consider the case $s\ne\Q^k$. By the corollary of Lemma~\hyperref\lemfour{\ref[lem:four]} the dimension of $s$ is $k-1$. Hence, there exists a vector $\v\in\Z^k$ with $\gcd(\v)=1$ such that the kernel of the $1\times k$ matrix $\v$ is $s$. By Lemma~\hyperref\lemfour{\ref[lem:four]}, for all $i\in\{1,\ldots,k\}$ there exist univariate $r_i\in K(z)$ such that $R_i(\z)=r_i(\v\cdot\z)$.

Since $\gcd(\v)=1$, there exists $\w\in\Z^k$ such that $\w\cdot\v=w_1v_1+\cdots w_kv_k=1$. 
For any univariate rational function $r \in K(z)$
and any
$n\in \Z$,
the rational 
function $r^{(n)} \in K(z)$ is defined by
$r^{(n)}(z)=r(z+n)$.
Define 
$$t=\gp i0{w_1}r_1^{(v_1i)}
\gp i0{w_2}r_2^{(v_1w_1+v_2i)}\cdots
\gp i0{w_k}r_k^{(v_1w_1+\cdots v_{k-1}w_{k-1}+v_ki)}.$$
We claim that $R_i(z_1,\ldots,z_k)=\gp j0{v_i}t^{(j)}(\v\cdot\z)$.
We first show that $r_i/r_i^{(1)}=t/t^{(v_i)}$. Since
$$\align
R_i^{\e_j}(z_1,\ldots,z_k)
&=(r(\v\cdot\z))^{\e_j}\\
&=r(\v\cdot\z+\v\cdot\e_j)\\
&=r(\v\cdot\z+v_j)\\
&=r^{(v_j)}(\v\cdot\z),
\endalign$$
it follows from $(1)$ that
$$\frac{r_i}{r_i^{(v_j)}}=\frac{r_j}{r_j^{(v_i)}}$$
for all $i,j\in\{1,\ldots,k\}$. Hence
$$\align
\frac t{t^{(v_j)}}
&=\gp i0{w_1}\left(\frac{r_1}{r_1^{(v_j)}}\right)^{(v_1i)}
\gp i0{w_2}\left(\frac{r_2}{r_2^{(v_j)}}\right)^{(v_1w_1+v_2i)}\cdots\\
&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\cdots
\gp i0{w_k}\left(\frac{r_k}{r_k^{(v_j)}}\right)^{(v_1w_1+
\cdots+v_{k-1}w_{k-1}+v_ki)}\\
&=\gp i0{w_1}\left(\frac{r_j}{r_j^{(v_1)}}\right)^{(v_1i)}
\gp i0{w_2}\left(\frac{r_j}{r_j^{(v_2)}}\right)^{(v_1w_1+v_2i)}\cdots\\
&\qquad\qquad\qquad\qquad\qquad\qquad\qquad\cdots
\gp i0{w_k}\left(\frac{r_j}{r_j^{(v_k)}}\right)^{(v_1w_1+
\cdots+v_{k-1}w_{k-1}+v_ki)}\\
&=\frac{r_j^{(0)}}{r_j^{(v_1w_1)}}\cdot
\frac{r_j^{(v_1w_1)}}{r_j^{(v_1w_1+v_2w_2)}}\cdots
\frac{r_j^{(v_1w_1+\cdots+v_{k-1}w_{k-1})}}{r_j^{(v_1w_1+\cdots+v_kw_k)}}\\
&=\frac{r_j}{r_j^{(v_1w_1+\cdots+v_kw_k)}}\\
&=\frac{r_j}{r_j^{(1)}}
\endalign$$
since $v_1w_1+\cdots+v_kw_k=1$.

We show that $r_j=c_j\gp i0{v_j}t^{(i)}$. Since $r_j/r_j^{(1)}=t/t^{(v_j)}$, letting $T_j=\gp i0{v_j}t^{(i)}$ it follows that $r_j/r_j^{(1)}=T_j/T_j^{(1)}$; hence $(r_j/T_j)=(r_j/T_j)^{(1)}$. It follows by Lemma~\hyperref\lemthree{\ref[lem:three]} that $r_j/T_j=c_j$ for some $c_j\in K$. Thus, $R_j(z_1,\ldots,z_k)=r_j(\v\cdot\z)=c_i\gp j0{v_j}t^{(j)}(\v\cdot\z)=c_i\gp j0{v_j}t(\v\cdot\z+j)$.
\ProofStop

Lemma~\hyperref\lemfourteen{\ref[lem:fourteen]} summarizes the results of this section thus far.

\Lemma[lem:fourteen]  \hyperdef\lemfourteen{Lemma}{fourteen}{} Let $R_1,\ldots,R_k\in K(z_1,\ldots,z_k)$ be rational functions satisfying the relation
$$R_iR_j^{\e_i}=R_jR_i^{\e_j}$$
for all $i,j\in\{1,\ldots,k\}$. For each subspace $s$ of $\Q^k$ let $R_{i,s}=\fix_sR_i$.
\Enumerate
\item[fourteen:one] \hyperdef\fourteenone{item}{one}{} If the dimension of $s$ is less than $k-1$, then there exists a rational function $r\in K(z_1,\ldots,z_k)$ such that for all $i\in\{1,\ldots,k\}$, 
$$R_{i,s}=r/r^{\e_i}.$$
\item[fourteen:two] \hyperdef\fourteentwo{item}{two}{} If the dimension of $s$ is $k-1$ then there exists a univariate rational function $t\in K(z)$, $c_1,\ldots,c_k\in K$,
 and a vector $\v\in\Z^k$ such that for all $i\in\{1,\ldots,k\}$
$$R_{i,s}=c_i\gp j0{\v_i}t(\v\cdot\z+j).$$
\item[fourteen:three] \hyperdef\fourteenthree{item}{three}{} If the dimension of $s$ is $k$ then $R_{i,s}\in K$ for all $i\in\{1,\ldots,k\}$.
\item[fourteen:four] \hyperdef\fourteenfour{item}{four}{} $R_i=\prod_sR_{i,s}$ for all $i\in\{1,\ldots,k\}$, where the product is taken over all subspaces $s$ of $\Q^k$.
\EnumerateStop
\LemmaStop

\Proof Write
$$R_i=\frac C{C^{\e_i}}\frac{D^{\e_i}}D\frac{A_i}{B_i}$$
as in Lemma~\hyperref\lemtwo{\ref[lem:two]} and let $C_s=\fix_sC$, $D_s=\fix_sD$, $A_{i,s}=\fix_sA_i$, and $B_{i,s}=\fix_sB_i$. By Lemma~\hyperref\lemnine{\ref[lem:nine]}
$$R_{i,s}=\frac{C_s}{C_s^{\e_i}}\frac{D_s^{\e_i}}{D_s}\frac{A_{i,s}}{B_{i,s}}.$$

(1) If the dimension of $s$ is less than $k-1$, then $A_{i,s}=B_{i,s}=1$ since the irreducible divisors of $A_i$ and $B_i$ are simple. Hence $R_{i,s}=r/r^{\e_i}$ where $r=C_s/D_s$.

(2) If the dimension of $s$ is $k-1$ then $R_{1,s},\ldots,R_{k,s}$ are simple by the corollary of Lemma~\hyperref\lemfour{\ref[lem:four]}. By Lemma~\hyperref\lemten{\ref[lem:ten]}
$$R_{i,s}R_{j,s}^{\e_i}=R_{j,s}R_{i,s}^{\e_j},$$
hence, by Lemma~\hyperref\lemthirteen{\ref[lem:thirteen]}, there exist $c_1,\ldots,c_k\in K$, $\v\in\Z^k$, and $t\in K(z)$ such that
$$R_{i,s}=c_i\gp j0{v_i}t(\v\cdot\z+j)$$
for $i\in\{1,\ldots,k\}$. 

(3) By Lemma~\hyperref\lemthree{\ref[lem:three]}, $r_{i,s}$ is free of $z_1,\ldots,z_k$, and thus constant.

(4) This is immediate from Lemma~\hyperref\lemsix{\ref[lem:six]}.
\ProofStop

\Lemma[lem:fifteen]  \hyperdef\lemfifteen{Lemma}{fifteen}{} Let $R_1,\ldots,R_k\in K(z_1,\ldots,z_k)$ be rational functions satisfying the relation
$$R_iR_j^{\e_i}=R_jR_i^{\e_j}$$
for all $i$ and $j\in\{1,\ldots,k\}$. There exist a rational function $r\in K(z_1,\ldots,z_k)$, constants $c_1,\ldots,c_k\in K$, finitely many vectors $\v_1,\ldots,\v_m\in\Z^k$, and corresponding univariate rational functions $t_1,\ldots,t_m\in K(z)$ such that for all $i\in\{1,\ldots,k\}$,
$$R_i(\z)=c_i\frac{r(\z)}{r^{\e_i}(\z)}\prod_{\ell=1}^m\gp j0{v_{\ell,i}}t_\ell(\v_{\ell}\cdot\z+j).$$
\LemmaStop

\Proof For each subspace of $s$ of $\Q^k$ and $i\in\{1,\ldots,k\}$ let $R_{i,s}=\fix_sR_i$. Let $s_1,\ldots,s_m$ be the subspaces $s$ of $\Q^k$ of dimension $k-1$ such that $R_{i,s}\ne1$ for some $i\in\{1,\ldots,k\}$. Let $t_1,\ldots,t_n$ be the subspaces of $\Q^k$ of dimension less than $k-1$ such that $R_{i,s}\ne1$ for some $i\in\{1,\ldots,k\}$.

By Lemma~\hyperref\lemfourteen{\ref[lem:fourteen]} (2), for each $\ell$, $1\le\ell\le m$, $R_{i,s_\ell}=\gp j0{v_{\ell,i}}t_\ell(\v_\ell\cdot\z+j)$ for some $\v_\ell\in\Z^k$ and $t_\ell\in K(z)$. By Lemma~\hyperref\lemfourteen{\ref[lem:fourteen]} (1), for each $p$, $1\le p\le n$, there exists $r_p\in K(z_1,\ldots,z_k)$ such that for $i\in\{1,\ldots,k\}$, $R_{i,t_p}=r_p/r_p^{\e_i}$. Let $r=\prod_{p=1}^nr_p$. 
Let $c_i=R_{i,\Q^k}$ for $i\in\{1,\ldots,k\}$. By Lemma~\hyperref\lemfourteen{\ref[lem:fourteen]} (4),
$$\align
R_{i,s}
&=c_iR_{i,t_1}\cdots R_{i,t_n}R_{i,s_1}\cdots R_{i,s_m}\\
&=c_i\frac{r_{t_1}}{r_{t_1}^{\e_i}}\cdots\frac{r_{t_n}}{r_{t_n}^{\e_i}}\prod_{\ell=1}^mR_{i,s\ell}\\
&=c_i\frac r{r^{\e_i}}\prod_{\ell=1}^m\gp j0{v_{\ell,i}}t_\ell(\v_\ell\cdot\z+j).
\endalign$$
\ProofStop



\Theorem[thm:15a]  \hyperdef\thmfifteena{Theorem}{15a}{} \hyperref\oresato{\OreSato}
Let $R_1,\ldots,R_k\in K(\z)$ be rational functions such that
$$R_iR_j^{\e_i}=R_jR_i^{\e_j}$$
for all $i,j\in\{1,\ldots,k\}$. Then there exist polynomials $C$ and $D\in K[\z]$, a finite set $V\subset\Z^k$, and univariate polynomials $a_{\v}$ and $b_{\v}\in K[z]$ for each $\v\in V$ such that for all $i\in\{1,\ldots,k\}$,
$$R_i(\z)=\frac{C(\z+\e_i)}{C(\z)}\frac{D(\z)}{D(\z+\e_i)}\prod_{\v\in V}\gp j0{\v_i}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)}.$$
\TheoremStop

\Proof The $c_i$ from Lemma~\hyperref\lemfifteen{\ref[lem:fifteen]} can be absorbed into the product by noting that
$$\gp j0{\e_i\cdot\w}c_i=\cases
c_i&\text{if }\w=\e_i,\\
1&\text{if }\w\in\{\e_1,\ldots,\e_k\}\setminus\{\e_i\}.
\endcases$$
The rest is just a change of notation.
\ProofStop

\Corollary[cor:16]  \hyperdef\corsixteen{Corollary}{16}{} For all $\w\in\Z^k$, let $R_{\w}\in K(\z)$ be rational functions such that
$$ R_{\v +\w}=R_{\v}R_{\w}^{\v}$$
for all $\w$ and $\v\in\Z^k$. Then there exist polynomials $C$ and $D\in K[\z]$, a finite set $V\subseteq\Z^k$, and univariate polynomials $a_{\v}$ and $b_{\v}\in K[z]$ for each $\v\in V$ such that for all $\w\in\Z^k$,
$$R_{\w}(\z)=\frac{C(\z+\w)}{C(\z)}\frac{D(\z)}{D(\z+\w)}\prod_{\v\in V}\gp j0{\v\cdot\w}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)}.$$
\CorollaryStop


\Proof
By symmetry,
$R_{\v +\w}=R_{\w}R_{\v}^{\w}$,
hence,
$R_{\w}R_{\v}^{\w}=R_{\v}R_{\w}^{\v}$.
Letting $R_i=R_{\e_i}$ for $i\in\{1,\ldots,k\}$, we have $R_iR_j^{\e_i}=R_jR_i^{\e_j}$. It follows by Theorem~\hyperref\thmfifteena{\ref[thm:15a]} that there exist polynomials $C,D\in K[\z]$, a finite set $V\in\Z$, and univariate polynomials $a_{\v}$ and $b_{\v}$ for $v\in V$ such that
$$R_{\w}(\z)=\frac{C(\z+\w)}{C(\z)}\frac{D(\z)}{D(\z+\w)}\prod_{\v\in V}\gp j0{\v\cdot\w}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)}$$
for $\w\in\{\e_1,\ldots,\e_k\}$. Let $\bar R_{\w}(\z)$ be the right side of the last equation. Thus $R_{\w}=\bar R_{\w}$ for $\w\in\{\e_1,\ldots,\e_k\}$.

We show that $R_{\w}=\bar R_{\w}$ for all $\w\in\Z^k$. It's clear that $R_{\vec 0}=1$ and $\bar R_{\vec 0}=1$ so $R_{\vec 0}=\bar R_{\vec 0}$. We show that $\bar R_{\u+\w}=\bar R_{\u}\bar R_{\w}^{\u}$.

$$\align
\bar R_{\u}\bar R_{\w}^{\u}
&=\vec c^{\u}\vec c^{\w}\frac{C^{\u}}C\frac D{D^{\u}}\left(\frac{C^{\w}}C\frac D{D^{\w}}\right)^{\u}\prod_{\v\in V}\gp j0{\v\cdot\u}\frac{a_{\v}(\v\cdot\z+j)}{b_{\v}(\v\cdot\z+j)}\left(\gp j0{\v\cdot\w}\frac{a_{\v}(\v\cdot\z+j)}{b_{\v}(\v\cdot\z+j)}\right)^{\u}\\
&=\vec c^{\u+\w}\frac{C^{\u}}C\frac D{D^{\u}}\frac{C^{\w+\u}}{C^{\u}}\frac{D^{\u}}{D^{\w+\u}}\prod_{\v\in V}\gp j0{\v\cdot\u}\frac{a_{\v}(\v\cdot\z+j)}{b_{\v}(\v\cdot\z+j)}\gp j0{\v\cdot\w}\frac{a_{\v}(\v\cdot(\z+\u)+j)}{b_{\v}(\v\cdot(\z+\u)+j)}\\
&=\vec c^{\u+\w}\frac{C^{\u+\w}}C\frac D{D^{\u+\w}}\prod_{\v\in V}\gp j0{\v\cdot\u}\frac{a_{\v}(\v\cdot\z+j)}{b_{\v}(\v\cdot\z+j)}\gp j{\v\cdot\u}{\v\cdot\w+\v\cdot\u}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)}\\
&=\vec c^{\u+\w}\frac{C^{\u+\w}}C\frac D{D^{\u+\w}}\prod_{\v\in V}\gp j0{\v\cdot(\u+\w)}\frac{a_{\v}(\z\cdot\v+j)}{b_{\v}(\z\cdot\v+j)}\\
&=\bar R_{\u+\w}.
\endalign$$
Substituting $\u-\w$ for $\u$ in $R_{\u+\w}=R_{\u}R_{\w}^{\u}$, it follows that $R_{\u-\w}=R_{\u}/R_{\w}^{\u-\w}$. Similarly $\bar R_{\u-\w}=\bar R_{\u}/\bar R_{\w}^{\u-\w}$. 
It follows that if $R_{\u}=\bar R_{\u}$ and $R_{\w}=\bar R_{\w}$ then $R_{\u+\w}=\bar R_{\u+\w}$ and $R_{\u-\w}=\bar R_{\u-\w}$. 
Thus, it follows by induction that $R_{\u}=\bar R_{\u}$ for all $\u\in\Z^k$.
\ProofStop


